FPGA Technology Mapping Using Sketch-Guided Program Synthesis

FPGA technology mapping is the process of implementing a hardware design expressed in high-level HDL (hardware design language) code using the low-level, architecture-specific primitives of the target FPGA. As FPGAs become increasingly heterogeneous, achieving high performance requires hardware synthesis tools that better support mapping to complex, highly configurable primitives like digital signal processors (DSPs). Current tools support DSP mapping via handwritten special-case mapping rules, which are laborious to write, error-prone, and often overlook mapping opportunities. We introduce Lakeroad, a principled approach to technology mapping via sketch-guided program synthesis. Lakeroad leverages two techniques -- architecture-independent sketch templates and semantics extraction from HDL -- to provide extensible technology mapping with stronger correctness guarantees and higher coverage of mapping opportunities than state-of-the-art tools. Across representative microbenchmarks, Lakeroad produces 2--3.5$\times$ the number of optimal mappings compared to proprietary state-of-the-art tools and 6--44$\times$ the number of optimal mappings compared to popular open-source tools, while also providing correctness guarantees not given by any other tool.

==> figures/correctness-comm-diagram.tex <==

\begin{figure}
\small
\adjustbox{scale=0.85,center}{%
\begin{tikzcd}
    \Spec \times \Sketch \times \VendorSemantics
       % LR
       \arrow[rrrrr, rightharpoonup, "{\lrfn}" description, bend left=30]
       % Run Spec
       \arrow[rrddd, "{\denote{s}_{\text{bv}}(i)}" description] 
       % Run Synth
        \arrow[rr, "\LRSynthFn", rightharpoonup]
      & & \lrir \arrow[rrr, "\HDLCompFn"]
                 \arrow[ddd, "{\denote{p}_{\lrir}(i)}" description]
      & & & \HDL\arrow[lllddd, "{\denote{v}_{\HDL}(i)}" description] \\
    & & & & &  \\
    & & & & &  \\
    & &  \textsc{Val} & & & 
\end{tikzcd}}
\caption{
  \lr Correctness Properties:
  {\small 
  The Synth-Correct Property (left triangle)
    running an \lrir program
    synthesized from a spec $s$
    has the same result
    as running the spec program directly.
  The Compile-Correct Property (right triangle)
    says that
    running an \lrir program
    is the same as compiling it to an HDL
    and simulating the HDL program.
The \lr-Correct Property
  combines the Synth-Correct Property
  and the Compile-Correct Property
  to provide a correctness guarantee for \lr.}}
\label{fig:correctness-comm-diagram}
\hl{fg is not in the diagram---how do we add?}
\hl{above specxsketchxsems, instead we have spec and sems going into that existing node, and sketch being generated by fg}


\hl{Another solution here (maybe what we currently have...) is that we just don't consider sketch generation in correctness, because it doesn't have an effect. then we would need to get rid of sketch generation section and all mentions of fg. we need to make sure to indicate why we can ignore sketch generation}
\end{figure}

==> figures/lakeroad-dsl-grammar.tex <==

%%%%%%%%%%%%%%%%%%%% Lakeroad DSL Grammar %%%%%%%%%%%%%%%%%%%%
\begin{figure}
% This line is causing a font error.
%\small
\setlength{\grammarparsep}{3pt plus 1pt minus 1pt} % increase separation between rules
\setlength{\grammarindent}{5em} % increase separation between LHS/RHS 
\small{}
\begin{grammar}

<\lowlrir> ::= `prim' name <list> <\lowlrir>
       \alt signal-const | signal-var  | <list> 
       \alt <signal-op> | <list-op>

<list>  ::= [<\lowlrir>\ldots]

<signal-op> ::= `extract' int int <\lowlrir>
         \alt `concat' <list>
%         \alt `zero-extend' int <lrir>

<list-op> ::= `list-ref' int <\lowlrir>
         % \alt `take' int <\lowlrir>
         % \alt `drop' int <\lowlrir>


% <routing> ::= `bitwise' | `bitwise-reverse'

% This isn't used
% <fpga-fn> ::= `ecp5-lut4' \ |\ \ldots

<sketch> ::= <\lowlrir> | <hole>

<hole> ::= `(' `bitvec' width `)' 
    \alt `(' `choose' <sketch> \ldots `)'
         
\end{grammar}

\caption{Syntax for \lrir.}
\label{fig:lakeroad-dsl-grammar}
\end{figure}
%%%%%%%%%%%%%%%%%%%% END LR DSL GRAMMAR %%%%%%%%%%%%%%%%%%%%

==> figures/lakeroad-dsl-interpreter.tex <==

%%%%%%%%%%%%%%%%%%%% LR DSL INTERPRETER %%%%%%%%%%%%%%%%%%%%
\begin{figure}
\begin{lstlisting}
(define (interpret expr)
 (match expr
  ;;; Lakeroad DSL
  [`(logical->physical ,_ ...)
   (interpret-log->phys interpret expr)]
  [`(physical->logical ,_ ...)
   (interpret-phys->log interpret expr)]
  
  ;;; FPGA Functions
  [`(ecp5-lut4 ,_ ...)
   (interpret-ecp5 interpret expr)]
 
  ;;; Racket functions lifted to Lakeroad DSL
  [`(append ,l0 ,l1)
   (append (interpret l0) (interpret l1))]
   ... 
   
  ;;; Rosette functions lifted to our language.
  [`(zero-extend ,v ,bv)
   (zero-extend (interpret v) bv)]
  [`(extract ,high ,low ,v)
   (extract high low (interpret v))]
  [`(concat ,v0 ,v1)
   (concat (interpret v0) (interpret v1))]
\end{lstlisting}
\caption{{\em The \lr DSL interpreter}}
\label{fig:lakeroad-dsl-interpreter}
\end{figure}
%%%%%%%%%%%%%%%%%%%% END LR DSL INTERPRETER %%%%%%%%%%%%%%%%%%%%


==> figures/lakeroad-dsl-semantics.tex <==
\begin{figure*}

\newcommand{\lrirSemanticsVspace}{5mm}

% \inference{\textrm{bv} ~ v}{v}[\lrir-bv]
% 
% \vspace{\lrirSemanticsVspace}

% \begin{subfigure}{0.32\textwidth}
%   \centering
  
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% LRIR-list
\mbox{
\inference{e_0 \Downarrow v_0 
   ~ \cdots ~ e_n \Downarrow v_n
}
          {     \left[ e_0,\, \ldots,\, e_n\right] 
                \Downarrow 
                \left[ v_0,\, \ldots,\, v_n\right] }
          [{\bf list}]}%
\quad
\mbox{\inference{l \Downarrow \lbrack v_0 \ldots v_i \ldots v_n\rbrack}
          {\texttt{list-ref}\ l\ i 
           \Downarrow 
           v_i}
          [{\bf list-ref}]
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% LRIR-prim
\quad
\mbox{
\inference%
  {e \Downarrow v 
  }
  {\texttt{prim}\ \rho\ \kappa\ e \Downarrow \Gamma(\rho)(\kappa)(v)}
  [{\bf prim}]
}

  \vspace{\lrirSemanticsVspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% LRIR-extract
\mbox{
\inference{e \Downarrow \left(\langle b_0 \ldots b_i \ldots b_j \ldots b_n\rangle, s \right)}
          {\texttt{extract}\ i\ j\ e \Downarrow \left( \langle b_i \ldots b_j \rangle, s \right)}
          [{\bf extract}]
}%
\quad
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% LRIR-concat
\mbox{
\inference{   e_0 \Downarrow \left(\langle b^0_0\ldots b^0_{n_1}\rangle, s_0 \right)
              ~ \cdots ~
              e_k \Downarrow \left( \langle b^k_0\ldots b^k_{n_k} \rangle, s_n\right)
& s = \bigcup^i s_i
              }
          {\texttt{concat}\ e_0,\,\ldots,\, e_k
           \Downarrow 
           \left(\langle b^0_0 \ldots b^0_{n_1} 
           \ldots
           b^k_0 \ldots b^k_{n_k} \rangle, 
           s\right)}
          [{\bf concat}]
}


% \end{subfigure}%
% \hspace{5mm}%
% \begin{subfigure}{0.25\textwidth}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% LRIR-take
% \inference{l \Downarrow \lbrack v_0 \ldots  
%                                 v_n\rbrack
%             & 0 \leq i \leq n+1}
%           {\texttt{take}\ l\ i 
%            \Downarrow 
%            \lbrack v_0,\, \ldots,\, v_{i-1} \rbrack}
%           [{\bf take}]
% \vspace{\lrirSemanticsVspace}

% \end{subfigure}\hspace{5mm}%
% \begin{subfigure}{0.32\textwidth}
%   \centering

          
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% LRIR-drop
% \inference{l \Downarrow \lbrack v_0 \ldots v_n\rbrack
%            & 0 \leq i \leq n+1 }
%           {\texttt{drop}\ l\ i 
%            \Downarrow 
%            \lbrack v_i,\, \ldots,\, v_{n} \rbrack}
%           [{\bf drop}]
% \vspace{\lrirSemanticsVspace}


          
% \end{subfigure}%


% \begin{subfigure}{.5\textwidth}
% \end{subfigure}%
% \hspace{5mm}%
% \begin{subfigure}{0.4\textwidth}
% \centering
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% LRIR-bitwise-phys-to-log
% \inference%
%   {l \Downarrow 
%          \lbrack 
%           \langle bv^0_0,\, \ldots,\,  bv^0_k\rangle,\,
%           \cdots,\,
%           \langle bv^n_0,\, \ldots,\,  bv^n_k\rangle
%          \rbrack}
%   {\texttt{wire}\ \ \texttt{bitwise}\ \ l
%    \Downarrow
%       \lbrack 
%        \langle bv^0_0,\, \ldots,\,  bv^n_0\rangle,\,
%        \cdots,\,
%        \langle bv^0_k,\, \ldots,\,  bv^n_k\rangle
%       \rbrack}
%   [{\bf bw-wire}]
% \vspace{\lrirSemanticsVspace}

% \end{subfigure}

\hspace{30mm}\begin{subfigure}{0.9\textwidth}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% LRIR-bwrev-phys-to-log
% \inference%
%   {l \Downarrow 
%          \lbrack 
%           \langle bv^0_0,\, \ldots,\,  bv^0_k\rangle,\,
%           \cdots,\,
%           \langle bv^n_0,\, \ldots,\,  bv^n_k\rangle
%          \rbrack}
%   {\texttt{wire}\ \ \texttt{bitwise-reverse}\ \ l
%    \Downarrow
%       \lbrack 
%        \langle bv_k^0,\, \ldots,\,  bv_k^n\rangle,\,
%        \cdots,\,
%        \langle bv_0^0,\, \ldots,\,  bv_0^n\rangle
%       \rbrack}
%   [{\bf bwrev-wire}]
% \vspace{\lrirSemanticsVspace}

\end{subfigure}
\caption{\lrir semantics. Angled brackets indicate bitvector literals, while square brackets indicate list literals.}
\label{fig:lrir-semantics}
\end{figure*}



% %%%% TRY 2 %%%%%
% \begin{figure*}
% \newcommand{\lrirSemanticsVspace}{5mm}

% \begin{subfigure}{0.3\textwidth}
%   \centering
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % LRIR-list
% \inference{e_0 \Downarrow v_0 & \cdots & e_n \Downarrow v_n}
%           {     \left[ e_0,\, \ldots,\, e_n\right] 
%                 \Downarrow 
%                 \left[ v_0,\, \ldots,\, v_n\right]}
%           [{\bf list}]
% \vspace{\lrirSemanticsVspace}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % LRIR-extract
% \inference{e \Downarrow \langle b_0 \ldots b_i \ldots b_j \ldots b_n\rangle}
%           {\texttt{extract}\ i\ j\ e \Downarrow \langle b_i \ldots b_j \rangle}
%           [{\bf extract}]
% \vspace{\lrirSemanticsVspace}
% \end{subfigure}
% \begin{subfigure}{0.3\textwidth}
%   \centering
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% % LRIR-prim
% \inference%
%   {e \Downarrow v 
%   }
%   {\texttt{prim}\ \rho\ \kappa\ e \Downarrow \Gamma(\rho)(\kappa)(x)}
%   [{\bf prim}]
% \vspace{\lrirSemanticsVspace}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % LRIR-list-ref

% \inference{l \Downarrow \lbrack v_0 \ldots v_i \ldots v_n\rbrack}
%           {\texttt{list-ref}\ l\ i 
%           \Downarrow 
%           v_i}
%           [{\bf list-ref}]
% \vspace{\lrirSemanticsVspace}
% \end{subfigure}
% \begin{subfigure}{0.3\textwidth}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % LRIR-take
% \inference{l \Downarrow \lbrack v_0 \ldots  
%                                 v_n\rbrack
%             & 0 \leq i \leq n+1}
%           {\texttt{take}\ l\ i 
%           \Downarrow 
%           \lbrack v_0,\, \ldots,\, v_{i-1} \rbrack}
%           [{\bf take}]
% \vspace{\lrirSemanticsVspace}
          
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % LRIR-drop
% \inference{l \Downarrow \lbrack v_0 \ldots v_n\rbrack
%           & 0 \leq i \leq n+1 }
%           {\texttt{drop}\ l\ i 
%           \Downarrow 
%           \lbrack v_i,\, \ldots,\, v_{n} \rbrack}
%           [{\bf drop}]
% \vspace{\lrirSemanticsVspace}
% \end{subfigure}
% \begin{subfigure}{\textwidth}
% \centering
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % LRIR-concat
% \inference{   e_1 \Downarrow \langle b^1_0\ldots b^1_{n_1}\rangle
%               & \cdots &
%               e_k \Downarrow \langle b^k_0\ldots b^k_{n_k} \rangle}
%           {\texttt{concat}\ e_1,\,\ldots,\, e_k
%           \Downarrow 
%           \langle b^1_0 \ldots b^1_{n_1} 
%           \ldots
%           b^k_0 \ldots b^k_{n_k} \rangle }
%           [{\bf concat}]
% \vspace{\lrirSemanticsVspace}
% \end{subfigure}
% \begin{subfigure}{\textwidth}
% \centering
% \inference%
%   {l \Downarrow 
%          \lbrack 
%           \langle bv^0_0,\, \ldots,\,  bv^0_k\rangle,\,
%           \cdots,\,
%           \langle bv^n_0,\, \ldots,\,  bv^n_k\rangle
%          \rbrack}
%   {\texttt{wire}\ \ \texttt{bitwise}\ \ l
%   \Downarrow
%       \lbrack 
%       \langle bv^0_0,\, \ldots,\,  bv^n_0\rangle,\,
%       \cdots,\,
%       \langle bv^0_k,\, \ldots,\,  bv^n_k\rangle
%       \rbrack}
%   [{\bf bw-wire}]
% \vspace{\lrirSemanticsVspace}
% \end{subfigure}
% %\hspace{30mm}\begin{subfigure}{0.9\textwidth}
% %\centering
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % LRIR-bitwise-phys-to-log
% \begin{subfigure}{0.9\textwidth}
% \centering
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % LRIR-bwrev-phys-to-log
% \inference%
%   {l \Downarrow 
%          \lbrack 
%           \langle bv^0_0,\, \ldots,\,  bv^0_k\rangle,\,
%           \cdots,\,
%           \langle bv^n_0,\, \ldots,\,  bv^n_k\rangle
%          \rbrack}
%   {\texttt{wire}\ \ \texttt{bitwise-reverse}\ \ l
%   \Downarrow
%       \lbrack 
%       \langle bv_k^0,\, \ldots,\,  bv_k^n\rangle,\,
%       \cdots,\,
%       \langle bv_0^0,\, \ldots,\,  bv_0^n\rangle
%       \rbrack}
%   [{\bf bwrev-wire}]
% \vspace{\lrirSemanticsVspace}
% \end{subfigure}
% \caption{\lrir semantics.}
% \label{fig:lrir-semantics}
% \end{figure*}


% \inference{l \in [\textrm{BV}], \textrm{logical-to-physical}~\textrm{bitwise}~l}
% {
% [(\textrm{concat}~(\textrm{extract}~0~0~l[0])~%
% (\textrm{extract}~0~0~l[1])~\dots)~%
% (\textrm{concat}~(\textrm{extract}~1~1~l[0])~%
% (\textrm{extract}~1~1~l[1])~\dots)~\dots ]
% }
% [\lrir-ltop-bitwise]

% \vspace{\lrirSem\lrirSemanticsVspace}

% \inference{l \in [\textrm{BV}], \textrm{logical-to-physical}~\textrm{bitwise-reverse}~l}
% {
% \begin{array}{@{}c@{}}
% [(\textrm{concat}~(\textrm{extract}~n~n~l[0])~%
% (\textrm{extract}~n~n~l[1])~\dots)   \\
% (\textrm{concat}~(\textrm{extract}~n-1~n-1~l[0])~%
% (\textrm{extract}~n-1~n-1~l[1])~\dots)~\dots ]
% \end{array}
% }
% [\lrir-ltop-bitwise-reverse]

% \vspace{\lrirSem\lrirSemanticsVspace}

% \inference
% {\textrm{primitive}~n~e}
% {\textrm{look up primitive semantics for $n$, run on $e$}}

==> figures/lakeroad-yosys-lattice.tex <==
\begin{table}[]
\caption{Synthesis time and resource usage when synthesizing various expressions for Lattice ECP5 using our \texttt{\lowercaselr} command and using the existing \texttt{synth\_ecp5} command in Yosys.}
\label{tab:yosys-lattice}
\hl{Replace this figure with more expansive DSP tables}
\setlength{\tabcolsep}{2pt}
\centering
\begin{tabular}{l|lll|lll}
\hline
instruction       & \multicolumn{3}{l|}{\texttt{\lowercaselr}} & \multicolumn{3}{l}{\texttt{synth\_ecp5}} \\
(all 16 bit)      & time (s)    & MULT         & ALU         & time (s)  & MULT        & CCU2C        \\ \hline
$a\times b$       & 1.42         & 1        & 1       & 0.65        & 1       &         \\
$(a\times b) + c$ & 1.87         & 1        & 1       & 0.74        & 1       & 8       \\
$(a\times b) - c$ & 1.61         & 1        & 1       & 0.61        & 1       & 8      
\end{tabular}
\end{table}

==> figures/lakeroad-yosys-xilinx.tex <==
\begin{table}[]
\caption{Synthesis time and resource usage when synthesizing various expressions for Xilinx UltraScale+ using our \texttt{\lowercaselr} command and using the existing \texttt{synth\_xilinx} command in Yosys.}
\label{tab:yosys-xilinx}
\hl{Replace this figure with more expansive DSP tables}
\setlength{\tabcolsep}{2pt}
\centering
\begin{tabular}{l|ll|llll}
\hline
instruction                      & \multicolumn{2}{l|}{\texttt{\lowercaselr}} & \multicolumn{4}{l}{\texttt{synth\_xilinx}} \\
(all 16 bit)                     & time (s)           & DSP          & time (s)  & DSP  & LUT2  & CARRY4 \\ \hline
$a\times b$                      & 2.49               & 1            & 4.03      & 1    &       &        \\
$((a+b) \times c)+d$             & 2.44               & 1            & 4.18      & 1    & 32    & 8      \\
$(a\times b) + c$                & 3.02               & 1            & 4.02      & 1    & 16    & 4      \\
$(a+b)\times c$                  & 1.75               & 1            & 3.83      & 1    & 16    & 4      \\
$(a+b)^2$                        & 1.84               & 1            & 3.83      & 1    & 16    & 4      \\
$(a-b)^2$                        & 2.29               & 1            & 3.82      & 1    & 16    & 4      \\
$(a-b)^2 - c$                    & 21.7               & 1            & 3.93      & 1    & 32    & 8      \\
$(a+b)^2 +c$                     & 2.17               & 1            & 3.92      & 1    & 32    & 8      \\
$((a+b)\times c) \oplus d$       & 1.87               & 1            & 3.92      & 1    & 32    & 4      \\
$\sim(((a+b)\times c) \oplus d)$ & 2.43               & 1            & 4.01      & 1    & 32    & 4     
\end{tabular}
\end{table}

==> figures/semantics.tex <==
\centering
$\textsc{BV} \inferrule {P[i] = v}
                            {\smallStep{P}{i}{E}{t}{v}}$ \quad 
%
$\textsc{Var} 
\inferrule {P[i] = x \quad E[x][t] = v } 
{ \smallStep{P}{i}{E}{t}{v} }$ \quad\\[1em]
%
$\textsc{Op} 
\inferrule { 
o \in \Op \quad
P[i] = o\ i_1\ \ldots\ i_n \quad
\smallStep{P}{i_1}{E}{t}{v_1} \quad
\ldots \quad
\smallStep{P}{i_k}{E}{t}{v_n} \quad    % INPUT n
\quad 
v = \llbracket o \rrbracket(v_1, \ldots, v_n)}
{ \smallStep{P}{i}{E}{t}{v} }$ \\[1em]

$\textsc{RegZero}
\inferrule{
  P[i] =\ $\IRReg$\ i_{clk}\ i_{data}\ v_{init}
}{\smallStep{P}{i}{E}{0}{v_{init}}}$\\[1em]

$\textsc{RegHold} 
\inferrule {
  t > 0 \quad
  P[i] =\ $\IRReg$\ i_{clk}\ i_{data}\ v_{init} \quad
  \smallStep{P}{i_{clk}}{E}{t}{v_{clk}} \quad
  \smallStep{P}{i_{clk}}{E}{t-1}{v_{oldClk}} \quad
  \smallStep{P}{i}{E}{t-1}{v_{oldQ}} \quad
  (v_{oldClk}, v_{clk}) \neq (0, 1)
  } 
{ \smallStep{P}{i}{E}{t}{v_{oldQ}} }$ \\[1em]

$\textsc{RegTick} 
\inferrule {
  t > 0 \quad
  P[i] =\ $\IRReg$\ i_{clk}\ i_{data}\ v_{init} \quad
  \smallStep{P}{i_{clk}}{E}{t}{v_{clk}} \quad
  \smallStep{P}{i_{clk}}{E}{t-1}{v_{oldClk}} \quad
  \smallStep{P}{i_{data}}{E}{t-1}{v_{oldData}} \quad
  (v_{oldClk}, v_{clk}) = (0, 1)
  } 
{ \smallStep{P}{i}{E}{t}{v_{oldData}} }$ \\[1em]

% 2023/10/21: Gus added a "hack" that might fix the prim problem of not putting streams in the environment, but we still may wanna do away with these inference rules altogether in favor of the interpreter pseudocode
$\textsc{Prim} 
\inferrule {
  P[i] = \SynPrim\ \langle x_1,\ldots, x_n\rangle\
                   \langle i_1, \ldots, i_n\rangle\
                   p \quad
  % \smallStep{P}{i_1}{E}{t}{v_1} \quad 
  % \ldots \quad 
  % \smallStep{P}{i_n}{E}{t}{v_n} \quad 
  1 \leq j \leq n\quad 
  \smallStep{P}{i_j}{E}{0}{v_j^0} \quad 
  \cdots \quad
  \smallStep{P}{i_j}{E}{t}{v_j^t} \quad 
  E^\prime = E\left[x_j \mapsto \left[v_j^0, \dots, v_j^t\right]\right] \quad
  \smallStep{p}{p.root}{E^\prime}{t}{v}
} 
{ \smallStep{P}{i}{E}{t}{v} }$ \\[1em]

$\textsc{Step}
\inferrule {
\smallStep{P}{P.root}{E}{t}{v}
}{\bigStep{P}{E}{t}{v}}
$

% \separatingline \vspace{1em}

% $\textsc{OneCycle} \inferrule { \evalsTo{e}{E}{S}{v}{S'} } { \multiEvalsTo{[E]}{e}{S}{v}{S'} }$ \quad
% $\textsc{MultiCycle} \inferrule { \evalsTo{e}{E_1}{S}{v_{ignore}}{S'} \quad 
% \multiEvalsTo{[E_2, \ldots, E_n]}{e}{S'}{v}{S''} } { \multiEvalsTo{[E_1, E_2, \ldots, E_n]}{e}{S}{v}{S''} }$ \\[1em]

==> figures/signal-pseudocode.tex <==
\begin{figure}
\begin{minted}[fontsize=\footnotesize]{python}
def register(clk, d):
  # look up previous values
  s = merge(clk.state, d.state)
  (old_clk_val, _) = s.get_or_default("clk", (0, _))
  (old_d_val, _) = s.get_or_default("d", (0, _))
  (old_q_val, _) = s.get_or_default("q", (0, _))

  # compute the output
  clock_ticked = old_clk_val == 0 and clk.value == 1
  new_q_val = old_d_val if clock_ticked else old_q_value
  new_state = s.update("clk", clk.value)
               .update("d", d.value)
               .update("q", new_q_value)
  
  return signal(new_q_val, new_state)

>>> v0 = register(signal(0), signal(0xa)); v0
signal(0, {"clk": (0, 0), "d": (0xa, 0), "q": (0, 0) })
>>> register(signal(1, v0.state), signal(0xa, v0.state))
signal(0xa, {"clk": (1, 1), "d": (0xa, 1), "q": (0xa, 1) })
\end{minted}
    \caption{
Pseudocode implementation 
  of a simple register 
  using the \texttt{signal} data structure.
The register takes two \texttt{signal}s as input:
  \texttt{clk} and \texttt{d}.
The states from the two inputs are first merged
  into a single map,
  which is used to look up old values of
  \texttt{clk}, \texttt{d},
  and the output \texttt{q}.
Finally, we compute
  the new value of \texttt{q}
  based on whether or not
  the clock ticked.
}
    \label{fig:signal-example}
\hl{explain: register is a very simple examplke, and we dont' actually have a register primitive, but registers are contained within many of our complex primitives}
\end{figure}

==> figures/signal-state.tex <==
\begin{figure} 
\begin{minted}[fontsize=\footnotesize]{python}
def merge(state0, ...):
  new_s = {}
  for s in [state0, ...], key in s:
    (new_val, new_vers) = s.get(key)
    (_, old_vers) = new_s.get_or_default(key, (_, -1))
    if new_vers > old_vers:
      new_s[key] = (new_val, new_vers)
  return new_s

def update(state, key, val):
  new_state = state.copy()
  (_, old_vers) = state.get_or_default(key, (_, -1))
  new_state[key] = (val, old_vers + 1)
  return new_state

def register(clk, d):
  # look up previous values
  s = merge(clk.state, d.state)
  (old_clk_val, _) = s.get_or_default("clk", (0, _))
  (old_d_val, _) = s.get_or_default("d", (0, _))
  (old_q_val, _) = s.get_or_default("q", (0, _))

  # compute the output
  clock_ticked = old_clk_val == 0 and clk.value == 1
  new_q_val = old_d_val if clock_ticked else old_q_value
  new_state = s.update("clk", clk.value)
               .update("d", d.value)
               .update("q", new_q_value)
  
  return signal(new_q_val, new_state)

>>> v0 = register(signal(0), signal(0xa)); v0
signal(0, {"clk": (0, 0), "d": (0xa, 0), "q": (0, 0) })
>>> register(signal(1, v0.state), signal(0xa, v0.state))
signal(0xa, {"clk": (1, 1), "d": (0xa, 1), "q": (0xa, 1) })
\end{minted}
    \caption{
Pseudocode implementation 
  of the core \signal operations
  (\texttt{merge} and \texttt{update}),
  and a demonstration of how \signal{}s
  can be used to implement the semantics
  of a simple register. 
The register takes two \texttt{signal}s as input:
  \texttt{clk} and \texttt{d}.
The states from the two inputs are first merged
  into a single map,
  which is used to look up old values of
  \texttt{clk}, \texttt{d},
  and the output \texttt{q}. 
Version numbers in the state maps
  help resolve potential merge conflicts.
Finally, we compute
  the new value of \texttt{q}
  based on whether or not
  the clock ticked. 
Note that this is just an example;
  \lrir does not include
  a register primitive.
Rather, registers are contained within
  the Verilog models
  we import, and their semantics
  are captured in 
  \cref{fig:verilog-semantics}
  (see \textbf{dff-hold} and \textbf{dff-tick}).
}
    \label{fig:signal-complete}
\end{figure}

==> figures/sketch-generation.tex <==
\begin{figure*}

\tikz{

\node[minimum width=3cm] at (0, .1) {\large\textsf{\textbf{Sketch Template}}};
\node[minimum width=3cm] at (6, 2.5) {\large\textsf{\textbf{Architecture Descriptions}}};
\node[minimum width=3cm] at (12, 2.1) {\large\textsf{\textbf{Sketches}}};

\node[rectangle,rounded corners, draw, minimum width=4.5cm]
at (0,-1)
(sketch-template)
{\begin{minipage}{.2\textwidth}
\begin{minted}[fontsize=\footnotesize,xleftmargin=-12pt]{python}
def dsp_sketch_template(
    clk, I0, I1, I2, I3):
  o = dsp(clk, I0, I1, I2, I3)
  return o
\end{minted}
\end{minipage}};

% Xilinx arch desc
\node[rectangle,rounded corners, draw, minimum width=5.3cm]
at (6,1)
(xilinx-arch-desc)
{\begin{minipage}{.25\textwidth}
\begin{minted}[fontsize=\footnotesize,xleftmargin=-5pt]{YAML}
# Xilinx
dsp:
- { module_name: DSP48E2,
    ports: {A: I0, ...},
    params: {AREG: <AREG>, ...},
    symbolics: {<AREG>: 32, ... }}
\end{minted}
\end{minipage}};

% lattice arch desc
\node[rectangle,rounded corners, draw, minimum width=5.9cm]
at (6,-2)
(lattice-arch-desc)
{\begin{minipage}{.25\textwidth}
\begin{minted}[fontsize=\footnotesize,xleftmargin=-10pt]{YAML}
# Lattice
dsp:
- { id: mul, module_name: MULT18X18C,
    ports: {A: I0, ... },
    params: {CMREG: <CMREG>, ...},
    symbolics: {<CMREG>: 5, ...},
- { module_name: ALU54A,
    ports: {B: mul.o, C: I2, ... },
    params: {RFCLK: <RFCLK>, ... },
    symbolics: {<RFCLK>: 5, ... }}
\end{minted}
\end{minipage}};



\node[rectangle,rounded corners, draw, minimum width=5.7cm]
at (12,1)
(xilinx-sketch)
{\begin{minipage}{.25\textwidth}
\begin{minted}[fontsize=\footnotesize,xleftmargin=-11pt]{python}
def sketch_xil(clk, I0, I1, I2, I3):
    o = DSP48E2(clk=clk, A=IO,
                AREG=<AREG>, ...)
    return o
\end{minted}
\end{minipage}};

\node[rectangle,rounded corners, draw, minimum width=5.7cm]
at (12,-2)
(lattice-sketch)
{\begin{minipage}{.25\textwidth}
\begin{minted}[fontsize=\footnotesize,xleftmargin=-11pt]{python}
def sketch_lat(clk, I0, I1, I2, I3):
    o1 = MULT18X18C(clk=clk, A=I0,
            CMREG=<CMREG>, ...)
    o2 = ALU54A(clk=clk, B=o1,
            C=I2, RFCLK=<RFCLK>, ...)
    return o2
\end{minted}
\end{minipage}};

\draw[->] (sketch-template) edge (xilinx-arch-desc);
\draw[->] (sketch-template) edge (lattice-arch-desc);
\draw[->] (xilinx-arch-desc) edge (xilinx-sketch);
\draw[->] (lattice-arch-desc) edge (lattice-sketch);




}

% \begin{subfigure}{0.32\textwidth}
% \centering
% \begin{minted}[frame=single,fontsize=\footnotesize]{python}
% def dsp_sketch_template(
%     clk, a, b, c, d):
%   (o, ...) = dsp(clk, a, b, c, d)
%   return o
% \end{minted}
% \vspace{2cm}
% \end{subfigure}

% \hspace{5mm}%
% \begin{subfigure}{0.25\textwidth}


% % # Xilinx
% % - module_name: DSP48E2
% %   ports: 
% %    [{name: A, dir: in, val: ...},
% %     {name: B, dir: in, val: ...}, ...]
% %   parameters: 
% %    [{name: MREG, val: ...}, ...]
% % # Lattice
% % - module_name: MULT18X18C
% %   ports:
% %   [{name: A, dir: in, val: ...},
% %    {name: B, dir: in, val: ...}, ...]
% %   parameters:
% %   [{name: MULT_BYPASS, val: ...}, ...]
% % - module_name: ALU45A
% %   ports:
% %   [{name: MA, dir: in, val: ...},
% %    {name: MB, dir: in, val: ...}]
% %  parameters:
% %   [{name: REG_FLAG_CLK, dir: in, val: ...}, ...]

% \begin{minted}[frame=single,fontsize=\footnotesize]{YAML}
% # Xilinx
% dsp:
% - { module_name: DSP48E2,
%     ports: ..., params: ... }
% \end{minted}
  
% \begin{minted}[frame=single,fontsize=\footnotesize]{YAML}
% # Lattice
% dsp:
% - { module_name: MULT18X18C,
%     ports: ..., params: ... }
% - { module_name: ALU54A,
%     ports: ..., params: ... }
% \end{minted}
% \end{subfigure}
% \hspace{5mm}%
% \begin{subfigure}{0.32\textwidth}
% \begin{minted}[frame=single,fontsize=\footnotesize]{python}
% def sketch_xilinx(clk, a, b, c, d):
%     (o, ...) = DSP48E2(clk, a, b, c,
%         d, MREG=..., ...)
%     return o
% \end{minted}

% \begin{minted}[frame=single,fontsize=\footnotesize]{python}
% def sketch_lattice(clk, a, b, c, d):
%     (o0, ...) = MULT18X18C(clk, a,
%         b, MULT_BYPASS=..., ...)
%     (o1, ...) = ALU54A(clk, c, 
%         o0, REG_FLAG_CLK=..., ...)
%     return o1
% \end{minted}
% \end{subfigure}

    \caption{
    The inputs/outputs of \lr's sketch generation flow.
    The first column is the abstract DSP sketch template.
    The second column contains condensed architecture descriptions for Xilinx UltraScale+ and Lattice ECP5, which are used to specialize the sketch template.
    % Observe that although Lattice's DSP is comprised of
    % two hardware primitives, the overall approach remains the same for each primitive.
    The third column represents the specialized sketches on each architecture.
}
    \label{fig:sketch-generation}

\end{figure*}

==> figures/state-merge-and-update.tex <==
\begin{figure}
\begin{minted}[fontsize=\footnotesize]{python}
def merge(state0, ...):
  new_s = {}
  for s in [state0, ...], key in s:
    (new_val, new_vers) = s.get(key)
    (_, old_vers) = new_s.get_or_default(key, (_, -1))
    if new_vers > old_vers:
      new_s[key] = (new_val, new_vers)
  return new_s

def update(state, key, val):
  new_state = state.copy()
  (_, old_vers) = state.get_or_default(key, (_, -1))
  new_state[key] = (val, old_vers + 1)
  return new_state
\end{minted}
% In case we want to add examples
% >>> v0 = register(signal(0), signal(0xa)); v0
% signal(0, {"clk": 0, "d": 0xa, "q": 0 })
% >>> register(signal(1, v0.state), signal(0xa, v0.state))
% signal(0xa, {"clk": 1, "d": 0xa, "q": 0xa })
    \caption{
% Pseudocode implementation 
%   of a simple register 
%   using the \texttt{signal} data structure.
% The register takes two \texttt{signal}s as input:
%   \texttt{clk} and \texttt{d}.
% The states from the two inputs are first merged
%   into a single map,
%   which is used to look up old values of
%   \texttt{clk}, \texttt{d},
%   and the output \texttt{q}.
% Finally, we compute
%   the new value of \texttt{q}
%   based on whether or not
%   the clock ticked.
Pseudocode implementation
  of merging two state
  maps.
Versioning guarantees
  resolution in the case
  of state merge conflict.
}

    \label{fig:state-merge-and-update}
\end{figure}

==> figures/verilog-syntax.tex <==
\begin{figure}
% This line is causing a font error.
%\small
\setlength{\grammarparsep}{3pt plus 1pt minus 1pt} % increase separation between rules
\setlength{\grammarindent}{5em} % increase separation between LHS/RHS 
\small{}
\begin{grammar}

<expr> ::= signal-const | signal-var  
\alt <unop> <expr> 
        \alt <binop> <expr> <expr>
        \alt <ternop> <expr> <expr> <expr>
        
<unop> ::=  `not' | `neg' | `reduce_and' | `reduce_xor'
    
<binop> ::= `and'  | `or' | `xor'
    \alt  `eq' | `ne' | `logic_and' | `logic_not' | `logic_or' 
    \alt  `mul' | `add' | `sub' 
    \alt  `dff'
    \alt `concat'

<ternop> ::=  `mux'  | `extract'

\end{grammar}

\caption{
Syntax for imported Verilog.
This syntax is largely drawn from
  Yosys's~\cite{wolf2013yosys} internal syntax.
}
\label{fig:verilog-syntax}
\end{figure}

==> figures/yosys-semantics.tex <==
% Stateful
% $ff
% OR should we do $dff?
% Probably $dff. The difference is that one gets a clock and the other doesn't. That is, dff takes D and CLK inputs and has Q output, ff has just D and Q.

% Combinational:
% $add        
% $and        
% $eq         
% $eqx        
% $logic_and  
% $logic_not  
% $logic_or   
% $mul        
% $mux        
% $ne         
% $not        
% $or         
% $reduce_and 
% $reduce_bool
% $reduce_or  
% $reduce_xor 
% $sub        
% $xor        

\begin{figure*}

\mbox{
\inference{
e \Downarrow (v, s)
}{
\texttt{not}(e) \Downarrow (\sim{} v, s)
}[\textbf{not}]
}
% \mbox{
% \inference{
% e \Downarrow (v, s)
% }{
% \texttt{neg}(e) \Downarrow (-v, s)
% }[\textbf{neg}]
% }
\mbox{
\inference{
e \Downarrow \left(\langle b_0, \dots, b_n \rangle, s\right)
}{
\texttt{reduce\_or}(e) \Downarrow \left(\langle b_0 \:|\: \dots \:|\: b_n \rangle, s\right)
}[\textbf{redor}]
}
\quad
\mbox{
\inference{
e_0 \Downarrow (v_0, s_0)
\quad
e_1 \Downarrow (v_1, s_1)
& 
s = s_0 \cup s_1
}{
\texttt{and}(e_0, e_1) \Downarrow \left(v_0 \:\&\: v_1, s\right)
}[\textbf{and}]
}%

\bigbreak

\mbox{
\inference{
e_0 \Downarrow (v_0, s_0)
\quad
e_1 \Downarrow (v_1, s_1)
& 
s = s_0 \cup s_1
}{
\texttt{eq}(e_0, e_1) \Downarrow \left(
\langle 1 \rangle~\text{if}~v_0 = v_1~\text{else}~\langle 0 \rangle, s\right)
}[\textbf{eq}]
}%
\quad
\mbox{
\inference{
e_0 \Downarrow (v_0, s_0)
\quad
e_1 \Downarrow (v_1, s_1)
\quad
e_s \Downarrow (v_s, s_s)
& 
s = s_0 \cup s_1 \cup s_s
}{
\texttt{mux}(e_s, e_0, e_1) \Downarrow \left(
v_0~\text{if}~v_s = \langle 0 \rangle~\text{else}~v_1, s\right)
}[\textbf{mux}]
}%

% \mbox{
% \inference{
% e_0 \Downarrow (v_0, s_0)
% & 
% e_1 \Downarrow (v_1, s_1)
% & 
% s = s_0 \cup s_1
% }{
% \texttt{or}(e_0, e_1) \Downarrow \left(v_0 \:|\: v_1, s\right)
% }[\textbf{or}]
% }%
\quad

\bigbreak

% DFF without clock tick
\mbox{
\inference{
    e =
    \texttt{dff}(e_\mathit{clk}, e_d)
    &
    e_\mathit{clk} \Downarrow 
        \left(\mathit{clk},
        s_\mathit{clk}\right)
    &
    e_d \Downarrow 
        \left(d, s_d\right)
    \\
    s = s_\mathit{clk} \cup s_d
    % &
    % \left(q', d', \mathit{clk}'\right)
    %     =
    %     \left(
    %     s[e], s[e_d], 
    %         s[e_\mathit{clk}]
    %     \right)
    % \\
    &
    \left(s[e_\mathit{clk}],
            \mathit{clk} \right)
    \neq
    \left( 0, 1 \right)
}{
    e 
    \Downarrow
    \left(
        s[e],
        s[
            e := s[e],
            e_\mathit{clk} :=
            \mathit{clk},
            e_d := d]
    \right)
}
[\textbf{dff-hold}]
}%
\quad
% DFF with clock tick
\mbox{
\inference{
    e =
    \texttt{dff}(e_\mathit{clk}, e_d)
    &
    e_\mathit{clk} \Downarrow 
        \left(\mathit{clk},
        s_\mathit{clk}\right)
    &
    e_d \Downarrow 
        \left(d, s_d\right)
    \\
    s = s_\mathit{clk} \cup s_d
    &
    % \left(q', d', \mathit{clk}'\right)
    %     =
    %     \left(
    %     s[e], s[e_d], 
    %         s[e_\mathit{clk}]
    %     \right)
    % \\
    \left( s[e_\mathit{clk}],
            \mathit{clk} \right)
    =
    \left( 0, 1 \right)
}{
    e 
    \Downarrow
    \left(
       s[e_d],
        s[
            e :=s[e_d],
            e_\mathit{clk} :=
            \mathit{clk},
            e_d := d]
    \right)
}
[\textbf{dff-tick}]
}

\caption{
A representative set
  of the semantics rules
  for the subset of Verilog
  supported by \lr.
$s_0\cup s_1$ and $s[k:=v]$ 
  represent state map merging
  and updating, respectively.
}\label{fig:verilog-semantics}

\end{figure*}



==> generated/XiLiNx.tex <==
\rotatebox{\titletilt}{ Instr } & \rotatebox{\titletilt}{ Template } & \rotatebox{\titletilt}{ Runtime in sec } & \rotatebox{\titletilt}{ \#LUTs } & \rotatebox{\titletilt}{ \#CARRY8s } & \rotatebox{\titletilt}{ DSP? (sec) } & \rotatebox{\titletilt}{ Runtime } & \rotatebox{\titletilt}{ \#LUTs } & \rotatebox{\titletilt}{ \#MUXs } & \rotatebox{\titletilt}{ \#CARRY4s } & \rotatebox{\titletilt}{ \#INVs } & \rotatebox{\titletilt}{ \#DSP } & \rotatebox{\titletilt}{ Runtime in sec } & \rotatebox{\titletilt}{ \#LUTs } & \rotatebox{\titletilt}{ \#CARRY8s } & \rotatebox{\titletilt}{ \#DSP } & \rotatebox{\titletilt}{ Support } \\\midrule
and8  & BW    & 1.5  & 8  & -- & \checkmark (3.0) & 2.6 & 8 & -- & -- & -- & --  & 32 & 4 & -- &  -- & $\times$ \\
and16 & BW    & 1.6  & 16 & -- & \checkmark (4.8) & 2.6 & 16 & -- & -- & -- &--   & 36 & 10 & -- &--   & $\times$ \\
and32 & BW    & 1.9  & 32 & -- &                  & 2.6 & 32 & -- & -- & -- &--   & 35 & 17 & -- &--   & $\times$ \\
or8   & BW    & 1.7  & 8  & -- & \checkmark (7.4) & 2.5 & 8 & -- & -- & -- & --  & 32 & 4 & -- &  -- & $\times$ \\
or16  & BW    & 1.8  & 16 & -- & \checkmark (7.1) & 2.6 & 16 & -- & -- & -- &--   & 34 & 10 & -- &--   & $\times$ \\
or32  & BW    & 1.7  & 32 & -- &                  & 2.6 & 32 & -- & -- & -- &--   & 31 & 17 & -- &--   & $\times$ \\
xor8  & BW    & 1.7  & 8  & -- & \checkmark (5.1) & 2.6 & 8 & -- & -- & -- & --  & 33 & 4 & -- &  -- & $\times$ \\
xor16 & BW    & 1.9  & 16 & -- & \checkmark (4.4) & 2.7 & 16 & -- & -- & -- &--   & 32 & 10 & -- &--   & $\times$ \\
xor32 & BW    & 2.2  & 32 & -- &                  & 2.5 & 32 & -- & -- & -- &--   & 33 & 17 & -- &--   & $\times$ \\
not8  & BW    & 1.6  & 8  & -- & \checkmark (2.8) & 2.6 & -- & -- & -- & 8 & --  & 34 & 4 & -- &  -- & $\times$ \\
not16 & BW    & 1.8  & 16 & -- & \checkmark (3.6) & 2.6 & -- & -- & -- & 16 &--   & 32 & 10 & -- &--   & $\times$ \\
not32 & BW    & 1.7  & 32 & -- &                  & 2.6 & -- & -- & -- & 32 &--   & 33 & 17 & -- &--   & $\times$ \\
mux8  & BW    & 6.0  & 8  & -- & \checkmark (4.1) & 2.6 & 8 & -- & -- & -- & --  & 35 & 8 & -- & --  & $\times$ \\
mux16 & BW    & 8.5  & 16 & -- & \checkmark (6.3) & 2.6 & 16 & -- & -- & -- &--   & 31 & 16 & -- & -- & $\times$ \\
mux32 & BW    & 12.7 & 32 & -- &                  & 2.8 & 32 & -- & -- & -- &--   & 22 & 32 & -- & -- & $\times$ \\
add8  & Carry & 2.0  & 8  & 1 & \checkmark (3.7) & 2.6 & 8 & -- & 2 & -- &   --& 33 & 11 & -- & -- & $\times$ \\
add16 & Carry & 2.3  & 16 & 2 & \checkmark (4.8) & 2.8 & 16 & -- & 4 & -- &  -- & 34 & 16 & 2 & -- & $\times$ \\
add32 & Carry & 2.3  & 32 & 4 &                  & 2.7 & 32 & -- & 8 & -- &  -- & 34 & 32 & 4 & -- & $\times$ \\
sub8  & Carry & 2.0  & 8  & 1 & \checkmark (3.3) & 2.6 & 8 & -- & 2 & -- &   --& 33 & 11 & -- & -- & $\times$ \\
sub16 & Carry & 1.9  & 16 & 2 & \checkmark (3.9) & 2.7 & 16 & -- & 4 & -- &  -- & 34 & 16 & 2 & -- & $\times$ \\
sub32 & Carry & 1.9  & 32 & 4 &                  & 2.7 & 32 & -- & 8 & -- &  -- & 34 & 32 & 4 & -- & $\times$ \\
mul8  & Mult  & 2.0  & 91 & 8 & \checkmark (7.6) & 2.8 & 55 & 15 & 2 & -- &  -- & 36 & 33 & 3 & -- & $\times$ \\
mul16 & --   & 2.4  & -- & -- & \checkmark (2.4) & 3.4 & -- & -- & -- & -- & 1 & 32 & -- & -- & 1  & $\times$ \\
mul32 & --    & --   & -- & -- &                  & 3.6 & -- & -- & -- & -- & 3  & 22 & -- & -- & 3  & $\times$ \\
eq8   & Comp  & 1.8  & 8  & 1 &                   & 2.6 & 3 & -- & -- & -- &  -- & 37 & 3 & -- &--    & $\times$ \\
eq16  & Comp  & 1.8  & 16 & 2 &                   & 2.7 & 9 & 12 & -- & -- &  -- & 35 & 7 & -- &--    & $\times$ \\
eq32  & Comp  & 3.3  & 32 & 4 &                   & 2.6 & 24 & 1 & -- & -- &  -- & 36 & 11 & 2 &--    & $\times$ \\
neq8  & Comp  & 2.1  & 8  & 1 &                   & 2.6 & 3 & -- & -- & -- &  -- & 33 & 3 & -- &--    & $\times$ \\
neq16 & Comp  & 2.6  & 16 & 2 &                   & 2.7 & 9 & 12 & -- & -- &  -- & 23 & 7 & -- &--    & $\times$ \\
neq32 & Comp  & 3.5  & 32 & 4 &                   & 2.7 & 24 & 1 & -- & -- &  -- & 33 & 11 & 2 &--    & $\times$ \\
ugt8  & Comp  & 2.7  & 8  & 1 &                   & 2.6 & 6 & -- & 1 & -- &   --& 37 & 4 & 1 &  --  & $\times$ \\
ugt16 & Comp  & 3.5  & 16 & 2 &                   & 2.7 & 12 & -- & 2 & -- &  -- & 38 & 8 & 1 & --   & $\times$ \\
ugt32 & Comp  & 3.4  & 32 & 4 &                   & 2.7 & 22 & -- & 3 & -- &  -- & 32 & 16 & 2 &--    & $\times$ \\
ult8  & Comp  & 2.7  & 8  & 1 &                   & 2.6 & 6 & -- & 1 & -- &   --& 30 & 4 & 1 &  -- & $\times$ \\
ult16 & Comp  & 3.3  & 16 & 2 &                   & 2.7 & 12 & -- & 2 & -- &  -- & 32 & 8 & 1 & --  & $\times$ \\
ult32 & Comp  & 3.7  & 32 & 4 &                   & 2.7 & 22 & -- & 3 & -- &  -- & 34 & 16 & 2 &--   & $\times$ \\
uge8  & Comp  & 2.5  & 8  & 1 &                   & 2.7 & 6 & -- & 1 & -- &   --& 32 & 4 & 1 &  -- & $\times$ \\
uge16 & Comp  & 2.4  & 16 & 2 &                   & 2.7 & 12 & -- & 2 & -- &  -- & 34 & 8 & 1 & --  & $\times$ \\
uge32 & Comp  & 2.8  & 32 & 4 &                   & 2.8 & 22 & -- & 3 & -- &  -- & 33 & 16 & 2 &--   & $\times$ \\
ule8  & Comp  & 2.6  & 8  & 1 &                   & 2.7 & 6 & -- & 1 & -- &   --& 34 & 4 & 1 &  -- & $\times$ \\
ule16 & Comp  & 2.5  & 16 & 2 &                   & 2.7 & 12 & -- & 2 & -- &  -- & 32 & 8 & 1 & -- & $\times$ \\
ule32 & Comp  & 2.5  & 32 & 4 &                   & 2.8 & 22 & -- & 3 & -- &  -- & 32 & 16 & 2 &--  & $\times$

==> generated/final-compressed.tex <==
\rotatebox{\titletilt}{ Instr } & \rotatebox{\titletilt}{ Template } & \rotatebox{\titletilt}{ Runtime in sec } & \rotatebox{\titletilt}{ \#LUTs } & \rotatebox{\titletilt}{ \#CARRY8s } & \rotatebox{\titletilt}{ Runtime } & \rotatebox{\titletilt}{ \#LUTs } & \rotatebox{\titletilt}{ \#MUXs } & \rotatebox{\titletilt}{ \#CARRY4s } & \rotatebox{\titletilt}{ \#INVs } & \rotatebox{\titletilt}{ Runtime in sec } & \rotatebox{\titletilt}{ \#LUTs } & \rotatebox{\titletilt}{ \#CARRY8s } & \rotatebox{\titletilt}{ Support } \\\midrule
and32 & BW    & 1.9  & 32 & -- & 2.6 & 32 & -- & -- & -- & 35 & 17 & -- & $\times$ \\
or32  & BW    & 1.7  & 32 & -- & 2.6 & 32 & -- & -- & -- & 31 & 17 & -- & $\times$ \\
xor32 & BW    & 2.2  & 32 & -- & 2.5 & 32 & -- & -- & -- & 33 & 17 & -- & $\times$ \\
% not32 & BW    & 1.7  & 32 & -- & 2.6 & -- & -- & -- & 32 & 33 & 17 & -- & $\times$ \\
% mux32 & BW    & 12.7 & 32 & -- & 2.8 & 32 & -- & -- & -- & 22 & 32 & -- & $\times$ \\
add32 & Carry & 2.3  & 32 & 4  & 2.7 & 32 & -- & 8 & --  & 34 & 32 & 4 & $\times$ \\
sub32 & Carry & 1.9  & 32 & 4 & 2.7 & 32 & -- & 8 & -- & 34 & 32 & 4 & $\times$ \\
eq32  & Comp  & 3.3  & 32 & 4 & 2.6 & 24 & 1 & -- & -- & 36 & 11 & 2 & $\times$ \\
ugt32 & Comp  & 3.4  & 32 & 4 & 2.7 & 22 & -- & 3 & -- & 32 & 16 & 2 &$\times$ \\
ult32 & Comp  & 3.7  & 32 & 4 & 2.7 & 22 & -- & 3 & -- & 34 & 16 & 2 &$\times$

==> generated/xilinx-compressed.tex <==
\rotatebox{\titletilt}{ Instr } & \rotatebox{\titletilt}{ Template } & \rotatebox{\titletilt}{ Runtime in sec } & \rotatebox{\titletilt}{ \#LUTs } & \rotatebox{\titletilt}{ \#CARRY8s } & \rotatebox{\titletilt}{ DSP? (sec) } & \rotatebox{\titletilt}{ Runtime } & \rotatebox{\titletilt}{ \#LUTs } & \rotatebox{\titletilt}{ \#MUXs } & \rotatebox{\titletilt}{ \#CARRY4s } & \rotatebox{\titletilt}{ \#INVs } & \rotatebox{\titletilt}{ \#DSP } & \rotatebox{\titletilt}{ Runtime in sec } & \rotatebox{\titletilt}{ \#LUTs } & \rotatebox{\titletilt}{ \#CARRY8s } & \rotatebox{\titletilt}{ \#DSP } & \rotatebox{\titletilt}{ Support } \\\midrule
and16 & BW    & 1.6  & 16 & -- & \checkmark (4.8) & 2.6 & 16 & -- & -- & -- &--   & 36 & 10 & -- &--   & $\times$ \\
and32 & BW    & 1.9  & 32 & -- &                  & 2.6 & 32 & -- & -- & -- &--   & 35 & 17 & -- &--   & $\times$ \\
or16  & BW    & 1.8  & 16 & -- & \checkmark (7.1) & 2.6 & 16 & -- & -- & -- &--   & 34 & 10 & -- &--   & $\times$ \\
or32  & BW    & 1.7  & 32 & -- &                  & 2.6 & 32 & -- & -- & -- &--   & 31 & 17 & -- &--   & $\times$ \\
xor16 & BW    & 1.9  & 16 & -- & \checkmark (4.4) & 2.7 & 16 & -- & -- & -- &--   & 32 & 10 & -- &--   & $\times$ \\
xor32 & BW    & 2.2  & 32 & -- &                  & 2.5 & 32 & -- & -- & -- &--   & 33 & 17 & -- &--   & $\times$ \\
not16 & BW    & 1.8  & 16 & -- & \checkmark (3.6) & 2.6 & -- & -- & -- & 16 &--   & 32 & 10 & -- &--   & $\times$ \\
not32 & BW    & 1.7  & 32 & -- &                  & 2.6 & -- & -- & -- & 32 &--   & 33 & 17 & -- &--   & $\times$ \\
mux16 & BW    & 8.5  & 16 & -- & \checkmark (6.3) & 2.6 & 16 & -- & -- & -- &--   & 31 & 16 & -- & -- & $\times$ \\
mux32 & BW    & 12.7 & 32 & -- &                  & 2.8 & 32 & -- & -- & -- &--   & 22 & 32 & -- & -- & $\times$ \\
add16 & Carry & 2.3  & 16 & 2 & \checkmark (4.8) & 2.8 & 16 & -- & 4 & -- &  -- & 34 & 16 & 2 & -- & $\times$ \\
add32 & Carry & 2.3  & 32 & 4 &                  & 2.7 & 32 & -- & 8 & -- &  -- & 34 & 32 & 4 & -- & $\times$ \\
sub16 & Carry & 1.9  & 16 & 2 & \checkmark (3.9) & 2.7 & 16 & -- & 4 & -- &  -- & 34 & 16 & 2 & -- & $\times$ \\
sub32 & Carry & 1.9  & 32 & 4 &                  & 2.7 & 32 & -- & 8 & -- &  -- & 34 & 32 & 4 & -- & $\times$ \\
mul16 & --   & 2.4  & -- & -- & \checkmark (2.4) & 3.4 & -- & -- & -- & -- & 1 & 32 & -- & -- & 1  & $\times$ \\
mul32 & --    & --   & -- & -- &                  & 3.6 & -- & -- & -- & -- & 3  & 22 & -- & -- & 3  & $\times$ \\
eq32  & Comp  & 3.3  & 32 & 4 &                   & 2.6 & 24 & 1 & -- & -- &  -- & 36 & 11 & 2 &--    & $\times$ \\
neq32 & Comp  & 3.5  & 32 & 4 &                   & 2.7 & 24 & 1 & -- & -- &  -- & 33 & 11 & 2 &--    & $\times$ \\
ugt32 & Comp  & 3.4  & 32 & 4 &                   & 2.7 & 22 & -- & 3 & -- &  -- & 32 & 16 & 2 &--    & $\times$ \\
ult32 & Comp  & 3.7  & 32 & 4 &                   & 2.7 & 22 & -- & 3 & -- &  -- & 34 & 16 & 2 &--   & $\times$ \\
uge32 & Comp  & 2.8  & 32 & 4 &                   & 2.8 & 22 & -- & 3 & -- &  -- & 33 & 16 & 2 &--   & $\times$ \\
ule32 & Comp  & 2.5  & 32 & 4 &                   & 2.8 & 22 & -- & 3 & -- &  -- & 32 & 16 & 2 &--  & $\times$

==> poster/incubator.tex <==
\section{New Overview}
\label{sec:overview}
\hl{Pick an example}

\hl{explain what it does and why you should care about it}

\hl{Show how existing tools don't handle the example (to the best of our knowledge)}

\hl{Step through how Lakeroad handles the example.}

\hl{The rest of this paper details how Lakeroad generalizes all of these steps.}

\hl{At the end of overview: make the point that, you can use the same sketch for different workloads, and you can use the same sketch for workloads on different architectures.}

% Now, we will describe
%   the state of the art
%   synthesis tool for Xilinx FPGAs
%   compiles \texttt{((a+b)*c)\&d} onto
%   a Xilinx FPGA.

How does a user map a design to a DSP?
Let's consider the Xilinx DSP48E2,
  which implements any expression (design) of the form
  $((a \pm b) * c) \odot d$,
  where $\odot \in \{\land, \lor, \!\, \pm, \oplus \}$.
If a user wants to map the design
  \hl{include bitwidth and pipeline stages}
  $((a+b)*c) \:\&\: d$ to their DSP,
  ideally,
  they write the high-level behavioral Verilog
  shown in Figure~\cref{somefigure}.
\hl{figure to show the ``simple'' behavioral verilog}
  and pass that Verilog
  to an FPGA hardware synthesis tool.
Unfortunately,
  the state-of-the-art hardware synthesis tool
  for Xilinx FPGAs
  will fail to map the above design
  to a single DSP.
Furthermore, note that we include an annotation \texttt{(*USE\_DSP="yes"*)}
  in the behavioral Verilog,
  which instructs the tool
  to map the module to a DSP%
  ---despite this explicit hint,
  the tool still fails!

Currently, mapping this workload
  onto the DSP48E2
  would require a user to instantiate it by hand, 
  using code like that shown in Figure~\hl{N}.
In contrast, \lr can automatically map
  such computations to DSPs.
  
\hl{a figure: the full DSP instantiation that they need to write}


\subsection{Lakeroad Workflow}

The \lr workflow is shown in \cref{fig:lakeroad-diagram}.


1: Template. 
In the first step of the workflow,
   \lr generates a \textit{sketch}, i.e.,
   a partially implemented hardware design
   with holes to be filled by a solver.
   The main input to this step is a
   \textit{sketch template} which
   captures the high-level structure
   of the design without specifying
   low-level details. Rather than
   specifying the concrete computations that a
   design will perform, these templates
   describe how an FPGA program should wire
   together abstract computational components called
   \textit{primitive interfaces}.
   Figure N shows the template
   for DSPs, which is simply a primitive
   interface for a generic DSP with two
   inputs and an output. Note that the DSP's
   primitive interface does not include
   any information about the internal
   ports/parameters, as those are
   architecture-specific.
   
In the sketch generation step, 
  \lr specializes the architecture-independent
  template to an architecture-specific sketch
  using the architecture description
  as shown in Figure Nb for
  the Xilinx DSP48E2. Figure Nc
  shows the specialized sketch for the
  original design. Observe that this sketch,
  like the initial template,
  represents the shape of an FPGA
  program rather than the program itself;
  although the sketch captures a DSP48E2 instead
  of a generic DSP, the ports/parameters that
  implement the design remain unconfigured.

2: Semantics. 
How does \lr know that the design
  can be implemented with the
  generated sketch?
  Program synthesis is the key technique
  used to generate a hardware design, but a
  necessary input to this step is the semantics
  of the hardware primitives that will be
  instantiated in the final design.
  Traditionally, this has been a hurdle
  discouraging the use of program synthesis
  in technology mappers. However,
  \lr leverages a semantics importer
  to automatically extract semantics from
  vendor-provided Verilog models. This
  gives a precise mathematical definition
  of each hardware primitive.
  

3: synthesis.
\lr queries Rosette to determine
  whether there is a setting of variables
  in the template
  to implement the desired workload.

{\Large OLD OVERVIEW}
%\section{Overview}
%\label{sec:overview}

\begin{figure}
    \centering
    \includegraphics[width=.8\columnwidth]{assets/lakeroad-diagram.drawio.png}
    \caption{\lr system diagram. \hl{instr. spec should be removed, remove design fragment?}}
    \label{fig:lakeroad-diagram}
\end{figure}
  
\cref{fig:lakeroad-diagram}
  illustrates \lr's high-level design.
In this section we discuss the design components,
  and we illustrate \lr's flow with
  an example mapping a MAC (multiply accumulate) onto
  a Xilinx Ultrascale+ DSP48E2.
\hl{change running example to something that doesn't work on Vivado}
  
\lr takes three inputs:
  (1) an \textit{HDL module} specifying
    the FPGA program 
    to be implemented
    for a given architecture,
  (2) an \textit{architecture description} YAML file
    that describes the ports and parameters
    of an architecture's 
    hardware primitives,
  and (3) \textit{vendor-provided Verilog models}
    for the target FPGA architecture.
\hl{Which are user provided?}
\hl{the three inputs come from three different places: hdl model written by user, arch description written by...lakeroad maintainers? and vendor-supplied verilog. This might need a separate sentence.}
% The HDL module is the design which the low-level
%   Verilog will implement.
% The architecture description is a short configuration file
%   describing the ports/parameters of architecture-specific
%   hardware primitives.
% Lastly, the vendor-provided
%   Verilog models correspond to the implementations of
%   architecture-specific primitives
%   (e.g., \texttt{DSP48E2.v} on Xilinx).

These inputs are passed to the \lr pipeline,
  which is responsible for mapping the high-level
  HDL module to an architecture-specific
  implementation.
\cref{fig:firstpage} gives an example
  of \lr's inputs for
  implementing a MAC on a Xilinx
  Ultrascale+ DSP48E2,
  and the resulting
  output.
  
The \lr pipeline consists of
  three main components:
  \textit{sketch generation},
  \textit{program synthesis},
  and \textit{HDL compilation},
  which
  we now describe 
  in greater detail.
 % Together with automated semantics extraction
 %  from vendor-supplied Verilog models of
 %  target FPGA primitives, or manual effort from the user.
  
% \lr takes as input
%   (1) a high-level specification of an instruction,
%   (2) a description of a target FPGA architecture, and
%   (3) vendor-provided Verilog
%   models of the target FPGA's combinational primitives.
% Given these inputs,
%   \lr automatically generates
%   an implementation of the instruction
%   in low-level, architecture-specific
%   Verilog.


\subsection{Sketch Generation}

\lr uses the HDL module and
  the architecture description
  to perform
  \textit{sketch generation}.
Sketch generation
  specializes architecture-independent
  representations of FPGA programs, called
  \textit{sketch templates},
  into architecture-dependent
  \textit{program sketches}.

A \textit{sketch template} specifies
  the \textit{structure}
  of an
  FPGA program
  without specifying
  low-level details;
  rather than describing the concrete
  computations that an FPGA will
  perform, a sketch template describes
  how a program should wire together
  abstract computational components
  called \textit{primitive interfaces}.
In particular,
  sketch templates do \textit{not} specify
  the configurations of programmable
  primitives like LUTs or DSPs. 
Sketch templates also permit 
  some flexibility in wire routing,
  allowing for different common
  wiring patterns
  (e.g., reversing)
  to be explored
  during program synthesis.
\lr
  includes a series of default
  sketch templates,
  but a user can easily add their own if needed.

\hl{Would it be useful to draw parallels 
  between sketches and things similar to sketches
  in existing tools? E.g. Yosys essentially
  has sketches as the right-hand sides of its
  rewrites.}
To synthesize a MAC operation onto a DSP48E2,
  the \texttt{dsp} sketch template would be employed.
  This sketch template is quite simple, and consists of the
  primitive interface of a generic DSP with two inputs and an output.
  The DSP primitive interface does not include any information
  about the internal ports/parameters, as those are architecture-specific.
  
% \lr provides a default set of
%   sketch templates,
%   but a user may
%   define their own
%   if needed.

% In the case of synthesizing a MAC operation,
%   the sketch template would consist of an
%   architecture-agnostic representation of a DSP.
%   The sketch generation process would specialize
%   this template to a representation of a Xilinx-specific
%   DSP.
% \hl{mention how the architecture
%   description gets used here}

Although the \texttt{dsp} sketch template is simple, sketch templates can
  also represent more complex structures of primitives.
  For example, the Bitwise Sketch Template
  captures the structure of
  bitwise operations such as
  bitwise \texttt{\&}
  or bitwise \texttt{|}.
This template takes
  $k$ $n$-bit
  inputs,
  routes the $i$th bit of
  each input
  to a primitive interface
  representing an
  abstract $k$-input LUT,
  and routes the outputs
  of the $i$th LUT primitive
  interface to the $i$th output
  bit. 
  
% Using the provided architecture description,
%   \lr specializes these sketch templates
%   for specific architectures by
%   systematically expanding the abstraction
%   in terms of available primitives,
%   e.g., using a sequence of 4-bit LUTs
%   to concretely implement an abstract 6-bit LUT.
  
% Using sketch templates enables \lr
%   to abstract over common implementation strategies,
%   and thus reuse them across different FPGA architectures,
%   and reduces the input required from the user.
% Sketch templates specialized to an FPGA also serve as the
%   ``sketches'' that Lakeroad leverages during
%   sketch-guided synthesis to fill in.
% Sketches specify the overall structure of
%   a potential low-level implementation,
%   but leave unspecified ``holes'' for
%   LUT, DSP, and carry chain configuration
%   parameters which are then synthesized by
%   a reduction to a sequence of SMT solver queries~\cite{torlak2013growing}.

%\paragraph{(Example) 4-Bit Adder:}
  

% {\it (Example) 4-Bit Adder:}
%   For a more complicated example,
%   consider building a 4-bit binary adder
%   that adds 4-bit bitvectors \texttt{a} and \texttt{b}.
  
% On Xilinx's Ultrascale+ this would
%   be built with four LUT2s,
%   each with configuration
%   \texttt{.INIT(4'h6)} to compute
%   the sum bits,
%   and a CARRY8.
% The outputs of the LUT2s would
%   be wired into the CARRY8's \texttt{.S} ports,
%   and \texttt{a} would
%   be wired into the \texttt{.DI} ports
%   of the CARRY8 to allow carry bit
%   generation.
% On Lattice ECP5 this could be built
%   by connecting 4 CCU2C components
%   into an 8-bit carry chain and connecting
%   8 LUT4s with configuration \hl{specify config}
%   into the carry chain's input.

% On SOFA, which only has LUT4s and does not
%   have a fixed carry-chain unit,
%   the sum bits would be computed with
%   four frac\_lut4s (SOFA's LUT4 primitive) with
%   configuration \texttt{.sram(16'hf77f)}.
%   The outputs of these LUTs as well
%   as one of the inputs (e.g., \texttt{a})
%   would be passed into a complicated
%   carry-chain structure
%   built from frac\_lut4s.
  
% Details differ between architectures but
%   both programs share a common shape:
%   both have four LUTs feeding into a
%   carry chain structure.
% A sketch template captures this
%   similarity by specifying that it wants four LUTs fed
%   into a carry chain.
% It does \textit{not} detail 
%   which FPGA components will be used, or
%   what their configurations will be.\hfill $\qed$

% \hl{is this qed intentional?}

Sketch generation then
  specializes
  sketch templates
  to partially complete
  architecture-specific
  FPGA programs called
  \textit{program sketches}. A program sketch
  contains \textit{holes};
these holes allow flexibility
  in potential program implementations
  and will be filled in later by the Program
  Synthesis component.

% This is repetitive?
A program sketch, like a sketch template, still
  represents the \textit{shape} of an FPGA program
  rather than the program itself:
  while it is now FPGA-specific,
  many of the computational
  components in a program
  sketch are unconfigured,
  and retains the
  same flexibility
  in wire routing
  choices that
  existed in the
  sketch template.
  
With a Xilinx architecture description, sketch
  generation would convert the DSP primitive interface
  to a partially complete representation of the DSP48E2.
  The ports and parameters at this point would be included
  in the representation, but their configuration would
  remain symbolic and need to be solved during Program
  Synthesis.
  
% \lr's templates capture common 
%   implementation patterns
%   used in FPGAs.
% For example,
%   to implement multiple-bit
%   logic operations
%   like 
%   \texttt{a \&\& b}
%   on most FPGAs,
%   the common strategy is to use
%   a one Look-up Table (LUT)
%   per pair of bits,
%   e.g.~\texttt{LUT(a[0], b[0])},
%   \texttt{LUT(a[1], b[1])},
%   and so on.
% Arithmetic operations
%   are implemented similarly,
%   but with an arithmetic carry chain
%   to carry information between bits.
% \lr's templates
%   capture these high-level patterns
%   in an architecture-independent way.

% \lr's templates rely on \textit{primitive interfaces}
%   that represent computations in
%   an architecture-independent way.
% For instance, the LUT-$n$ primitive
%   interface represents
%   an $n$-input 1-output lookup table,
%   and the Carry-$n$ represents an $n$-bit
%   carry chain.
% Architecture descriptions provide implementations
%   for primitive interfaces.
% These implementations may be done with a
%   single hardware primitive
%   or with a combination of hardware
%   primitives.
% \lr also provides logic to perform common
%   primitive combinations, such as
%   recursively building
%   a larger LUT from smaller LUTs.
  

% \textit{Sketch generation}
%   transforms a template to
%   a \textit{sketch}.
% A sketch is a \lrir program with
%   \textit{holes}, or symbolic values
%   that will be later filled in by
%   synthesis to make a concrete \lrir program.
% Sketch generation 
%   queries an
%   \textit{architecture configuration}
%   to find architecture-specific
%   implementations for a
%   template's primitive interfaces.
% These implementations may still be
%   symbolic (that is, they may have holes).

\subsection{Program Synthesis}
\lr uses \textit{sketch-guided program synthesis}~\cite{??}
  to find a low-level, architecture-specific
  FPGA implementation.
Sketch-guided program synthesis is a
  technique that uses a solver
  to look for values to fill in
  a sketch's holes so that it
  implements the specified instruction. For a MAC,
  the end result of program synthesis would be a
  correct configuration of the ports/parameters of
  the DSP48E2 that would implement the operation.

Sketch-guided program synthesis
  requires an interpreter to define
  the semantics of the language that
  the sketch is written in, and
  this usually requires up-front
  investment from
  the user.
This is often a barrier to
  entry and is not an option
  for our use-case.
To avoid this problem, \lr
  \textit{automatically constructs}
  an interpreter by
  (i) providing a base interpreter
  that specifies all
  FPGA-independent semantics
  (e.g., wiring operations, etc),
  and
  (ii) \textit{automatically importing}
  the semantics of FPGA-specific primitives
  from vendor-supplied Verilog models;
A user only
  needs to provide
  a high-level
  description of 
  the target FPGA
  architecture rather
  than explicitly
  writing the interpreter.


This final program will be in \lrir,
  \lr's domain-specific synthesis language.
Both sketch templates and program sketches
  are partial \lrir programs.
  
\subsection{HDL Compilation} 

After program synthesis,
  the \lrir program has filled in all holes
  corresponding to programmable primitive configuration and thus represents a complete low-level design.
Finally, the \lrir program
  is compiled to a HDL that can
  be placed on the physical FPGA.
This compilation is purely syntactic:
  it does no optimization and simply
  maps from one structure to another.
This translation is a simple
  one-to-one correspondence to
  help ensure the correctness
  of the \lrir implementation
  and the compiled HDL program.
For a MAC, this would be a conversion from \lrir to
  the corresponding low-level Verilog.

%\section{\ThePlatonicApproach{} (old)}
%\label{sec:overview}
%
%In this section we introduce \textit{\theplatonicapproach{}}, a novel approach for
%automatically implementing ISA instructions for a target FPGA architecture from
%formal models of the ISA instructions and of  the target architecture.
%%
%\note{Note: I want \theplatonicapproach to include the DSL...THIS IS PART OF THE TECHNIQUE! How do we phrase this?}
%Central to \ThePlatonicApproach is a \textit{customizable} and \textit{extensible} domain specific language (DSL).
%%
%Here is an outline of \theplatonicapproach:
%\begin{itemize}
%    \item A user encodes formal models of each target ISA instruction in the DSL
%    \item The user models \textit{primitives} for the target FPGA architecture by extending the DSL
%    \item \note{are users providing templates/search spaces for the program we are synthesizing? should we be explicit here?}
%    \item \Theplatonicapproach invokes an SMT solver to find a program in the DSL that
%          implements the encoded ISA instruction for the FPGA architecture
%\end{itemize}
%\note{\ldots just a solver? why \textit{constrain}  ourselves (yuk yuk yuk) to SMT solvers?}
%
%\hl{
%System diagram
%
%non-eval contributions explained at a high level
%
%when you finish the overview, you should have an idea of the blocks within lakeroad, but you shouldn't know how they're implemented.
%
%want to mention that it's solver aided
%
%
%what do we care about/what do we want people to continue caring about for the next n years
%
%we want people to care that this is solver-aided
%
%we want people to care that it is user-extensible, to easily support new architectures
%}
%
%\hl{put synthesis statement in overview:}
%FIND \textit{init}\ .\ $\forall a,b,c,d$\ .\  lut(a,b,c,d, \textit{init}) == bvand(a, b)

==> poster/table.tex <==
\begin{table}[]
\caption{Synthesis time and resource usage when synthesizing various expressions for Xilinx UltraScale+ using our \texttt{\lowercaselr} command and using the existing \texttt{synth\_xilinx} command in Yosys.}
\label{tab:yosys-xilinx}
\hl{Replace this figure with more expansive DSP tables}
\setlength{\tabcolsep}{2pt}
\centering
\begin{tabular}{l|ll|ll}
\hline
instruction                      & \multicolumn{2}{l|}{\texttt{\lowercaselr}} & \multicolumn{2}{l}{\texttt{synth\_xilinx}} \\
(all 16 bit)                     & time (s)           & DSP          & time (s)  & Prim \\ \hline
$a\times b$                      & 2.49               & 1            & 4.03      & 1   \\
$((a+b) \times c)+d$             & 2.44               & 1            & 4.18      & 41    \\
$(a\times b) + c$                & 3.02               & 1            & 4.02      & 21  \\
$(a+b)\times c$                  & 1.75               & 1            & 3.83      & 21 \\
$(a+b)^2$                        & 1.84               & 1            & 3.83      & 21 \\
$(a-b)^2$                        & 2.29               & 1            & 3.82      & 21 \\
$(a-b)^2 - c$                    & 21.7               & 1            & 3.93      & 41 \\
$(a+b)^2 +c$                     & 2.17               & 1            & 3.92      & 41 \\
$((a+b)\times c) \oplus d$       & 1.87               & 1            & 3.92      & 37 \\
$\sim(((a+b)\times c) \oplus d)$ & 2.43               & 1            & 4.01      & 37    
\end{tabular}
\end{table}

==> text/completeness-motivation.tex <==
% Gus integrated this content into the intro.

% \section{Motivation: Techmapping Completeness}
% \label{sec:completeness}

% In this section,
%   we empirically motivate
%   the need for 
%   \lr.
% We first give a formal definition
%   for 

% \hl{
% I'm split on whether
%   we should introduce completeness
%   up front in its own section,
%   or split it up into existing sections.
% Specifically,
%   we have two components to be introduced:
%   the formal completeness defintion
%   and the empirical incompleteness evidence
%   of other tools

  
% }



\section{Motivation: Limitations of Current Approaches}
\label{sec:completeness}

Hand-written syntactic matching
  has several key limitations 
  when applied to programmable primitives.
\paragraph{Limitation 1: Mapping Completeness}
We refer to completeness as 
  a tool's ability to map a design
  to a primitive, if such a mapping exists.
Completeness is challenging
  to guarantee for programmable primitives,
  as there may be many designs that can
  map to a primitive---far too many to 
  capture via handwritten patterns.
This rigidity \hl{don't think this is the word} 
  is further exacerbated by the fact that a high-level operation can be represented with 
  several equivalent designs, meaning that each representation of a design would require
  a pattern.
As shown in \hl{andrew teaser table},
  even canonical representations of small workloads are not mapped 
  correctly \hl{finish off this sentence strongly}.

\paragraph{Limitation 2: Correctness Guarantees}
Handwritten patterns also do not provide formal
  correctness guarantees; a rewrite can
  match any pattern in the design, and 
  replace it with anything else.
Perhaps unsurprisingly, as a result, a
  significant number of bugs have been found
  across all major hardware synthesis tools \hl{sneak peek table?}
\hl{sentence about "if only formal semantics existed maybe? might be a bit tacky}
\paragraph{Limitation 3: Extensibility}
Even if a handful of patterns can be
  derived and implemented for a new primitive,
  adding full support requires writing patterns 
  to cover \textit{all possible ways} the primitive can be used, a daunting task.
This process then must be \textit{repeated}
  each time a new primitive needs to be supported.


==> text/formalization-old-0.tex <==
\section{Formalization}
\label{sec:formalization}

% SpecIR example:
% (bvand a b) (a and b are (bitvector 8))
% LRIR:
% (hash-ref
%  (hw-module-instance 
%   "LUT2"
%   memory = 4'b1000,
%   i0 = a,
%   i1 = b)
%  'O)

% (rosette-synthesize SpecIR-program LRIR-program)
% -> assert SpecIR-program == LRIR-program
% -> solve

% I_S : SpecIR -> bitvector
%  --> "just" Rosette/Racket. (bvand a b) evals automatically.
%  we don't have to do (interpret (bvand a b))
% I_LR : LRIR -> bitvector
%  (lr:hash-ref ...)
%  (interpret (lr:hash-ref ...))

% exists M, 
%  forall inputs, I_S(P_S, inputs, M) 
%                   == I_LR(P_LR, inputs, M).
% synthesis: find M

% in the past/in the current version of the paper:
% I_S and I_LR -> bitvectors
%
% New thing:
% I_S and I_LR -> signals

% This will change the synthesis problem
% Old problem:
% exists M, 
%  forall inputs, I_S(P_S, inputs, M) 
%                   == I_LR(P_LR, inputs, M).
% synthesis: find M

% now we have multiple possible synthesis problems
% exists M, 
%  forall inputs, (signal-value I_S(P_S, inputs, M))
%                   == (signal-value I_LR(P_LR, 
%                                     inputs, M)).
% synthesis: find M

% exists M, 
%  forall inputs, 
%   (let o0 = I_S(P_S, inputs + clk=0, M);
%    let o1 = I_S(P_S, inputs + clk=1 + state(o0), M);
%    let o2 = I_S(P_S, inputs + clk=0 + state(o1), M);
%    ...
%    (signal-value oN))
%   == 
%   (let o0 = I_LR(P_LR, inputs + clk=0, M);
%    let o1 = I_LR(P_LR, inputs + clk=1 + state(o0), M);
%    let o2 = I_LR(P_LR, inputs + clk=0 + state(o1), M);
%    ...
%    (signal-value oN))
% synthesis: find M

In this section, we formalize \lr
  and provide a mathematical argument
  for its correctness.
We start by introducing and 
  formalizing the semantics used in \lr,
  beginning with introducing
  its base value type:
  the \signal datatype (\cref{sec:signal}).
Then, we define syntax and semantics
  of the imported Verilog (\cref{sec:verilog-semantics})
  and of the \lr IR, \lrir (\cref{subsec:spec-ir-and-lrir}).
Finally, we present
  a mathematical model
  of the \lr workflow
  (formalized via the \lrfn function)
  and prove its correctness
  (assuming the correctness of the underlying program synthesis tool and HDL compiler) in \cref{sec:correctness-argument}.
%Then we introduce the \lrfn function
  %to formalize the \lr workflow
  %introduced in \cref{sec:overview}
  %and argue for its correctness
  %via stating the \lr-Correct property
  %(\cref{sec:correctness-argument}).

  
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
% Subsection: Signals
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
\subsection{The \texttt{signal} Datatype}
\label{sec:signal}

To formalize
  expressions
  in both the
  imported Verilog 
  and \lrir,
  we first introduce their base value type:
  the \signal datatype.
\signal{}s are fundamental to \lr's ability
  to synthesize sequential designs.
While bitvectors alone are expressive enough
  to capture the semantics of 
  \textit{combinational} expressions,
  they are not expressive enough to capture
  \textit{sequential} expressions.
Thus, we introduce \signal{}s
  as a more expressive datatype
  for capturing hardware expressions.
  
A \signal represents
  the value on an $n$-bit
  wire and
  the current state
  of the stateful elements
  in the context where the \signal
  was produced.
Consequently, we represent a
  \signal{} as a pair $(v,m)$,
  where $v$ is a bitvector
  capturing the value on the wire
  and $m$ is a map
  capturing the current state.

% \input{figures/state-merge-and-update}
\input{figures/signal-state}
The state map $m$
  maps keys (which uniquely identify
    an expression's internal state elements)
  to a tuple $(\mathit{sv}, \mathit{vers})$,
  where $\mathit{sv}$
  is the value of the state
  and $\mathit{vers}$ is
  its version number 
  (necessary for handling conflicts during merging).
Beyond indexing into a state map,
  we define two core operations of state maps:
  \textit{merging} and \textit{updating,}
  both defined via pseudocode
  in \cref{fig:signal-complete}.
Merging two state maps
  simply unions the two maps together,
  while handling conflicts by taking the value
  with the highest version number.
Updating a state map
  involves setting a key to a value
  while incrementing the version (or defaulting to 0).
  
  
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
% Subsection: Verilog Semantics
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
\subsection{Imported Verilog Semantics}
\label{sec:verilog-semantics}

\input{figures/verilog-syntax}

\input{figures/yosys-semantics}

\lr extracts semantics from Verilog,
  both from the user-provided Verilog file
  to be compiled,
  and the vendor-supplied FPGA primtive
  simulation models.
The process for extracting these semantics
  is described in detail in
  \cref{sec:implementation:importing-semantics}.
In this section, we formalize 
  the semantics
  which result from this extraction process.
While this formalization
  is a contribution of this paper,
  the underlying semantics
  of the subset of Verilog
  \lr supports
  are designed and implemented by
  the Yosys synthesis tool~\cite{wolf2013yosys}.

\cref{fig:verilog-syntax}
  lists the syntax for the subset of Verilog 
  supported for import by \lr,
  while \cref{fig:verilog-semantics}
  defines its semantics.
Imported Verilog expressions evaluate to \signal{}s.
In general, the imported Verilog expressions
  cover a wide swath
  of bitvector operations,
  including bitwise operations,
  arithmetic operations,
  comparisons,
  and muxes.

\texttt{dff} represents
  a D flip-flop: a state element
  with a clock and data input,
  which stores the value on the data input
  when the clock changes from low to high.
The semantics for this expression
  are given by \textbf{dff-hold}
  and \textbf{dff-tick}.
\textbf{dff-hold}
  describes 
  the case when the clock doesn't tick,
  i.e., there's no \textit{positive edge}
  going from 0 to 1.
In this case,
  the flip flop expression holds
  its previous value $q'$,
  which it gets from the state map.
\textbf{dff-tick}
  describes the case in which
  the clock ticks,
  and thus the expression
  takes on the new value $d'$.
Note, crucially,
  that the value becomes $d'$
  (the \textit{previous} value of $d$,
  read from the state map)
  and not the current value of $d$.\footnote{
  These semantics are defined by
  Yosys's \texttt{clk2fflogic} pass.
}


The \texttt{dff} expression is the 
  only expression
  in both Verilog and \lrir semantics
  that updates the state map.
All other expressions
  are \textit{combinational},
  meaning they do
  not alter state.
% This is significant as it allows us
%   to simplify our mental model of 
%   imported Verilog and \lrir semantics.
% Knowing that \texttt{dff} is the only
%   expression to update the state map,
%   we can interpret
%   all other expressions
%   in the imported Verilog
%   and \lrir
%   as being purely combinational.
% (Note that expressions generally \textit{merge}
%   state maps, seen in most rules in 
%   \cref{fig:verilog-semantics,fig:lrir-semantics},
%   but crucially, only \texttt{dff} \textit{updates}
%   values in the map).
  


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
% Subsection: Spec IR and LRIR
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
\subsection{\lrir}
\label{subsec:spec-ir-and-lrir}

% \lr defines two Intermediate Representations (IRs),
%   \Spec IR and \lrir;
%   syntax for both is defined
%   in \cref{fig:lakeroad-dsl-grammar}.
% \lr uses \Spec IR
%   to give specifications for
%   instructions to synthesize.
% Terms in \Spec IR are either
%   bitvector constants,
%   variables which represent
%   inputs to the instruction,
%   or operators
%   applied to smaller terms.
% \Spec IR is a subset of the SMT-LIB language~\cite{smtlib},
%   from which it derives its semantics.

\input{figures/lakeroad-dsl-grammar}

\input{figures/lakeroad-dsl-semantics}

\lr uses the \lr Intermediate Representation (\lrir) to represent
  wire operations and computations on FPGAs.
The syntax for \lrir is shown in
  \cref{fig:lakeroad-dsl-grammar},
  while its semantics are in \cref{fig:lrir-semantics}.
In general, the \lrir syntax and semantics 
  are straightforward.
\lrir expressions evaluate to \signal{}s or
  lists of \signal{}s.
Fundamental operations over lists
  (construction, 
  indexing via \texttt{list-ref})
  and \signal{}s
  (\texttt{concat}, \texttt{extract}) 
  are supported.

The only \lrir expression
  which can perform actual computation
  or manipulate state
  (beyond the state merging in \texttt{concat})
  is \texttt{prim}.
\texttt{prim}
  represent instances
  of \textit{hardware primitives} (e.g., LUTs and DSPs).
A \texttt{prim} has a \textit{name}
  (e.g., ``LUT4''), a \textit{configuration},
  and an \textit{input}.

The semantics of a \texttt{prim} expression
  are the semantics extracted from the
  primitive's vendor-supplied Verilog model,
  as introduced in the previous section.
Evaluating \texttt{prim} expressions
  ``drops through'' to these imported
  semantics.
\lrir stores these semantics in
  a context 
  \[\Gamma: \left(\forall p: \textsc{Prim},
            \textsc{Config}\ p\right)
            \rightarrow [\texttt{signal}] 
            \rightarrow [\texttt{signal}]\]
  that takes a configuration
  for a primitive $p$
  and returns a function from
  \texttt{signal}s to \texttt{signal}s
  that captures the semantics
  of $p$ with that configuration.
A configuration of primitive $p$,
  \textsc{Config} $p$,
  is the list of parameters that
  an instantiation of $p$ expects
  (e.g., a Xilinx Ultrascale+ DSP48E2's
  \texttt{AREG}
  and \texttt{BREG}
  parameters, which configure pipelining).
  
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
% Subsection: Correctness of the LR Function
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
\subsection{Mathematical Model of \lr}
\label{sec:correctness-argument}

\newcommand{\SketchGenFn}{f_{\text{G}\xspace{}}}
\newcommand{\LRSynthFn}{f_{\text{S}\xspace{}}}
\newcommand{\HDLCompFn}{f_{\text{C}\xspace{}}}

Now that we have formalized
  \lr's fundamental components---%
  signals,
   imported Verilog semantics,
   and \lrir---%
  we now formalize the \lr workflow
  as a function \lrfn{}.
We define the function to be
the composition of two sub-functions, which we describe in the below sections:
% \[\lrfn: \Spec \times \Sketch \times \VendorSemantics \rightharpoonup \HDL.\]
$$\lrfn : \Spec \times \Sketch \times \VendorSemantics \times \textsc{Input} \rightharpoonup \HDL = \HDLCompFn \circ \LRSynthFn$$
where $\Spec$ represents hardware designs, $\Sketch$ represents program sketches, $\VendorSemantics$ represents vendor-provided semantics for FPGA components, and $\textsc{Input}$ represents partially symbolic inputs (discussed below).

\lrfn does not include sketch generation,
  instead taking the sketch as an input.
This is for the benefit of stating the correctness properties:
  There is no \textit{a priori} notion of the ``correctness'' of a sketch---%
  a sketch is ``correct'' 
  so long as program synthesis succeeds 
  in filling the holes in the sketch.
A sketch does, however, influence
  the search space for program synthesis, as we note in \hl{todo fill in forward reference}.
  
% This is because our correctness properties
%     state that any synthesized program is correct.
% If an incorrect sketch is generated then synthesis
%     will fail and the correctness
%     properties will hold vacuously.

% \hl{New user input needed: number of clock cycles, among other things?}

% \hl{should sems be gamma?}

%\hl{ben is pointing out that these functions don't actually compose in their current states b/c of their input/output types. we could do a few things: (1) change figure 2 so everything goes through sketch generator. (2) have the two differ but acknowledge the difference. or (3) go full formal and have the semantics "pass through"}

%\hl{see notes under figure. we can just drop fg, and mention that fg isn't necessary to correctness}

% %%%%%  Sketch Generation
%
% NOTE: I've removed this subsection, but we can include it
% later if we think we should. It's not part of the lr function
% so if we do include it, it should be put elsewhere!
%
% \subsubsection{\SketchGeneration}
% \lrfn begins by performing \SketchGeneration
%   on each available sketch 
%   template\footnote{While sketch
%   templates can in theory
%   be provided by users, the \lr tool supplies
%   a set of base templates and, for simplicity
%   of the formalization, we treat
%   them as being internal to the tool.}.
% We formalize \SketchGeneration with the function
% \hl{should also include the spec, b/c we need to know the input/output widths}
%   \[\SketchGenFn :\SketchTemplate \times \ArchDescr \rightharpoonup \Sketch,\]
%   where \(\rightharpoonup\)
%   indicates that this operation is partial.
% $\SketchGenFn$ is partial because a sketch template
%   may use a primitive interface that isn't supported
%   by a given architecture's description.
  
%%%%%  LRSynthesis
\subsubsection{\LRSynthesis: $\LRSynthFn$}
\label{sec:lr-synth-defs}
\lrfn begins by attempting to synthesize an \lrir{} program
  that implements a provided specification using
  a program sketch.
We formalize this component with 
  the $\LRSynthFn{}$ function:
  \[\LRSynthFn: \Sketch \times \Spec \times \VendorSemantics \times \textsc{Input} \rightharpoonup \lrir.\]
$\LRSynthFn$ is partial since
  synthesis may not find an
  implementation for a spec
  using the given sketch---%
  Rosette may conclude that no implementation exists
  or it may time out.
%\hl{Maybe add signal 
  %mention in this section 3.2.2.}
  
\newcommand{\lrinterp}[0]{\mathcal{I}_{Ax}}

We formalize synthesis
  in terms of an interpretation
  function 
  $\lrinterp$,
  which expects
  an \lrir program $p$,
  vendor-provided semantics $e$ 
  (used for interpreting the
  semantics of any \texttt{prim}
  constructs in $p$),
  a vector $\mathbf{i}$ of
  partially symbolic values,
  and a partially symbolic
  state map $m$
  as input values,
  and produces a partially
  symbolic signal as output.
A \textit{partially
  symbolic signal} is a pair $(v, m)$
  of a partially symbolic value $v$
  and a partially symbolic
  state map $m$.
A \textit{partially symbolic value} $v$
  is either a concrete bitvector
  or a symbolic bitvector.
A \textit{partially symbolic map} $m$
  is a map from concrete keys
  to partially symbolic values.
% For a symbolic bitvector $v$,
%   $f(v) = g(v)$ means that $\forall v^\prime, f(v^\prime) = g(v^\prime)$,
%   where $v^\prime$ is a concrete bitvector;
%   that is, we quantify 
%   over all possible instantiations 
%   of the symbolic values.

%\hl{we need to get $(v,m)$/$(v,s)$ consistent across the paper. $s=(v,m)$ is probably better. Needs to be propagated to first half of formalization. -gs}


We define $\lrinterp$ recursively:
\begin{align*}
    \lrinterp(p, e, [\mathbf{v_1}], m) &= \llbracket p \rrbracket (\mathbf{v_1}, m) \\
    \lrinterp(p, e, [\mathbf{v_1}, \mathbf{v_2}, \ldots, \mathbf{v_n}], m)  &= \lrinterp(p, e, \\
    & \hspace{15mm} [\mathbf{v_2}, \ldots, \mathbf{v_n}], \pi_S(\llbracket p \rrbracket (\mathbf{v_1}, m)))
    % a little nasty but it breaks margins otherwise
\end{align*}
% $$\lrinterp(p, e, [\mathbf{v_1}]) = \llbracket p \rrbracket (\mathbf{v_1})$$
% $$\lrinterp(p, e, [\mathbf{v_1}, \mathbf{v_2}, \ldots, \mathbf{v_n}]) = \lrinterp(p, e, [S_{\mathbf{v_1}}(\mathbf{v_2}), \ldots, S_{\mathbf{v_1}}(\mathbf{v_n})])$$
%\hl{i think we can make these prettier -- perhaps use aligned env?}
  where $\llbracket p \rrbracket(\textbf{v})$ evaluates $p$ 
  with respect to its semantics 
  (Figure~\ref{fig:lrir-semantics},
  substituting the elements of $\mathbf{v}$ for each \texttt{signal-var} in $p$), and $\pi_S$ projects
  the state map from a signal.
We similarly define $\mathcal{I}_V(d, \mathbf{i}, m)$,
  which behaves identically to $\lrinterp$,
  except that it takes as input a Verilog design $d$ 
  ($\llbracket d \rrbracket$
  evaluates the design
  according to the Verilog semantics
  in Figure~\ref{fig:verilog-semantics})
  and it does not use $e$,
  since there are no
  \texttt{prim} constructs in Verilog.

Given a hardware design $d \in \Spec$,
  vendor-provided semantics $e \in \VendorSemantics$,
  $s \in \Sketch$,
  and a input vector of partially symbolic values,
  $\LRSynthFn$ is defined as sending the following query to Rosette:
$$\exists p \in \lrir\ \text{s.t.}\ \lrinterp(p, e, \mathbf{i}) = \mathcal{I}_V(d, \mathbf{i}).$$
Synthesis succeeds if Rosette
  finds a program $p$ 
  (constructed by filling the holes in $s$)
  that satisfies this property.
How the input 
  $\mathbf{i}$
  is constructed 
  is an important design decision;
  we describe the specific decisions
  made by \lr
  in 
  \cref{sec:implementation:program-synthesis}.
(Note that our formalization has no need
  to ``privilege'' the clock---%
  it can be treated like any other signal.)

% [[d]]([t]) = [[d]]'(t)
% [[d]](s) = s
% Interp(e, i (vector)) each elem of i = tuple of signals
% Interp(e, [] ::' i) = [[e]](i)
% Interp(e, is ::' i) = let (_, s) = Interp(e, is) in
%   Interp(e, [i.update(s)]
% update: update((sig0, sig1, sig2), s) -> overwrites sig0, sig1, sig2 states with s
% vector i: list of concrete length
% element of vector i: tuple of concrete length
% element of that tuple: signal
% that signal: concrete or symbolic value, 
%   state map has concrete keys, concrete or symbolic values

% symbolic inputs are just variables, always bitvectors
% if Rosette succeeds, then it's quantified for all symbolic values


% The $\LRSynthFn{}$ takes
%   $(d, n) \in \Spec$ and attempts
%   to synthesize a program in \lrir
%   with the semantics of $d$.
% When $d$ is sequential, successful
%   synthesis yields a program that
%   implements $d$ after $n$ clock cycles.
% \hl{Ben: \@Gus I'll need you to give more detail on this}
% $\LRSynthFn{}$ does this by applying the
%   interpreter to the sketch multiple times
%   to simulate each cycle of the clock.
% We can treat a sketch $s$ as a function that
%   outputs values on the wire and 
%   updated state (e.g., incremented clock).
% Then Synthesis tries to find an instantiation
%   $S$ of $s$ such that $S^n(i)$
%   implements $d(i)$.
% \hl{I'm not saying the above correctly, we need
%   fix! But this is the basic idea}.
% Here we use the notation $S^n(i)$ to mean
%   the following:
%   \begin{itemize}
%       \item $S^1(i, \sigma_0)$ is defined to  be
%         the 2-tuple $(v, \sigma_1)$
%         of the output value $v$
%         and state $\sigma_1$
%         resulting from applying
%         $S$ to input $i$
%         with initial state $\sigma_0$.
%       \item $S^{n+1}(i, \sigma_0)$ is defined
%         to be the 2-tuple $(v, \sigma_{n+1})$ 
%         of the output value $v$ and the
%         state $\sigma_{n+1}$ resulting from
%         applying $S$ to input $0$ and state
%         $\sigma_n$.
%   \end{itemize}
%   \hl{Ben: This is not quite what we discussed, but I think it's correct for the formalism. We can go into the more detailed approach w/ multiple interpreter calls in implementation.

% I'm also happy to go into more detail here, but I want to start simple and see what this misses.}
  
% When $d$ is combinational,
%   successful synthesis yields a 
%   program that implements the
%   semantics of $d$ being run a
%   single time (no updated state or
%   clock cycles).


%%%%%  HDL Compilation
\subsubsection{\HDLCompilation}
Next, \lrfn compiles each synthesized design
  to an HDL. This is formalized with the function
  \[\HDLCompFn: \lrir \rightarrow \HDL.\]
This compilation is done as a very 
  straightforward syntactic mapping:
  each component
  of \lrir maps directly to the
  resulting Verilog implementation.

% \subsubsection{Combining Components into \lrfn}
%
% NOTE: We no longer need this section
%
% The \lrfn function is built by combining the three above components, as sketched in the following pseudocode:

% \lstset{style=pystyle}
% \begin{lstlisting}[basicstyle=\normalsize\ttfamily]
% def LR(spec, arch, sems):
%   hdl_impls = {}
%   for t in sketch_templates:
%     sketch = generate_sketch(t, arch)
%     lrir = synth_lrir(spec, sketch, sems)
%     if lrir is not None:
%         hdl_impls.add(compile2hdl(lrir))
%   return hdl_impls
% \end{lstlisting}
% \lstset{style=lispstyle}

  

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
% SubSection: Correctness of LRFN Function
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
\subsection{Properties of \lrfn{}}

From the above definitions,
  we can prove certain correctness properties
  about \lrfn{} and $\LRSynthFn$
  if we make certain assumptions about our some components of \lr (our trusted computing base):
\begin{enumerate}
\item \textbf{Rosette}: We assume that Rosette is correct (if it returns a program for a synthesis query, the program satisfies the specification) and sketch-complete modulo timeout (given a sketch, if there exists any solution using that sketch, Rosette will either find a solution or time out---it will not falsely conclude that no solution exists).
\item \textbf{Yosys}: We assume that Yosys's conversion of Verilog into bitvector expressions is correct.
\item \textbf{Vendor-supplied semantics}: We assume that these Verilog files correctly model the semantics of the FPGA components they model.\footnote{
  Note that this assumption may not always be true,
    as we will see in
    \cref{sec:completeness}.
}
\item \textbf{The implementation of $\lrinterp$}: In synthesis, we include an interpreter for the semantics of \lrir. We assume that our implementation correctly implements the claimed semantics in Figure~\ref{fig:lrir-semantics}.
\item $\mathbf{\HDLCompFn}$: We assume that our compilation from \lrir to Verilog is correct and complete. We do not prove this, though it could be done in principle via the semantics in Figures~\ref{fig:lrir-semantics} and~\ref{fig:verilog-semantics}; we rely instead on the simplicity of the implementation.
\end{enumerate}

\subsubsection{Correctness of Synthesis}

We can state this property as follows: 
If $\LRSynthFn(d, s, e, \mathbf{i}) = p$
  for design $d$, 
  sketch $s$,
  vendor-provided semantics $e$,
  and a partially symbolic input $\mathbf{i}$, 
  then for all inputs $\mathbf{i}^\prime$ 
  that are valid concrete instantiations of $\mathbf{i}$,
  $\mathcal{I}_V(d, \mathbf{i}^\prime) = \lrinterp(p, e, \mathbf{i}^\prime)$.
This follows directly from our assumptions about the correctness of Rosette and the correctness of Yosys (which is used to implement $\mathcal{I}_V$) and the definitions in \cref{sec:lr-synth-defs}.

\subsubsection{Sketch-Completeness of Synthesis Modulo Timeout}

Given design $d$,
  sketch $s$,
  vendor-provided semantics $e$,
  and a partially symbolic input $\mathbf{i}$,
  if there exists an instantiation of $s$ called $p$ for which $\mathcal{I}_V(d, \mathbf{i}^\prime) = \lrinterp(p, e, \mathbf{i}^\prime)$ 
  for all
  valid instantiations $\mathbf{i}^\prime$ of $\mathbf{i}$, 
  then $\LRSynthFn(d, s, e, \mathbf{i})$ 
  will either return some value or time out.
This follows from the sketch-completeness (modulo timeout) of Rosette.

\subsubsection{Correctness and Completeness of \lrfn{}}

Given the above properties of $\LRSynthFn$
  and our assumption of the correctness and completeness of $\HDLCompFn$,
  it follows that their composition will have analogous properties:
For design $d$,
  sketch $s$,
  vendor-provided semantics $e$,
  and a partially symbolic input $\mathbf{i}$,
  if $\lrfn(d, s, e, \mathbf{i}) = d^\prime$, then $\mathcal{I}_V(d, \mathbf{i}^\prime) = \mathcal{I}_V(d^\prime, \mathbf{i}^\prime)$ for all valid instantiations $\mathbf{i}^\prime$ of $\mathbf{i}$.
Additionally, with $d$, $s$, $e$, and $i$,
  if there exists some instantiation $p$ of $s$ for which
  $\mathcal{I}_V(d, \mathbf{i}^\prime) = \lrinterp(p, e, \mathbf{i}^\prime)$ 
  for all
  valid instantiations $\mathbf{i}^\prime$ of $\mathbf{i}$,
  then $\lrfn(d, s, e, \mathbf{i})$
  will either return a value or time out.

% \subsection{Correctness of the \lrfn{} Function}

% \hl{Gus:Enumerate the 
%  TCB,
%  if we really want to show
%  that we're serious
%  about correctness Solver, semantics importer (a number of components within Yosys + our $\sim$300 line btor to Racket compiler)}
%  \hl{Ben: The TCB is roughly enumerated after Property 3 is listed.}

% The \lr-Correct property says that
%   for instruction specification $s$, 
%   HDL program $v$,
%   architecture description $d$,
%   vendor-supplied semantics $e$,
%   and inputs $i$,
%   if synthesis and HDL compilation
%   with \lrfn on the instruction
%   specified by $s$
%   and architecture described by $d$
%   results in a HDL implementation $v$,
%   then simulating $v$ on inputs $i$
%   produces the same result as evaluating $s$
%   on inputs $i$. \hl{Should we talk here about how signals aren't relevant to the output comparison, just a way for interpretation to get to the output?}\\

% \newtheorem{property}{Property}
% \begin{property}[\lr-Correct]
% For all \(s \in \Spec\),
%         \(v \in \HDL\),
%         \(d \in \ArchDescr\),
%         \(e \in \VendorSemantics\)
%         and inputs \(\mathbf{i}\)
%   \[\lrfn(s,d,e) = v \implies 
%      \denote{s}_{\text{bv}}(i) 
%          = 
%      \denote{v}_{\text{HDL}}(i).\]
% \end{property}

% \hl{should we have
% (flr(...) = fc(fs(...)) = ...? or just one of those things? in which case, which one?}

% The commutative diagram in \cref{fig:correctness-comm-diagram}
%   shows how the \lr-Correct property
%   is composed from the
%   the Synth-Correct (bottom left triangle) and
%   Compile-Correct (bottom right triangle) properties,
%   which we describe below.
  
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % COMMUTATIVE DIAGRAM FIGURE
% \input{figures/correctness-comm-diagram}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % Synth Correct Theorem Section
% The Synth-Correct property states
%   that when performing \LRSynthesis on a specification produces
%   a result, that result is correct.\\


% \hl{
% TODO:
% we have a big down arrow for what lakeroad program evals to over one timestep, we need a big down arrow that represents time stepping over multiple timesteps.}

% %%%%%%%%%%%%%%%%%%%%%%
% % Synth Correct Theorem
% \begin{property}[Synth-Correct]
%   For all \(k \in \Sketch\),
%   \(s \in \textsc{Spec}\),
%   \(c \in \ArchDescr\),
%   \(e \in \VendorSemantics\),
%   \(p \in \lrir\),
%   and inputs \(\mathbf{i}\),
%   \[\LRSynthFn(k, s, e) = p \implies \denote{s}_{bv}(i) = \denote{p}_{\lrir}(e)(i)\]
% \end{property}
% \label{thm:synth-correct}
% % End Synth Correct Theorem
% %%%%%%%%%%%%%%%%%%%%%%

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % Compile Correct Theorem Section

% The Synth-Correct property asserts that 
%   the \HDLCompilation component preserves semantics.\\

% %%%%%%%%%%%%%%%%%%%%%%
% % Compile Correct Theorem
% \begin{property}[Compile-Correct]
%   For all \(p \in \textsc{Impl}\) and all inputs \(i\),
%   \[\HDLCompFn(p) = v \implies \denote{p}_\lrir(e)(i) = \denote{v}_\HDL(i).\]
% \end{property}
% \label{thm:compile-correct}
% % End Compile Correct Theorem
% %%%%%%%%%%%%%%%%%%%%%%

% The Synth-Correct property depends on
%   the correctness of the synthesis tool (in our case Rosette~\cite{torlak2014lightweight, torlak2013growing}),
%   the correctness of vendor-supplied HDL FPGA primitive semantics,
%   and the correctness of our \lrir interpreter.
% All three of these pieces are real software and are thus subject
%   to bugs in principle,
%   but all are heavily tested and thus reasonable
%   inclusions in our trusted computing base.
% Rosette in particular is a widely-used
%   by the Programming Languages and Program Synthesis communities.
% \lr's core \lrir interpreter is straightforward and
%   lifts bitvector and list manipulation
%   functions from Rosette and Racket.
% As such its correctness depends primarily on that of the host languages, though we  have also extensively tested it.
% All hardware-specific portions of the \lrir interpreter are imported
%   automatically from vendor-supplied HDL primitive specifications.
% We assume that these specs are correct as they are provided as ground truth
%   by vendors.
% Again, we have also validated this 
%   importing process through
%   extensive testing.
% Finally, the Compile-Correct property relies
%   on the simplicity of \lrir: each component
%   of \lrir maps directly to the
%   resulting Verilog implementation,
%   and compilation is a simple
%   syntactic transformation.


  
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% GRAVEYARD
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \begin{figure}
% \hl{ben: ltop and ptol should also have some shift functionality}
% \begin{verbatim}
% spec ::= <bv-const> | <bv-var>
%       | <binop> <spec> <spec>
%       | <unop> <spec> <spec>
%       | extract <nat> <nat> <spec>
%       | concat <spec> ...
%       | zero-extend <spec> <nat>
%       | list <spec> ...
%       | list-ref <spec> <nat>

% binop ::= bvand | bvor | bvxor 
%         | bvadd | bvsub | bvmul
        
% unop  ::= bvnot

% impl  ::= bv <bv-const-or-var>
%         | extract <nat> <nat> <impl>
%         | logical-to-physical <ltop> <impl> ...
%         | physical-to-logical <ptol> <impl> ...
%         | primitive <name> <spec> ...

% sketch ::= impl with holes
        
% ltop  ::= bitwise
%         | bitwise-reverse

% ptol  ::= bitwise
%         | bitwise-reverse
% \end{verbatim}
% \caption{Caption}
% \label{fig:syntax}
% \end{figure}


==> text/formalization-old-1.tex <==
\section{Formalization}
\label{sec:formalization}

In this section we formalize
  the syntax and semantics of \lr,
  and then state and prove
  soundness and completeness properties (assuming the correctness of the underlying program synthesis tool and HDL compiler).
%We begin by stating the soundness and
  %and completeness properties, and then
  %build up the necessary machinery to prove
  %them bottom up.

%\hl{TODO: State soundness and completeness theorems}

%\hl{Note: This is a rough narrative pass/overview of formalization. It should be compiled town to paper-worth latex.
%}

%To talk about correctness and completeness we need to construct an abstract mathematical model of Anaxi. So, the outline of this writeup is:

% \begin{enumerate}
% \item Syntax and Semantics
% \item Mathematical Model of Anaxi
% \item Correctness of Anaxi
% \item Completeness of Anaxi
% \end{enumerate}

\subsection{Syntax and Semantics}

%\input{figures/lakeroad-dsl-grammar}

%\input{figures/lakeroad-dsl-semantics}

\lr uses the \lr Intermediate Representation (\lrir) to represent
  wire operations and computations on FPGAs, the grammar for which is given in Figure~\ref{fig:lakeroad-dsl-grammar}.
Sketches use the \texttt{hole} construct
  to indicate where
  program synthesis should be used
  to find a replacement AST subtree
  for that hole 
  (either finding a bitvector to substitute or choosing between a list of alternatives).
Otherwise, the grammar consists
  of constructs corresponding to
  what can be implemented on the FPGA.
Wire operations are performed
  by direct
  bitvector manipulations
  like \texttt{concat}
  and \texttt{extract},
  and by high-level manipulations
  via the \texttt{wire} construct;
  these are all architecture-independent.
\lrir supports
  only these simple bitvector operations directly.
More complex manipulations
  are supported through calls 
  to \textit{hardware primitives} (e.g., LUTs and DSPs).
These hardware module invocations
  are captured in \lrir
  by \texttt{prim} terms,
  which refer to primitives
  by name (e.g., ``\texttt{LUT4}'')
  and pass in a configuration.
These constructs can all be lowered
  straightforwardly to HDL code
  that can in turn be compiled
  to an FPGA configuration.

\subsubsection{Combinational Semantics}

The basic operations in \lrir%
  ---all other than \texttt{prim}---%
  have stateless (combinational) semantics.
Namely, they are defined over
  bitvectors and lists,
  taking bitvectors or lists of bitvectors as arguments
  and returning a new bitvector or list of bitvectors,
  without any other changes
  to the program state.
The semantics for these constructs 
  is given in Figure~\ref{fig:lrir-semantics}.


% At its core,
%   \lrir is
%   an IR for manipulating
%   bitvectors and lists, where \lrir expressions should convert directly to low-level, FPGA-specific Verilog
%   code.
% % A primary design goal of \lrir
% %   is that expressions
% %   should convert directly
% %   to low-level, FPGA-specific
% %   Verilog code.
% This means that
%   \lrir directly supports only a limited subset
%   of possible bitvector operations
%   (e.g., bit extraction
%   or bitvector concatenation).
% More complex manipulations,
%   including computations
%   over bitvectors,
%   are supported only through calls to
%   \textit{hardware primitives} (e.g., LUTs and DSPs)
%   by using a \texttt{prim} expression;
%   these \texttt{prim} expression
%   can be directly converted
%   to Verilog module instantiations.
% Its leaf expressions
%   are bitvector constants
%   and variables,
%   where variables
%   represent the inputs
%   to the program.

\hl{The semantics define an interpreter $\mathcal{I}$}

We need to define the semantics for:

1. \textit{Combinational evaluation (w/out state...state is elided)}
2. \textit{Sequential evaluation (w/ state)}


\subsubsection{Combinational Semantics}
\hl{Update and reference figure 7 in paper; discuss}

\subsubsection{Sequential Semantics}
\hl{Update and reference figure 5 in paper; discuss}

\subsection{Mathematical Model of Anaxi}

In this section formalize Anaxi by modelling it a function 

$$f_A : Sketch \times Design \times Sems \to HDL$$
$$f_A := f_{HDL} \circ f_{Synth}$$

where
$$f_{Synth} : Sketch \times Design \times Sems \to IR$$
and
$$f_{HDL} : IR \to HDL.$$

We do not include sketch generation
  as part of our formalization, and treat
  it as a preprocessing step.


\subsubsection{Anaxi Synthesis: $f_{Synth}$}

The synthesis step takes a sketch $s$, a design $d$, and some interpreter $\mathcal{I}$, and queries Rosette to find an implementation $p$ of sketch $s$ such that for all inputs $i$, $p(i) = d(i)$. Here our design $d$ is being used as a specification.

We need to be able to
  synthesize \textit{combinational}
  and \textit{sequential} programs. 

\begin{itemize}
\item \textbf{Synthesizing a Combinational Program:}
  To synthesize a combinational
    program we pass the sketch
    $s$ to Rosette,
    along with an interpreter
    defined by the combinational
    semantics described in the
    \hl{Combinational Semantics}
    section.
  No state (e.g., clock cycles,
    etc) are used here.

  We then issue a query to Rosette:
  
  $$\forall i\ \in Inputs\ \exists p \in AxIR\ s.t. p(i) = d(i)$$

  Rosette performs exhaustive
    search to find
    a $p$ that satisfies
    these constraints
    if one exists.
    
\item \textbf{Synthesizing Sequential Programs:}
  To synthesize a sequential
    program we need to
    implement the semantics of
    multiple clock cycles.
  We do this by treating
    a program $p$ as a
    function from $k$ input
    bits and an input
    state to $\ell$ output
    bits and an output
    state $\Sigma$:

  $$p : \mathbb B^k \times \Sigma \to \mathbb B^\ell \times \Sigma.$$

  We represent $n$ 
    sequential applications
    of program $p$ with
    the function
    
  \[ p^{*}: \left(\mathbb{B}^k\right)^n \times \Sigma \to \mathbb{B}^\ell \times \Sigma,\]

  where

  \[p^{*}( \langle b_1, b_2, \ldots, b_n\rangle,\ \sigma_0)\]
  
  is defined to be
  
  $$p(b_1,\ \sigma_0)$$
  
  if $n = 1$, and
  \[p^{*}(\langle b_2, \ldots, b_n\rangle,\ \pi_\Sigma(s(b_1, \sigma_0)))\]
  
  if $n > 1$.



  Each $b_i \in \mathbb{B}^k$ 
    is the input bits 
    being wired to the
    circuit at time step $i$,
    and $\pi_\Sigma: \mathbb{B}^\ell \times \Sigma \to \Sigma$
    is the projection 
    function that drops
    the output bits and
    returns only the
    resulting state.

\hl{NOTE: we can model this in two ways: as a vectorized notation, or as an inductive definition. Both are usable; the above is inductive.}

  We then issue a query to Rosette:

  $$\forall \hat{b} \ \in \left(\mathbb{B}^k\right)^n,\ \exists p \in AxIR\ s.t.\ \pi_{Val} (p(\hat{b}, \sigma_0)) = \pi_{Val}(d(\hat{b}, \sigma_0)),$$

  where $\hat{b} = \langle b_1, \ldots, b_n\rangle$.

\end{itemize}

\subsubsection{Anaxi Compilation: $f_{HDL}$}
\hl{TODO: Discuss the process of compilation (Gus will need to do this!)}

\subsection{Program Synthesis}

The definition of program synthesis is

$$\exists p\,\, \forall \hat{i} \quad Spec(\hat{i}) = p(\hat{i})$$


\subsection{Correctness of Anaxi}

Correctness of Anaxi is decomposed into correctness of synthesis and correctness of compilation.

\hl{TODO: add commutative diagram!}

\subsubsection{Correctness of Compilation}

Correctness of compilation states that whenever $f_{HDL}$ maps an IR program $p$ to an HDL program $v$, this transformation preserves the semantics of the IR program: $\llbracket p\rrbracket = \llbracket v \rrbracket$.

We claim that compilation is correct. While we do not have a formal proof (e.g., from a proof assistant), compilation is a simple process and we have tested it extensively.

\subsubsection{Correctness of Synthesis}

\begin{itemize}
\item \textbf{Our TCB}
  \begin{itemize}
	\item Rosette/Solvers
	\item Interpreter $\mathcal{I}$ , which in turn depends on
     \begin{itemize}
		\item Vendor-supplied semantics
		\item Translation of semantics into an interpreter
        \end{itemize}
    \end{itemize}
\end{itemize}

Correctness of synthesis states that whenever $f_{Synth}$ maps a sketch $s$, a design $d$, and an interpreter $\mathcal{I}$ to an IR program $p$, then the semantics of the original design are preserved: $[|d|] = [|p|]$.

We get correctness of synthesis from Rosette: by the definition of program synthesis, as long as our query that we have constructed is correct then the resulting. Correctness of synthesis relies on the correctness of Rosette. We construct a query

\subsection{Completeness of Anaxi}

Anaxi cannot claim full completeness, but it can claim \textit{sketch completeness:} if there is a sketch that can be instantiated to a program that implements a design $d$, then up to timeouts Anaxi will find it. We break sketch completeness down into \textit{Sketch Completeness of Synthesis} and \textit{Completeness of Compilation}.

\subsubsection{ Sketch-Completeness of Synthesis}

We argue that $f_{Synth}$
  is sketch-complete: that is,
  if there exists a program $p'$
  that can be formed by
  implementing a sketch 
  $s$ such that
  $\llbracket p'\rrbracket = \llbracket d \rrbracket$
  then $f_{Synth}$ will
  produce some program 
  $p$ (where $p \equiv p'$).

Stated another way,
  sketch-completeness of
  synthesis states that $f_{Synth}$
  is total on the restricted 
  domain of 
  $Sketch \times Design \times Sems$.
This follows from the
  definition of program
  synthesis \hl{(todo: elaborate)}.

\subsubsection{Completeness of Compilation}

Completeness of compilation says that $f_{HDL}$ is a total function (i.e., compilation never fails).



==> text/formalization-old-2.tex <==
\section{Formalization}
\label{sec:formalization}

\input{figures/syntax}


In this section we formalize
  the syntax and semantics of \lr,
  and then state and prove
  soundness and completeness properties (assuming the correctness of the underlying program synthesis tool and HDL compiler).
%We begin by stating the soundness and
  %and completeness properties, and then
  %build up the necessary machinery to prove
  %them bottom up.

%\hl{TODO: State soundness and completeness theorems}

%\hl{Note: This is a rough narrative pass/overview of formalization. It should be compiled town to paper-worth latex.
%}

%To talk about correctness and completeness we need to construct an abstract mathematical model of Anaxi. So, the outline of this writeup is:

% \begin{enumerate}
% \item Syntax and Semantics
% \item Mathematical Model of Anaxi
% \item Correctness of Anaxi
% \item Completeness of Anaxi
% \end{enumerate}

\subsection{Syntax and Semantics}

%\input{figures/lakeroad-dsl-grammar}

%\input{figures/lakeroad-dsl-semantics}

\lr uses the \lr Intermediate Representation (\lrir) to represent
  wire operations and computations on FPGAs, the grammar for which is given in Figure~\ref{fig:lakeroad-dsl-grammar}.
Sketches use the \texttt{hole} construct
  to indicate where
  program synthesis should be used
  to find a replacement AST subtree
  for that hole 
  (either finding a bitvector to substitute or choosing between a list of alternatives).
Otherwise, the grammar consists
  of constructs corresponding to
  what can be implemented on the FPGA.
Wire operations are performed
  by direct
  bitvector manipulations
  like \texttt{concat}
  and \texttt{extract},
  and by high-level manipulations
  via the \texttt{wire} construct;
  these are all architecture-independent.
\lrir supports
  only these simple bitvector operations directly.
More complex manipulations
  are supported through calls 
  to \textit{hardware primitives} (e.g., LUTs and DSPs).
These hardware module invocations
  are captured in \lrir
  by \texttt{prim} terms,
  which refer to primitives
  by name (e.g., ``\texttt{LUT4}'')
  and pass in a configuration.
These constructs can all be lowered
  straightforwardly to HDL code
  that can in turn be compiled
  to an FPGA configuration.

\subsubsection{Combinational Semantics}

The basic operations in \lrir%
  ---all other than \texttt{prim}---%
  have stateless (combinational) semantics.
Namely, they are defined over
  bitvectors and lists,
  taking bitvectors or lists of bitvectors as arguments
  and returning a new bitvector or list of bitvectors,
  without any other changes
  to the program state.
The semantics for these constructs 
  is given in Figure~\ref{fig:lrir-semantics}.


% At its core,
%   \lrir is
%   an IR for manipulating
%   bitvectors and lists, where \lrir expressions should convert directly to low-level, FPGA-specific Verilog
%   code.
% % A primary design goal of \lrir
% %   is that expressions
% %   should convert directly
% %   to low-level, FPGA-specific
% %   Verilog code.
% This means that
%   \lrir directly supports only a limited subset
%   of possible bitvector operations
%   (e.g., bit extraction
%   or bitvector concatenation).
% More complex manipulations,
%   including computations
%   over bitvectors,
%   are supported only through calls to
%   \textit{hardware primitives} (e.g., LUTs and DSPs)
%   by using a \texttt{prim} expression;
%   these \texttt{prim} expression
%   can be directly converted
%   to Verilog module instantiations.
% Its leaf expressions
%   are bitvector constants
%   and variables,
%   where variables
%   represent the inputs
%   to the program.

\hl{The semantics define an interpreter $\mathcal{I}$}

We need to define the semantics for:

1. \textit{Combinational evaluation (w/out state...state is elided)}
2. \textit{Sequential evaluation (w/ state)}


\subsubsection{Combinational Semantics}
\hl{Update and reference figure 7 in paper; discuss}

\subsubsection{Sequential Semantics}
\hl{Update and reference figure 5 in paper; discuss}

\subsection{Mathematical Model of Anaxi}

In this section formalize Anaxi by modelling it a function 

$$f_A : Sketch \times Design \times Sems \to HDL$$
$$f_A := f_{HDL} \circ f_{Synth}$$

where
$$f_{Synth} : Sketch \times Design \times Sems \to IR$$
and
$$f_{HDL} : IR \to HDL.$$

We do not include sketch generation
  as part of our formalization, and treat
  it as a preprocessing step.


\subsubsection{Anaxi Synthesis: $f_{Synth}$}

The synthesis step takes a sketch $s$, a design $d$, and some interpreter $\mathcal{I}$, and queries Rosette to find an implementation $p$ of sketch $s$ such that for all inputs $i$, $p(i) = d(i)$. Here our design $d$ is being used as a specification.

We need to be able to
  synthesize \textit{combinational}
  and \textit{sequential} programs. 

\begin{itemize}
\item \textbf{Synthesizing a Combinational Program:}
  To synthesize a combinational
    program we pass the sketch
    $s$ to Rosette,
    along with an interpreter
    defined by the combinational
    semantics described in the
    \hl{Combinational Semantics}
    section.
  No state (e.g., clock cycles,
    etc) are used here.

  We then issue a query to Rosette:
  
  $$\forall i\ \in Inputs\ \exists p \in AxIR\ s.t. p(i) = d(i)$$

  Rosette performs exhaustive
    search to find
    a $p$ that satisfies
    these constraints
    if one exists.
    
\item \textbf{Synthesizing Sequential Programs:}
  To synthesize a sequential
    program we need to
    implement the semantics of
    multiple clock cycles.
  We do this by treating
    a program $p$ as a
    function from $k$ input
    bits and an input
    state to $\ell$ output
    bits and an output
    state $\Sigma$:

  $$p : \mathbb B^k \times \Sigma \to \mathbb B^\ell \times \Sigma.$$

  We represent $n$ 
    sequential applications
    of program $p$ with
    the function
    
  \[ p^{*}: \left(\mathbb{B}^k\right)^n \times \Sigma \to \mathbb{B}^\ell \times \Sigma,\]

  where

  \[p^{*}( \langle b_1, b_2, \ldots, b_n\rangle,\ \sigma_0)\]
  
  is defined to be
  
  $$p(b_1,\ \sigma_0)$$
  
  if $n = 1$, and
  \[p^{*}(\langle b_2, \ldots, b_n\rangle,\ \pi_\Sigma(s(b_1, \sigma_0)))\]
  
  if $n > 1$.



  Each $b_i \in \mathbb{B}^k$ 
    is the input bits 
    being wired to the
    circuit at time step $i$,
    and $\pi_\Sigma: \mathbb{B}^\ell \times \Sigma \to \Sigma$
    is the projection 
    function that drops
    the output bits and
    returns only the
    resulting state.

\hl{NOTE: we can model this in two ways: as a vectorized notation, or as an inductive definition. Both are usable; the above is inductive.}

  We then issue a query to Rosette:

  $$\forall \hat{b} \ \in \left(\mathbb{B}^k\right)^n,\ \exists p \in AxIR\ s.t.\ \pi_{Val} (p(\hat{b}, \sigma_0)) = \pi_{Val}(d(\hat{b}, \sigma_0)),$$

  where $\hat{b} = \langle b_1, \ldots, b_n\rangle$.

\end{itemize}

\subsubsection{Anaxi Compilation: $f_{HDL}$}
\hl{TODO: Discuss the process of compilation (Gus will need to do this!)}

\subsection{Program Synthesis}

The definition of program synthesis is

$$\exists p\,\, \forall \hat{i} \quad Spec(\hat{i}) = p(\hat{i})$$


\subsection{Correctness of Anaxi}

Correctness of Anaxi is decomposed into correctness of synthesis and correctness of compilation.

\hl{TODO: add commutative diagram!}

\subsubsection{Correctness of Compilation}

Correctness of compilation states that whenever $f_{HDL}$ maps an IR program $p$ to an HDL program $v$, this transformation preserves the semantics of the IR program: $\llbracket p\rrbracket = \llbracket v \rrbracket$.

We claim that compilation is correct. While we do not have a formal proof (e.g., from a proof assistant), compilation is a simple process and we have tested it extensively.

\subsubsection{Correctness of Synthesis}

\begin{itemize}
\item \textbf{Our TCB}
  \begin{itemize}
	\item Rosette/Solvers
	\item Interpreter $\mathcal{I}$ , which in turn depends on
     \begin{itemize}
		\item Vendor-supplied semantics
		\item Translation of semantics into an interpreter
        \end{itemize}
    \end{itemize}
\end{itemize}

Correctness of synthesis states that whenever $f_{Synth}$ maps a sketch $s$, a design $d$, and an interpreter $\mathcal{I}$ to an IR program $p$, then the semantics of the original design are preserved: $[|d|] = [|p|]$.

We get correctness of synthesis from Rosette: by the definition of program synthesis, as long as our query that we have constructed is correct then the resulting. Correctness of synthesis relies on the correctness of Rosette. We construct a query

\subsection{Completeness of Anaxi}

Anaxi cannot claim full completeness, but it can claim \textit{sketch completeness:} if there is a sketch that can be instantiated to a program that implements a design $d$, then up to timeouts Anaxi will find it. We break sketch completeness down into \textit{Sketch Completeness of Synthesis} and \textit{Completeness of Compilation}.

\subsubsection{ Sketch-Completeness of Synthesis}

We argue that $f_{Synth}$
  is sketch-complete: that is,
  if there exists a program $p'$
  that can be formed by
  implementing a sketch 
  $s$ such that
  $\llbracket p'\rrbracket = \llbracket d \rrbracket$
  then $f_{Synth}$ will
  produce some program 
  $p$ (where $p \equiv p'$).

Stated another way,
  sketch-completeness of
  synthesis states that $f_{Synth}$
  is total on the restricted 
  domain of 
  $Sketch \times Design \times Sems$.
This follows from the
  definition of program
  synthesis \hl{(todo: elaborate)}.

\subsubsection{Completeness of Compilation}

Completeness of compilation says that $f_{HDL}$ is a total function (i.e., compilation never fails).



==> text/graveyard.tex <==
\section{Related Work}
\label{sec:background-and-related-work}

% \hl{Vector Instruction Selection for Digital Signal Processors using Program Synthesis}

% \hl{metasketches bornholt}

% \hl{Synthesizing an instruction selection rule library from semantic specifications}

% \hl{TODO: find papers
% where people automatically synthesize
% implementations
% of LLVM or other ISAs
% for specific CPU architectures.}

% People keep challenging FPGA compilation; people are reinventing things; we want to do soemthing foundational. Their work can leverage our work.
% Remember: you're giving people control of their "destiny"
% Simplest example: how do i do an addition with or without the carry chain? the tool doesn't let them do that!
% Or maybe a different way to think about it: we can give you a pareto curve of different instruction impls
% https://www.csl.cornell.edu/~zhiruz/pdfs/impress-fccm2022.pdf


% \section{Related Work from Generals, filter into above section}
  
\subsection{Hardware Compilation}
\label{sec:background-hardware-compilation}

Hardware compilation
  is the process of lowering
  a high-level hardware representation
  into a final form, ready for
  fabrication.
For FPGAs,
  this final form
  is a binary ``bitstream''
  which is sent to the FPGA
  and which configures the various
  lookup tables,
  digital signal processors,
  memories,
  interconnects,
  and other programmable components.
Within the field
  of hardware design,
  hardware compilation
  is called
  \textit{hardware synthesis.}
We will avoid
  this terminology,
  however,
  as
  ``synthesis''
  has a different meaning
  in the field of
  programming languages,
  where it
  generally
  refers to
  solver-aided programming.
To resolve the overloading,
  we will refer to 
  \textit{hardware synthesis}
  as \textit{hardware compilation,}
  and only use the term \textit{synthesis}
  to refer to processes
  which rely on solver-aided reasoning.

Traditional hardware compilation
  involves a number of stages:
  \textit{logic synthesis}
  (another, independent use
    of the word \textit{synthesis!}),
  in which the design is
  compiled to boolean logic
  and optimized;
  \textit{technology mapping,}
  in which portions of the
  boolean logic
  are grouped into higher-level
  functional units;
  and
  \textit{placement and routing,}
  in which gates and wires
  are assigned to actual locations
  on the device.
Our work will only deal with
  logic synthesis
  and technology mapping.
Furthermore,
  we will deal specifically with
  compilation to FPGAs.
Hardware compilation for ASICs
  is far more complicated,
  and out of the scope of this thesis.

Unlike software compilation
  tools
  in recent decades,
  hardware compilation
  continues to be dominated
  by proprietary toolchains
  controlled by each
  target platform's vendor,
  such as Xilinx's
  Vivado Design Suite~\cite{vivado}.
A number of open source tools
  have been developed
  in academia
  and in industry%
  % Catchall list of cites that we don't write
  % about otherwise.
  ~\cite{rose2012vtr, lavin2018rapidwright}.
A notable example
  with fairly widespread use
  is Yosys~\cite{wolf2013yosys}.
  
A recent high-profile
  entry into the hardware compilers space
  is the CIRCT project~\cite{eldridge2021mlir,urbach2022hls}.
CIRCT is part of
  the new compiler framework
  MLIR~\cite{lattner2021mlir},
  whose vision
  is to unify the growing web
  of compilers
  spread across different abstraction
  levels
  and targeting different backends
  under one 
  infrastructure,
  allowing for easier translation
  and greater sharing
  between compiler projects.
CIRCT seeks to treat
  hardware compilation
  more like software compilation,
  by lowering hardware designs
  through their various levels of abstraction.
  
A common theme
  for experiments
  with new hardware compilation tools
  are attempts to bring
  ideas from software compilation
  into hardware compilation.
PLD~\cite{xiao2022pld}
  brings the idea of 
  \texttt{-O0}
  and
  \texttt{-O1}
  flags from common software
  compilers such as
  GCC to hardware compilation.
Rather than recompiling
  an entire hardware design
  on every compilation,
  as is the norm with current tools,
  PLD gives users the option
  of faster compilation
  by trading off for
  a
  less-optimized placement and routing result,
  in addition to the ability
  to forego compilation entirely
  and use software simulators
  for portions of the design.
\cite{schkufza2019cascade}
  tackles the same issue
  of long compilation times
  by borrowing the idea of
  just-in-time (JIT)
  compilation
  from software compilers.
When the developer
  initiates a test
  on the hardware,
  it initially launches
  as a software simulation.
In the background,
  hardware compilation is running;
  as it runs,
  simulated
  components of the hardware design
  are swapped for their
  freshly-compiled
  real counterparts
  on the fly.
  
In addition to focusing
  on \textit{usability,}
  there is a focus on
  \textit{correctness}
  in new hardware compilers.
Those without experience
  in software
  might be surprised by
  the bugs
  and instabilities in
  modern commercial
  hardware compilers.
\cite{herklotz2021empirical} finds that
  a number of commercial HLS compilers
  produce incorrect hardware
  in 2.5\% of cases;
  as a result,
  \cite{herklotz2021formal} presents
  the first formally-verified
  HLS compiler from C
  by building a Verilog backend
  for the formally verified CompCert
  C compiler~\cite{leroy2016compcert}.
Works which focus on correctness
  will be further highlighted
  in Section%
  ~\ref{sec:background-formal-hardware-models}
  

%\hl{Anna Goldie}
%Researchers are experimenting
%  with AI techniques
%  to revolutionize
%  hardware compilers.
%\cite{mirhoseini2021graph}
%  utilizes 
%  deep reinforcement learning
%  to implement floorplanning,
%  a crucial step
%  in hardware compilation.


%\hl{heterohalide}
%% https://vast.cs.ucla.edu/~chiyuze/publication/heterohalide/
%I'm not sure
%  why I don't like this; it's just not really in my taste.
%They go from Halide
%  to HeteroCL to FPGA?
%One of their innovations is this lazy vs immediate
%  application
%  of schedule primitives,
%  which I'm not sure I really buy.
%They output through three
%  backends:
%  SODA, PolySA, and Merlin.
  
Another feature of software compilation
  which has been ported
  to hardware
  is \textit{portability:}
  the ability for hardware designs
  to be compiled to 
  multiple underlying
  FPGA platforms.
This is generally done by 
  building a "virtual"
  FPGA architecture
  which designs can target,
  and building an optimized
  implementation
  of that virtual architecture
  for each underlying FPGA%
  ~\cite{lysecky2005firm,brant2012zuma, landgraf2021compiler}.
Virtual FPGA architectures
  come with a steep resource
  and performance overhead.
  
Faster and
  more flexible
  hardware compilation
  is so desirable
  that 
  a number of approaches 
  go so far as to
  propose special 
  hardware for which
  compilation is easier%
  ~\cite{xiao2022pld,lysecky2004configurable,sekanina2000r,lysecky2004dynamic,stitt2003dynamic}.


%\hl{Multiplication by constant block}
% \hl{https://citeseerx.ist.psu.edu/viewdoc/download?doi=10.1.1.119.2295&rep=rep1&type=pdf}

New approaches to compilation
  often take issue
  with a fundamental step
  in traditional hardware compilation,
  in which the input design---%
  represented in a high-level,
  semantically rich language
  like behavioral SystemVerilog---%
  is compiled all the way down
  to a low-level representation
  like and--inverter graphs%
  ~\cite{callahan1998fast}.
This makes the process of
  technology mapping
  for FPGAs challenging,
  as the low-level representation
  must be lifted up
  to the 
  higher level of abstraction
  of FPGA primitives,
  such as look-up tables (LUTs)
  or even digital signal processors (DSPs).
Reticle~\cite{vega2021reticle},
  which our work builds directly off of,
  introduces a new representation
  which is compiled directly to
  FPGA primitives
  via instruction selection.
  
  
%\hl{Utah prof's FPGA work, openFPGA}
%https://github.com/lnis-uofu/OpenFPGA


\subsection{Formal Hardware Models}
\label{sec:background-formal-hardware-models}

Given that my goal
  is to use formal hardware models
  to automatically generate
  compiler components,
  it is first important to
  give an idea of
  the formal hardware models
  that are
  in common use,
  and others that have been proposed
  in the literature.
  
Classic examples
  of these languages
  are VHDL~\cite{ieee20191076}
  and Verilog/SystemVerilog~\cite{design2005ieee}.
These languages
  were initially designed
  for hardware verification tasks.
Note that
  ``verification'' has different meanings
  in hardware and in software,
  as is well explained
  in the introduction of \cite{choi2017kami}.
The verification tasks
  which Verilog and VHDL
  were initially built for
  are perhaps more appropriately
  called ``simulation,''
  in which the verification engineer
  designs a model of the hardware
  in VHDL/SystemVerilog,
  and tests the real hardware
  against the model
  on test inputs.
Eventually,
  the languages also
  began to be used
  as frontend languages
  for hardware design;
  rather than simply simulating
  the design,
  why not convert the model
  directly to hardware itself?
SystemVerilog and VHDL
  contain two distinct
  levels of abstraction.
The lowest level
  SystemVerilog or VHDL---%
  referred to as
  \textit{structural}---%
  fully describes a hardware design
  at the 
  \textit{register transfer level:}
  which gates and registers
  are present,
  and which wires connect to
  which ports.
Both languages can also describe
  designs
  \textit{behaviorally,}
  as well.
Behavioral SystemVerilog and VHDL
  describe the behavior
  of designs
  at each clock tick,
  or at the change
  of other signals.
  
Many or all of what I will refer to
  as the newer hardware design
  and modeling languages
  fall under the umbrella term
  \textit{high-level synthesis} (HLS).
In general,
  HLS refers
  to the process of compiling
  (or \textit{synthesizing})
  a hardware design
  from a
  high-level specification.
By this definition,
  some may even consider
  hardware compilation
  from behavioral
  SystemVerilog
  a form of HLS.
In practice, though,
  the term HLS
  is often very specifically used
  for hardware compilers
  which take subsets of C or C++
  as their input languages,
  for example,
  Vivado HLS, Intel i++, LegUp, and Bambu.
Much like in the case of
  the overloading
  of the term ``synthesis'', 
  I will avoid using
  ``high-level synthesis.''
  
Bluespec SystemVerilog~\cite{nikhil2004bluespec}
  raises the abstraction level
  of SystemVerilog.
While previous attempts
  at raising the abstraction level
  on SystemVerilog and VHDL
  went in the direction
  of using C and C++,
  Bluespec goes the opposite direction.
Bluespec embraces
  the massively parallel nature
  of hardware,
  using the abstraction of
  guarded atomic actions
  to express
  the fact that 
  many computations
  may be happening simultaneously,
  without a set ordering.
Compilers of Bluespec
  must decide on a
  definite
  \textit{schedule}
  when generating hardware.
\koika~\cite{bourgeat2020essence} introduces
  more control over scheduling
  which depends on dynamic analyses
  which might incur hardware overhead
  but can be simplified away
  potentially by static analyses.
Kami~\cite{choi2017kami}
  is a recent formalization
  of a subset of Bluespec
  in the theorem prover Coq.
Being embedded in Coq,
  Kami allows for 
  verification---%
  in the software sense of the word,
  that is, formal verification
  of mathematical properties---%
  of hardware designs
  by stating and proving theorems
  about them.
Kami can also be compiled
  to FPGAs.


The Instruction-Level Abstraction (ILA)
  is a representation developed
  for verifying complex
  systems-on-chip (SOCs),
  in which many specialized
  accelerators
  exist alongside
  the main processor~\cite{huang2018instruction}.
It provides a useful model of accelerators
  by assigning them
  an ISA-like
  set of instructions
  as their interface.

A number of recent representations
  enrich
   hardware design representations
  with new semantics.
Calyx~\cite{nigam2021compiler}
  explicitly separates
  datapath specification
  from control logic.
Dahlia~\cite{nigam2020predictable}
  uses affine types
  to more richly describe
  the semantics of
  reading to 
  and writing from
  memories
  in FPGAs.
Aetherling~\cite{durst2020type}
  presents a
  language
  which captures
  the spatial/temporal tradeoff
  of custom hardware,
  and uses the language
  to build streaming accelerators.
Reticle~\cite{vega2021reticle}
  adds placement information
  directly into the language
  representation,
  conveying useful information
  to the underlying tools.
  
%VTR~\cite{rose2012vtr}
%  allows users
%  to model FPGA architectures
%  in an XML-based representation.
  

%\hl{Lava}
% https://dl.acm.org/doi/10.1145/291251.289440
%It's a functional
%  language for hardware design.
%I'm not sure
%  how much more
%  I need to dig into it.
  
% \subsection{Compiler Backends and their Automated Construction}
% \label{sec:background-constructing-compilers}

% In this section,
%   I present
%   relevant
%   background
%   on compiler backends
%   and their automatic
%   construction.
% First, 
%   I cover compiler backends.
% Then, I describe the tools
%   useful in automating
%   compilation
%   and compiler generation,
%   namely equality saturation
%   and solver-aided programming.

% Compilers
%   are a broad topic,
%   but specifically relevant to us
%   are compiler
%   \textit{backends:}
%   the middle
%   and bottom layers
%   of a compiler
%   which deal with low-level
%   and often target-specific
%   optimizations,
%   and generate
%   target-specific
%   code.
% Two primary components
%   of
%   compiler backends
%   which we care about
%   are
%   the \textit{optimization pipeline}
%   and 
%   the \textit{code generator.}
% The optimization pipeline
%   for a compiler backend
%   performs optimizations such as
%   \textit{scheduling transformations,}
%   which seek to make the code
%   more performant
%   on the target architecture.
% The code generator
%   converts the final, optimized program
%   from its higher-level
%   representation
%   to the target-specific
%   instruction set
%   (often called
%   \textit{instruction selection}
%   or \textit{mapping})
%   and outputs it in the format
%   expected by the 
%   target architecture
%   (or by the next stage
%   of the compilation pipeline).
  
  
  

%\subsection{Tensor Language Representations}
%
%\hl{CFDlang}
%% https://www.cfaed.tu-dresden.de/files/Images/people/chair-cc/publications/1802_Rink_RWDSL.pdf
%Might be comparable to \g?
%
%{\color{green}\hl{Gilbert's ATL paper}}
%ATL~\cite{liu2022verified, bernstein2020differentiating}
%  is an array-based language.
%Recently, it has been used
%  to
%  enable rewriting
%  over tensor-based
%  programs.
%\hl{Read more}

% \subsection{Optimization Pipelines}

% Tensor compilers for ML and HPC applications strive
%   to balance clear, high-level operator semantics
%   and support for the low-level optimizations
%   necessary to target specialized accelerators.
% Halide~\cite{ragan2013halide}
%   achieves this balance by separating
%   operator \textit{specifications} (what is computed) from
%   \textit{schedules} (how, when, and where
%   each output element is generated).
% This style of separation has proven
%   highly effective across both
%   application domains and hardware targets;
%   numerous compilers including TVM~\cite{chen2018tvm},
%   FireIron~\cite{hagedorn2020fireiron},
%   LIFT~\cite{lift}, and Accelerate~\cite{accelerate}
%   follow variations of this strategy.
  
% The specification/schedule separation approach
%   allows the same high-level program (specification)
%   to be flexibly optimized for and mapped to
%   different hardware targets by applying different schedules.
% From this perspective,
%   schedules represent different rewriting strategies
%   to explore various loop ordering and memory layouts;
%   in LIFT and Accelerate these
%   take the form of functional combinators
%   closely related to \g's approach.
% As in classic term rewriting,
%   experts must often carefully craft
%   schedules for each target to achieve
%   the best performance and mitigate
%   phase ordering challenges~\cite{phase-ordering},
%   though recent projects have produced promising results
%   in automatic scheduling~\cite{
%     chen2018autotvm, zheng2020ansor, anderson2020learning}.

% Other tensor IRs like
%   TACO~\cite{taco}, Keops~\cite{keops},
%   and COMET~\cite{tian2021highperformance}
%   rely on \textit{index notation}\footnote{
%     Index notation is closely related to
%     ``Einstein notation'' where reduction
%     indices are implicit.}
%   to concisely express tensor operators
%   and simplify optimization by
%   uniformly representing
%   per-output-element computations.
% These approaches also rely on
%   rewriting passes to generate
%   kernel implementations specialized to
%   tensor sparsity / density,
%   operator combinations arising in
%   the source application, and
%   details of the target hardware.
 
% Finally, polyhedral compilers~\cite{polyhedral-survey}
%   like Tensor Comprehensions~\cite{vasilache2018tensor}
%   and Tiramisu~\cite{baghdadi2019tiramisu}
%   optimize loop-filled programs
%   by modeling loop nests as polyhedra
%   and applying geometric transformations.
% The polyhedral approach exploits
%   regular loop structure,
%   but is also restricted
%   to geometrically affine transformations.
% In contrast, term rewriting is
%   neither guided nor restricted by
%   geometric constraints, making
%   these approaches broadly complementary.
  
\subsection{Mapping}

% In principle, many DSLs allow for supporting custom accelerators via bespoke translations from DSL operators to specific accelerator APIs,
% e.g., as in the original TVM~\cite{chen2018tvm} support for VTA~\cite{moreau2019hardware},
%   and ISA mapper's~\cite{sotoudeh2019isa}
%   support for mapping
%   to custom hardware.
% %
% TVM's BYOC~\cite{chen2021byoc} interface
% % provides a more convenient mechanism for
% eases incorporating custom accelerators
% %, especially for coarser-grained operations,
% by performing syntactic pattern matching to offload computations via user-provided code generators.
% % By building on TVM,
% %   BYOC inherits support for multiple frontends
% %   and additionally provides extensible pattern matching to facilitate
% %   adding new rules for mapping DSL fragments to new accelerators.
% %\hl{merge next two sentences?}
% However, BYOC leaves
%   all matters of code generation, e.g., MMIO invocations,
%   to the user.
% Additionally, BYOC's pattern matching
% cannot search the space of programs equivalent to the input,
% limiting the number of potential accelerator invocations.

Past work has also explored rewrite-based techniques for
  automatically inferring instruction selection passes
  between ISAs~\cite{ramsey2011resourceable}.
  
Recent work on accelerator generation and integration~\cite{
    bahr2020creating, truong2020fault}
  has explored adding support in the Halide~\cite{ragan2013halide}
  compiler flow for specialized Coarse-Grained Reconfigurable Array (CGRA) accelerators.
That work composes an
  impressive array of custom tools to
  generate and verify specialized CGRA accelerators
  and also map Halide program fragments
  down to accelerator invocations.
HeteroCL~\cite{lai2019heterocl} also provides
  a similar custom flow.
  
%designed around the details of the HeteroCL compiler flow.

%\subsection{ISA exploration}
%
%% 3/7/22 dreamcoder
%\hl{dreamcoder}
%% https://arxiv.org/pdf/2006.08381.pdf
%
%Creates languages, uses ML to search for programs within the language?
%
%Humans build from experience.
%Wake-sleep bayesian program induction.
%Off the bat: it feels too complicated for the task at hand.
%
%"Learning as program induction"---perhaps their goal really is different? They're really taking the AI angle, and just by chance making something that's interesting in the PL world?
%
%"Learning tasks in many different domains can be formulated as inducing a program that explains a small number of input output examles, orthat generats ano bserved sequence, image or scene.
%
%Wake-sle3ep: during wake te generative model is used to interpret new data (generated from where? from the model?) while during sleep the recognition model is learned from "imagined" datasets which are sampled from the generative model (ok so the first thing is not generated from the model, then?)
%
%Dreamcoder~\cite{ellis2018dreamcoder, ellis2020dreamcoder, ellis2021dreamcoder}
%  aims to learn programs
%  by building up libraries of concepts.
%They do so in ``wake--sleep cycles",
%  in which a generative model
%  is alternately trained
%  and drawn from (not sure??).
%This is similar
%  to our work, which also seeks
%  to learn concepts
%  from a corpus of hardware designs,
%  though we do so
%  in a more brute-force
%  and exhaustive manner.

% \subsection{Term Rewriting and Equality Saturation}

% Term rewriting is a useful tool
%   for program transformation,
%   and surely an inevitable part
%   of any automatic
%   compilation pipeline.
% Equality saturation
%   is a specific type of term rewriting
%   highly optimized for
%   running many rewrites.

% Term rewriting is a classic
%   program optimization technique~\cite{baader1999term}
%   that relies on iteratively applying
%   rewrite rules of the form $\ell \xrightarrow{} r$:
%   when part of a program
%   matches the pattern $\ell$
%   under substitution $\sigma$,
%   it is rewritten into $\sigma(r)$.
% This approach is ubiquitous,
%   frequently used in both mainstream and DSL compilers
%   to implement features including preprocessing,
%   strength reductions, and
%   peephole optimizations~\cite{garavel2018rewrite-context}.
  
% Classic term rewriting systems where
%   rewrites are applied destructively suffer
%   phase ordering problems~\cite{phase-ordering}:
%   the order in which rewrites are applied can
%   enhance or severely diminish performance.
% Recent work has shown how program synthesis
%   can help address this challenge in
%   peephole optimizers like Halide's
%   scalar expression rewriter~\cite{
%     newcomb2020halide-rewrite}.
  
% Advances in alternate rewriting techniques
%   like equality saturation~\cite{tate2009equality}
%   also mitigate phase ordering by exploiting
%   the e-graph data structure from SMT solvers
%   to repeatedly apply all rewrites simultaneously,
%   thus obviating rule ordering considerations.
% In particular,
%   the \tcd{egg} library~\cite{willsey2021egg}
%   has been used to develop new synthesis and
%   optimization tools across diverse domains~\cite{
%     herbie, szalinski, wang2020spores},
%   including DSP compiler vectorization~\cite{
%     vanhattum2021vectorization} and
%   tensor computation graphs~\cite{yang2021equality}.


% \subsection{Constraint Programming, Solver-Aided Programming, and Synthesis}

% Constraint programming
%   is a type of programming
%   in which,
%   rather than developing the algorithm
%   to solve a problem,
%   the programmer instead develops
%   a set of constraints
%   which define valid solutions
%   to the problem.
% The programmer then feeds the constraints
%   to a \textit{constraint solver,}
%   which searches for
%   a solution satisfying the constraints.
% At base, constraint programming
%   involves searching for solutions
%   which satisfy the provided constraints.
% For example, in the
%   boolean satisfiability (SAT) problem,
%   we seek
%   valid assignments to boolean variables
%   that satisfy a set of
%   boolean constraints.
% % GS: these sentences can be removed if 
% % we don't talk at all about optimization.
% % but I think lancelot uses optimization!
% Constraint programming
%   can also involve optimizing
%   a cost function,
%   subject to the provided constraints.
% Linear programming (LP)
%   and integer linear programming (ILP),
%   for example,
%   find assignments to real-valued
%   or integer-valued variables
%   which
%   minimize an objective function
%   while satisfying a set of linear constraints
%   over the variables.
  
% GS: SMT/z3 paragraph
\textit{Satisfiability modulo theories} (SMT)
  is a generalization of the SAT problem
  allowing for variables and constraints
  from domains
  (or \textit{theories})
  other than boolean,
  such as the bitvectors
  and uninterpreted functions.
Rosette~\cite{torlak2013growing,torlak2014lightweight}
  embeds SMT solving capabilities
  within the programming language
  Racket,
  enabling users to easily formulate
  constraint problems,
  or even use solvers
  to write programs themselves,
  also known as 
  \textit{solver-aided programming}
  or \textit{synthesis.}
Under the hood,
  Rosette is powered by
  Z3~\cite{de2008z3},
  a popular SMT solver.
Rosette and Z3 also support
  optimization:
  Rosette via Z3 can produce
  a solution which satisfies
  the constraints
  and which is optimal
  relative to a given
  cost function.


%\subsection{traditional sw compilation}
%
%\hl{norman ramsey}
%\hl{
%what if your ISA isn't fixed?
%why isn't norman ramsey's stuff good there?
%granularity mismatch
%for heterogeneous targets,
%isas alone are not enough for your model
%}
%\hl{yacc and other compiler compilers}

%\subsection{unsorted}
%
%\hl{exo compiler} % It's in our 3LA drive
%
%A Dynamically Scheduled HLS Flow in MLIR
%https://infoscience.epfl.ch/record/292189
%
%Multi-input Serial Adders for FPGA-like Computational Fabric: Google research on invetigating luts (has a video in supplemental material)
%
%Direct Spatial Implementation of Sparse Matrix
%Multipliers for Reservoir Computing (this was from the same authors as the google lut work, i think they used the above work to implement this)
%
%C. Wolf, J. Glaser. Yosys - A Free Verilog Synthesis Suite. In Proceedings of Austrochip 2013. [download pdf]
%
%
%J. Glaser and C. Wolf. Methodology and Example-Driven Interconnect Synthesis for Designing Heterogeneous Coarse-Grain Reconfigurable Architectures. In Jan Haase, editor, Models, Methods, and Tools for Complex Chip Design. Lecture Notes in Electrical Engineering. Volume 265, 2014, pp 201-221. Springer, 2013. [download pdf]
%
%
%D. Shah, E. Hung, C. Wolf, S. Bazanski, D. Gisselquist, and M. Milanovic. Yosys + nextpnr: an Open Source Framework from Verilog to Bitstream for Commercial FPGAs. In 2019 IEEE 27th Annual International Symposium on Field-Programmable Custom Computing Machines (FCCM). IEEE, 2019. [arXiv]
%
%Stratefied synthesis
%
%stoke
%
%Just-in-Time Compilation for Verilog
%
%Compiler-Driven FPGA Virtualization with SYNERGY
%
%FPGA Interchange format to enable interoperable FPGA tooling
%https://opensource.googleblog.com/2022/02/FPGA%20Interchange%20format%20to%20enable%20interoperable%20FPGA%20tooling.html
%
%Hashing Modulo Alpha-Equivalence






% Accelerators and parallel architectures 
%   present many opportunities 
%   for tuning and improving tensor operator implementations for the best performance.
% Many systems, 
%   including deep learning frameworks like PyTorch~\cite{pytorch},
%   make extensive use of hand-optimized tensor operator implementations
%   (such as those in the CuDNN library~\cite{chetlur2014cudnn}).
% While these hand-optimized implementations
%   achieve strong performance,
%   various systems, including \g,
%   have been proposed to automatically
%   generate optimized tensor operators
%   to reduce development time,
%   support varied hardware platforms,
%   and avoid reliance on a small number of experts.
% These tensor compilers 
%   rely on specifying tensor computations 
%   in a form that allows for
%   conveniently exploring options for optimizations, 
%   such as by changing loop orderings
%   to best utilize caches.

% \hl{Surely there's a better summary/gloss here.}
% Many tensor operator compilers 
%   use index notation
%   to specify tensor operators
%   (defining how each element of the output
%   is to be computed
%   based on corresponding elements 
%   of the input).
% TACO~\cite{taco} uses index notation 
%   for automatically generating and optimzing both sparse and dense tensor computations,
%   permitting particular dimensions 
%   to be specified as dense or sparse,
%   introducing various structures for reasoning about how 
%   to iterate over sparse dimensions.
% %Tensor operators in TACO
%   %are described using index notation, 
%   %with particular tensor dimensions 
%   %being either dense or sparse.
% %\cite{taco} initially 
%   %focused on compiling for CPU, 
%   %while subsequent work~\cite{senanayake2020}
%   %has extended TACO to target
%   %GPUs and vector units.
% %  is a compiler notable for its handling
% %  of computations over sparse tensors.
% %\hl{unsure how to draw any connection here, but i feel like i need to at least mention taco}
% Keops~\cite{keops} also uses
%   index notation to describe tensor operations
%   for both dense and spare matrices,
%   but introduces another matrix representation
%   called symbolic matrices, 
%   in which each element of the symbolic matrix
%   is computed from two smaller data matrices.
% Computations on symbolic matrices 
%   can more easily be deployed to GPUs and other accelerators 
%   than sparse computations
%   but require less data movement than dense computations.
% %% I think MLIR isn't relevant in this discussion: IRs built _in_ MLIR might be
% %MLIR~\cite{mlir} is a general-purpose compiler framework intended to facilitate the development of IRs.
% %While MLIR itself does not have a built-in notion of tensorization, it has been used to implement polyhedral IRs and other tensor operator representations.
% COMET~\cite{tian2021highperformance} is another
%   CPU-focused sparse tensor algebra IR,
%   implemented using MLIR~\cite{mlir},
%   that additionally uses information about sparse storage formats 
%   in its representation 
%   to increase temporal and spatial locality.

% Halide~\cite{ragan2013halide}
%   %while not a machine learning compiler
%   has been influential
%   in using a representation
%   that separates
%   an tensor operator's specification (what it computes)
%   from its schedule (what order elements are computed),
%   allowing many optimizations
%   to be described as different schedules
%   for the same specification
%   and facilitating operator fusion.
% As discussed in~\cite{newcomb2020halide-rewrite},
%   Halide applies a term rewriting system
%   for producing optimized code.
%   \hl{Any insight for why Halide is amenable to a rewrite system?}
% TVM~\cite{chen2018tvm}
%   uses a similar specification-schedule split
%   for describing its tensor operators.
% FireIron~\cite{hagedorn2020fireiron} is another system
%   using a split between a computation specification 
%   and its realization
%   (using a decompositions, rather than Halide-style schedules,
%   for scheduling parts in a top-down style).
% \g can be understood
%   as a further refinement
%   on an algorithm's specification,
%   disambiguating
%   how data is accessed
%   from the computation being performed
%   over the data,
%   enabling transformations
%   like mapping to hardware
%   before the program is scheduled.
%   \hl{What does it mean
%   that mapping to hardware
%   is done before the program is scheduled?}

% Like \g, several other systems 
%   use functional representations
%   of tensor operators.
% LIFT~\cite{lift}
%   separates specifications from schedules
%   using combinators like maps and reductions to specify schedules,
%   an idea further explored in~\cite{hagedorn2020func-high-perf}.
% \hl{anything else to say about LIFT? Contrast with Halide/TVM's scheduling languages?}
% Accelerate~\cite{accelerate} 
%   uses functional combinators 
%   to map Haskell code 
%   to GPU programming primitives.
% \hl{Discussion comparing these to \g?}

% The polyhedral representation~\cite{polyhedral-survey} 
%   has also proven useful
%   for expressing tensor operators.
% %Polyhedral compilation~\cite{polyhedral-survey}
%   %is a powerful alternative
%   %to term rewriting-based compilers.
% Polyhedral compilers optimize
%   loop-filled programs
%   by modeling loop nests
%   as polyhedra
%   and transforming them geometrically.
% Tensor Comprehensions~\cite{vasilache2018tensor}
%   and Tiramisu~\cite{tiramisu}
%   are examples of machine learning compilers
%   powered by the polyhedral framework.
% \hl{Need note about deploying to accelerators?}
% \hl{Implications for term rewriting?}
% Multidimensional homomorphisms~\cite{multidimensional-homomorphism} 
%   are another mathematical representation 
%   of tensor operations
%   that has been amenable to automatic parallelization 
%   and allows for hierarchical composition.
%   \hl{any comment in relation to \g?}

%There are at least as many
  %tensor IRs
  %as there are
  %deep learning frameworks,
  %and many frameworks
  %use more than one.
%TVM \cite{chen2018tvm},
  %for example,
  %uses the high-level
  %Relay IR~\cite{relay}
  %for optimizations
  %in the sequencing of tensor kernels,
  %while it uses low-level TIR
  %to optimize kernels themselves.
%\hl{If you're going to complain about TIR not being pure, you need to establish that purity is a requirement before this. Maybe discuss this later}
%Relay and TIR
  %are a perfect example
  %of our impedance mismatch problem:
  %Relay is pure but too high-level,
  %while
  %TIR is low-level but impure.


% Should we talk about BYOC here?
%Recently,
%  the Bring Your Own Codegen
%  (BYOC)
%  framework
%  was merged into TVM \cite{byoc}.
%BYOC
%  is novel,
%  as it allows for the 
%  fast implementation
%  of a full compiler
%  for deep learning models
%  down to custom hardware backends
%  with fairly little additional code,
%  assuming the users
%  have written a codegen
%  for their hardware
%  already.
%BYOC includes
%  a matching framework,
%  for matching
%  user-specified
%  patterns
%  of Relay code.
%As we will see
%  in Section \ref{sec:case-study-tensorization},
%  one of our primary case studies
%  of \g{}
%  is as a pattern matcher
%  for matching such computational patterns---%
%  in fact,
%  it was the original
%  intended use case
%  of \g{}!
%In some sense,
%  the two pattern matchers
%  are incomparable,
%  because,
%  as we've described above,
%  \g{}
%  and Relay
%  operate at different levels
%  of abstraction.
%Yet if we ignore the differences
%  in the levels of abstraction,
%  we can compare
%  the matchers
%  in how they operate.
%In this comparison,
%  \g{} shines through
%  with the help of
%  the \egr{}.
%Because rewrites
%  are so cheap and easy
%  within the \egr{},
%  we can run a huge number
%  of exploratory rewrites,
%  potentially finding places
%  to map in user-defined
%  patterns.
%BYOC,
%  on the other hand,
%  expects the user to provide
%  multiple equivalent patterns
%  to cover the numerous ways
%  their pattern might appear 
%  in the program
%  \hl{(verify this)}.

%Named tensors \cite{chiang2021named}
%  are a primary inspiration
%  for the access pattern data structure
%  at the core of \g.
%%Tensors have a specific layout
%%  in memory,
%%  a hardware detail
%%  that often bubbles up
%%  even to the highest levels
%%  of tensor abstractions.
%%For example,
%%  in both TVM and TensorFlow,
%%  the \tcd{conv2d} operator
%%  requires the user to specify
%%  the layout of the activation tensor---%
%%  \tcd{NCHW} or \tcd{NHWC},
%%  where \tcd{N} is the batch dimension,
%%  \tcd{C} is the channels dimension,
%%  and \tcd{H} and \tcd{W} are the spatial
%%  (height and width)
%%  dimensions.
%%Rather than pass layout information
%%  externally,
%%  named tensors
%%  incorporate dimension names
%%  directly into the tensor abstraction.
%%Named tensors
%%  acknowledge the fact
%%  that
%%  not all dimensions
%%  are made the same,
%%  and that different dimensions
%%  have different functions.
%Named tensors
%  assign names
%  to the dimensions of a tensor,
%  increasing code readability
%  and acknowledging that different dimensions
%  have different functions.
%Though
%  we do not actually adopt
%  this notation
%  in \g{}---%
%  the dimensions of tensors
%  are still just indexed
%  with integers---%
%  this core idea
%  is reflected
%  in the design
%  of access patterns,
%  which encode the fact that
%  some dimensions are
%  for
%  \textit{iterating over,}
%  while others are meant to be 
%  \textit{computed upon.}

%Many machine learning frameworks
  %have an optimization step
  %in which they match program patterns
  %to efficient low-level implementations,
  %whether that be offloading to hardware
  %or calling into a tuned library.
%TVM \cite{chen2018tvm}, 
%% Steve: I would say Latte is not very relevant here
%% It provides AD, but it requires the user to manually implement just about everything else
  %Latte \cite{latte},


%% Steven: Not clear it's relevant to this context
%Norman Ramsey instruction selection~\cite{dias2010instruction-selection}

%\hl{even further back:} apl?~\cite{apl-survey} % probably no

%\subsection{Term Rewriting, Equality Graphs, and Equality Saturation}

% {\color{red} \noindent\rule{8.5cm}{10pt}}

% \g utilizes
%   the power of equality saturation
%   in
%   low-level tensor program
%   transformation---%
%   namely, mapping programs
%   to custom hardware.
  
% Term rewriting
%   is a classic technique
%   in program optimization
%   in which rewrite rules of the form
%   $\ell \xrightarrow{} r$
%   are applied over a program.
% When an expression in the program
%   matches
%   the pattern $\ell$,
%   it is rewritten
%   into the pattern $r$.
% In classic term rewriting systems,
%   the ordering
%   in which rewrites are applied
%   can affect whether optimizations
%   are found,
%   as some rewrites
%   may reverse or muddle
%   the effects
%   of other rewrites.
% Equality saturation
%   is a technique
%   developed to sidestep
%   this 
%   phase ordering problem.
% The technique
%   has recently re-emerged
%   with the development
%   of the \tcd{egg} library
%   \cite{willsey2021egg},
%   and with the successful application
%   of equality saturation
%   to floating point optimization \cite{herbie}
%   and CAD program simplification \cite{szalinski},
%   among other varied fields.

% %A primary feature
% %  of equality saturation
% %  is its ability to
% %  efficiently store
% %  all previously discovered
% %  versions 
% %  of the program
% %  being transformed.
% %The data structure which enables this
% %  is the
% %  \textit{equality graph}
% %  (\egr),
% %  which resembles
% %  a standard program graph (\hl{not sure on words to use here?}),
% %  except
% %  each node in the program
% %  is replaced with a \textit{set} of nodes,
% %  called an \textit{equivalence class}
% %  or \textit{eclass.}
% %All nodes within an eclass
% %  are equivalent, and thus 
% %  can be substituted for one another
% %  to produce an equivalent program.
% %This property is only possible
% %  when the language used
% %  within the \egr
% %  is pure,
% %  which thus becomes a requirement
% %  for any language
% %  we'd like to transform
% %  with equality saturation.
  
% Diospyros \cite{vanhattum2021vectorization}
%   is a vectorizing compiler
%   for DSPs
%   which uses equality saturation
%   to match program fragments
%   to hardware primitives.
% Diospyros
%   starts from scalar programs
%   and, via symbolic evaluation
%   and equality saturation,
%   lifts them to vectorized
%   expressions,
%   while \g starts
%   from a higher level of abstraction
%   and searches downwards.
  
% SPORES \cite{wang2020spores}
%   and Tensat \cite{yang2021equality}
%   utilize equality saturation
%   to optimize
%   linear algebra expressions
%   and tensor computation graphs,
%   respectively.
% While both
%   show the potential
%   of equality saturation
%   for tensor program transformation,
%   both of their IRs
%   are too high-level
%   for the task of mapping to hardware.

% TODO mention somewhere in here that lambdas (which a lot of langs will use) are a problem for first-order rewrite systems


Chlorophyll~\cite{phothilimthana2014chlorophyll}
  is a prime example
  of how solvers can be used
  in compilers.
Chlorophyll
  uses Z3
  to compile programs
  for a unique
  architecture:
  an array of power-efficient
  processors.
It does so by
  expressingt he particular,
  architecture-specific concerns
  of code compilation
  as constraints
  to Z3.


==> text/motivating-example.tex <==
\section{Motivating Example: 8-bit Add}
\label{sec:motivating-example}


\begin{figure}
\begin{minted}{systemverilog}
module add8(input [7:0] a, b, output [7:0] y);
  assign y = a + b;
endmodule
\end{minted}
\caption{Behavioral SystemVerilog implementation of 8-bit add.}
\label{fig:8-bit-add-behavioral}
\end{figure}
  
\begin{table}
    \centering
    \begin{tabular}{c|ccc}
        & LUTs & CARRY8s & Datapath Delay (ns)  \\
        \hline
         first attempt& 11 & 0 & {\color{red}{0.799}}  \\
         second attempt& 8 & 1&  {\color{OliveGreen}{0.410}}  \\
    \end{tabular}
    \caption{Vector add statistics}
    \label{tab:vector-add-stats}
\end{table}
  
\begin{figure}
\begin{minted}{systemverilog}
module add8(input [7:0] a, b, output [7:0] y);
  impl _impl (a, b, y);
endmodule

module impl(input [7:0] a, b, output [7:0] y);
  wire [7:0] p;
  LUT2 #(.INIT(4'h6)) l0 (a[0], b[0], p[0]);
  // ...7 LUT2s omitted...
  CARRY8 carry0 (.CI(1'b0), .DI(a), .S(p), .O(y));
endmodule
\end{minted}
\caption{Structural Xilinx UltraScale+ SystemVerilog implementation of 8-bit add.}
\label{fig:8-bit-add-structural}
\end{figure}

To motivate the use
  of solver-aided programming
  to generate ISA instruction implementations,
  let's walk through an example
  of implementing an 8-bit add instruction
  for Xilinx UltraScale+ FPGAs.
As a first pass,
  we will attempt to 
  generate an UltraScale+ implementation
  of 8-bit add
  using the traditional flow.
In the traditional flow, we start with 
  a high-level,
  behavioral SystemVerilog implementation
  of 8-bit add,
  shown in \cref{fig:8-bit-add-behavioral},
  and use Xilinx'x Vivado toolchain
  to synthesize%
  \footnote{Note that we use the term ``synthesis'' here to specifically represent the step in traditional hardware compiler flows in which the design is compiled into logic gates, optimized, and then mapped to FPGA primitives.}
  , place, and route the design
  for an UltraScale+ board.

The result,
  recorded in the first row of
  \cref{tab:vector-add-stats},
  uses 11 LUTs,
  and has a datapath delay of 0.799ns.
At first glance,
  this may seem just fine.
However, those familiar with
  Xilinx FPGAs
  will notice that the implementation
  doesn't use a single CARRY8---%
  a specialized fast carry chain unit
  designed specifically for speeding up
  addition.
Noticing that,
  we attempt a more brute-force implementation,
  shown in
  \cref{fig:8-bit-add-structural}.
In this implementation,
  we manually implement the 8-bit addition
  using the UltraScale+ primitives
  \texttt{LUT2} and \texttt{CARRY8}.
This requires more intimate
  knowledge of the FPGA backend.
In the first place, we need to know
  the FPGA contains
  specialized carry logic.
Knowing that,
  we are then required to connect the wires by hand,
  and to determine the \texttt{INIT}
  values for the LUTs.
But our effort pays off:
  when we synthesize, place, and route
  our new implementation,
  the resulting design
  has a datapath delay of
  0.410ns---an improvement of nearly 2x!
  
This example clearly illustrates the problem:
  even on simple designs---indeed,
  just a single 8-bit add,
  traditional hardware compilers behave
  in unexpected ways,
  and users need backend-specific knowledge
  to extract maximum performance.
Note that we can also recover the performance
  of our behavioral implementation
  by explicitly clocking the result of
  \texttt{a + b}
  into a register, using an
  \texttt{always_ff}
  block,
  but an inexperienced user is unlikely
  to figure this out
  without first scouring the internet
  for help.
Furthermore,
  whether or not a design uses a register
  is irrelevant
  to the carry;
  this gives a clear example of the
  underlying heuristics
  producing unexpected results.




==> text/old-intro-dont-use-it.tex <==
\section{Introduction}
\label{sec:intro}

\input{figures/firstpage}

Given a high-level hardware design specification
  (e.g., expressed in behavioral Verilog),
  FPGA technology mappers
  search for an equivalent
  low-level implementation
  in terms of the target FPGA's
  primitives.
Recent trends in \textbf{FPGA heterogeneity}---%
  the inclusion of increasingly specialized and diverse primitive elements on FPGAs---%
  have made effective
  technology mapping
  crucial for achieving
  high performance~\cite{vega2021reticle}.
  % possibly relevant cite: zhu2022fpgaheterogeneity

Historically,
  FPGA compute primitives
  consisted primarily of
  generic, homogeneous 
  lookup tables (LUTs) and carry chains.
Automated tools like 
  ABC~\cite{ABC,abc2,brayton2010abc}
  can efficiently map such basic primitives
  by translating \asplos{hardware} designs
  to a library of simple logic gates
  and then packing those gates
  into LUTs.

No comparable
  automatic solution supports
  the wide array of increasingly diverse, highly configurable
  specialized units like digital signal processors (DSPs)
  in modern FPGAs.
For example, Xilinx's DSP48E2
  is a multifunction DSP with over
  100 ports and parameters which
  allow it to
  support a large variety of computations.
  However, this also presents a large search space
  for technology mappers,
  making it challenging
  to correctly configure the primitive
  while also satisfying complex restrictions and dependencies.
% Configuring even a single DSP48E2 is difficult:
%   implementing a given design fragment $D$
%   requires constructing a large configuration
%   that sets each DSP port and parameter
%   to simulate $D$ while also
%   satisfying complex restrictions and dependencies.

Current technology mappers search for such
  configurations via ad hoc, handwritten procedures.
These procedures do not provide strong correctness guarantees;
  recent work highlights the significant number of bugs found across 
  all major hardware synthesis tools~\cite{herklotz2020finding}.
These procedures are difficult to extend;
  \textit{each} new complex primitive requires
  supporting detailed semantics\footnote{
      The Xilinx manual for the DSP48E2 alone
      is over 75 pages long.}
  and adding hundreds of new, special-case
  syntactic pattern matching rules~\cite{wolf2013yosys}.
Finally, these procedures are incomplete;
  they miss many mapping opportunities,
  even across microbenchmarks based on vendor documentation.
\cref{fig:firstpage} (above) shows a
  simple example design consisting of
  \verb-+-, \verb-*-, and \verb-&-,
  which \textit{should} fit on a single DSP48E2,
  but is instead mapped to multiple DSPs and LUTs
  by current state-of-the-art tools.\footnote{
    Licensing restrictions forbid naming the
    specific proprietary tools, but they are familiar,
    standard packages used by many hardware designers.
  }\tighten
  
Our key observation is that
  the configuration space for
  each kind of FPGA primitive
  essentially serves as a small, bespoke
  \textit{programming language}
  that must be used
  to map design fragments
  down to those low-level primitives.
% From this perspective,
%   mapping an HDL design fragment $D$ down to
%   target FPGA-specific primitives
%   reduces to searching for programs
%   (configurations) of the available
%   primitives that are equivalent to $D$.
This paper explores how
  \textit{program synthesis}~\cite{gulwani2017program}
  can be applied to
  simplify the design and implementation of
  FPGA technology mappers while providing
  \textbf{correct},
  \textbf{extensible}, and
  \textbf{more complete}
  support for diverse, highly configurable primitives
  like DSPs.

Program synthesis techniques rely on
  automated theorem provers like
  SAT and SMT solvers~\cite{de2008z3, barbosa22cvc5}
  to automatically generate programs
  satisfying a given specification.
We demonstrate how
  sketch-guided program synthesis~\cite{solar2008program}
  can be adapted
  for FPGA technology mapping:
  given a specification as a
  design fragment $D$ expressed in behavioral HDL,
  we use the Rosette~\cite{torlak2014lightweight} program synthesis framework embedded in the Racket language
  to efficiently search for
  configurations of
  low-level, FPGA-specific primitives,
  i.e., programs in structural HDL
  that implement $D$.\tighten

% We developed two new techniques to enable
%   building correct, extensible, and more-complete
%   FPGA technology mappers
%   via program synthesis:
%   (1) \textbf{semantics extraction from HDL}
%       to provide mostly-automated encoding of the
%       programming language and semantics
%       for each kind of FPGA primitive, and
%   (2) \textbf{architecture-independent sketch templates}
%       to encode generic, high-level implementation strategies
%       that efficiently map design fragments across
%       multiple FPGA architectures.

Sketch-guided program synthesis requires
  encoding the \textit{semantics}
  of the target language:
  in our case,
  a machine-readable,
  mathematical model specifying
  the behavior of each
  FPGA-specific primitive
  being mapped to.
In a typical synthesis tool,
  which generates programs
  for a single target language,
  this is a one-time cost.
However,
  in our setting,
  each new FPGA primitive
  introduces yet another new target language,
  which in turn requires
  extending the tool to encode
  yet another formal semantics.

To support
  \textit{extensible} and \textit{correct}
  technology mapping, we propose
  automating this process with
  \textbf{semantics extraction from HDL}, 
  adapted from past work~\cite{daly2022synthesizing},
  to automatically extract
  complete primitive semantics
  from vendor-published HDL models
  (\cref{fig:firstpage}, ``input 2'').
Traditionally, such models have
   only been used
  for simulation and validation;
  we show that using them for
  target language semantics within a
  program-synthesis-based approach
  yields substantially more
  \textit{complete} FPGA technology mapping.

Sketch-guided program synthesis also
  requires \textit{sketches},
  partially complete programs with ``holes'' to be filled in
  by the solver.
Sketches primarily serve to
  scale synthesis by
  constraining the set of programs that 
  solvers explore when searching for
  one that satisfies
  the given specification,
  i.e., performance at the cost of completeness.
In our setting,
  sketches correspond to
  primitive configurations with
  holes for the port and parameter settings.
The synthesizer will ``fill in the holes''
  as necessary for
  the low-level FPGA-specific primitive to implement
  a given high-level behavioral design fragment.
Unfortunately,
  developing effective sketches
  still requires synthesis expertise~\cite{10.1145/3140587.3062353,vanGeffenJITSynth}.
  Naively, our approach would also
  require new sketches for each new
  FPGA primitive we want to target.


% %Naively, both obtaining
%   %semantics and
%   %writing sketches would
%   %hamper a program synthesis
%   %approach to technology mapping.
% At first glance,
%   obtaining semantics
%   and writing sketches
%   would appear to be difficult
%   manual steps
%   that would impede the use of program synthesis
%   and negating any benefits of automation.
% (Incidentally, current
%   technology mappers also manually
%   specify the semantics
%   via 
%   their unstructured hand-written 
%   patterns and procedures.)
% % Current technology mappers only
% %   reason about primitive semantics
% %   in the unstructured hand-written 
% %   procedures,
% %   and requiring users
% %   to provide sketches
% %   would hamper extensibility, 
% %   as sketches require primitive-specific details
% %   that would negate the automation benefit
% %   of such an approach. 
% However, we apply two key insights
%   to make this approach practical.

 
To address this challenge, 
  we introduce
  \textbf{architecture-independent sketch templates.}
% There are a few common classes 
%   of
%   FPGA primitives
%   present across most architectures:
%   LUTs, carry chains, muxes, and DSPs.
Hardware designs are often implemented
  using similar high-level blueprints
  across most FPGA architectures---%
  sketch templates
  capture these blueprints
  and make them reusable across architectures.
Using sketch templates, we
  greatly reduce the overhead of supporting
  new architectures and
  diverse primitives.
Typically, when adding
  a new primitive, the user
  does not need to write or modify
  any sketch templates.


% However,
%   FPGA primitives across architectures
%   fall into a few common classes, e.g.,
%   LUTs, carry chains, and DSPs, and
%   the way these primitives
%   are used to implement designs
%   is similar across architectures.
% Hence, we introduce abstractions
%   to capture these similarities to build
%   \textbf{architecture-independent
%   sketch templates},
%   reducing the effort required to
%   support a new primitive.



We leveraged these techniques---%
  semantics extraction
  from HDL
  and architecture-independent
  sketch templates---%
  in \lr\footnote{
    \lr is open source and available at
    \textbf{link redacted for anonymity}.
  }, a new FPGA technology mapper
  based on program synthesis.
\lr's prototype implementation automatically
  imports semantics for the LUTs, arithmetic carry chains,
  and DSPs of the Xilinx UltraScale+, Lattice ECP5,
  %Intel MAX,
  and SOFA~\cite{sofa} FPGA architectures. 
The only additional user input to \lr is a short
  architecture description
  %between 20 and 300 source lines 
  %of code,
  which lists the target FPGA's
  primitives.
With the automatically
  extracted primitive semantics
  and the user-provided architecture description,
  we demonstrate that \lr
  is more complete than proprietary tools on a variety
  of microbenchmarks,
  each of which should fit on a single DSP.
In particular,
  we map up to 40$\times$ 
  more designs to 
  DSPs than Yosys, 
  and 1.9--2.7$\times$ 
  more designs than 
  state-of-the-art
  tools for Xilinx and Lattice.\looseness=-1
% We further show the practical applicability
%   of \lr
%   in real-world applications
%   by integrating it into the open-source
%   hardware synthesis tool
%   Yosys~\cite{wolf2013yosys}.

\vspace{1ex}
\noindent
This paper provides 
the following key contributions:
\begin{itemize}
\item A technique for applying
  \textit{semantics extraction from HDL}
  for extensible,
  program synthesis-based
  technology mapping.
\item A design for
  \textit{architecture-independent
  sketch templates.}
\item A language to capture hardware design sketches.
% \item Formal semantics
%   languages for combinational and sequential logic, 
\item A formalization of the \lr
  toolchain, and an argument
  for its correctness as well as
  its completeness modulo sketches.
\item Empirical comparisons of
  \lr and existing hardware synthesis
  tools to evaluate both their
  relative completeness and
  ease of extensibility.


  
% \item The \lr prototype toolchain for
%   practical FPGA technology mapping 
%   via program synthesis.


% \item An evaluation of \lr mapping
%     primitives on Xilinx, Lattice, Intel,
%     and SOFA
%     FPGAs.

\end{itemize}

The rest of this paper is organized as follows.
In \cref{sec:overview},
  we give an overview
  of \lr's design and key features.
In \cref{sec:formalization},
  we formalize \lr and
  demonstrate its correctness.
In \cref{sec:implementation}
  we discuss \lr's implementation.
In \cref{sec:evaluation}
  we evaluate \lr on its
  completeness of mapping,
  extensibility,
  and expressiveness.
  % terms of
  % effort to synthesize technology mappers
  % and the quality of the generated FPGA
  % implementations.
\cref{sec:background-and-related-work}
  discusses related work, and
  \cref{sec:conclusion} concludes.
  


%Modern architectures have traditional 
  %primitives like lookup tables (LUTs) and carry chains,
  %as well as an increasingly diverse array of specialized,
  %highly configurable units like digital signal processors
  %(DSPs).
% In modern FPGAs, types of primitives include
%   both traditional units like
%     lookup tables (LUTs) and  carry chains,
%   as well as an increasingly diverse array of
%     specialized, highly configurable units like
%     digital signal processors (DSPs). 
% For these traditional units, automated tools like 
%     ABC~\cite{ABC,abc2,brayton2010abc}
%     can achieve high-quality mapping results
%     in the context of
%     homogeneous
%     FPGAs (consisting only of
%     LUTs)
%     by efficiently mapping designs
%     to a library of simple logic gates
%     and then packing those gates
%     into LUTs.
% Today's specialized primitives are highly complex
%   and sophisticated, requiring significant knowledge
%   of their behavior to use effectively.


% \hline
% 
% % What is technology mapping
% Technology mapping
%   is one step
%   in the process of mapping
%   a hardware design
%   onto an FPGA.
% During technology mapping,
%   FPGA synthesis tools
%   determine how to implement
%   the high-level description
%   of the design
%   using an FPGA platform's
%   specific primitives.
% To compile designs effectively,
%   it is critical that technology mappers
%   utilize all available types of primitives
%   on an architecture, e.g.,
%   lookup tables (LUTs),
%   carry chains, and
%   digital signal processors (DSPs).
%  
% % Technology mapping is difficult to implement.
% Technology mapping is difficult to implement.
% % What can we say in the general case? We don't know how it's implemented in Vivado, Diamond.
% Generally, technology mappers
%   apply a combination of
%   low-level,
%   automated search
%   and
%   high-level, hand-written
%   pattern matching
%   to explore potential mappings
%   of designs to primitives.
% For example,
%   the Yosys synthesis suite~\cite{wolf2013yosys}
%   utilizes the logic synthesis tool ABC~\cite{abc}
%   automatically map hardware designs
%   to simple gates with concrete semantics,
%   such as \texttt{AND}, \texttt{OR},
%   and \texttt{NOT},
% % Is conversion to LUTs special-cased?
% % See https://people.eecs.berkeley.edu/~alanmi/abc/
%   and then packs those gates
%   into look-up tables (LUTs).
% Though this process is automatic,
%   it is limited to simple primitives.
% 
% % Increasing heterogeneity is good, dsps are good
% To increase performance
%   and decrease power,
%   FPGAs are becoming increasingly heterogeneous.
% While originally FPGAs were homogeneous arrays
%   of LUTs,
%   FPGAs now include primitives
%   specialized for common task,
%   such as arithmetic carry chains.
% Beyond specialized combinational logic,
%   increasingly FPGAs include
%   \textit{digital signal processors}
%   (DSPs):
%   complex programmable primitives with a
%   wide range of potential behavior.
% When utilized correctly,
%   DSPs significantly boost the performance
%   of compiled hardware designs.
% 
% % but Increasing heterogeneity makes techmapping harder
% While heterogeneity
%   gives hardware designers access
%   to specialized primitives,
%   it also increases the difficulty
%   of technology mapping.
% Each new primitive
%   must be supported
%   in the current technology mapping solution.
% This requires
%   
% Cite RapidWright~\cite{lavin2018rapidwright}
% 
% % This needs to be broken into multiple paragraphs:
% % - What is sketch-guided program synthesis
% % - Sketch-guided program synthesis is usually used in constrained cases. Previously, FPGA technology mapping was not constrained, i.e. one big search with ABC. however, new compilers break the problem down into instructions. Program synthesis now becomes feasible.
% % - Uses sketches capture useful, general patterns and constrain search (in contrast to ABC and other techniques?)
% % - But requires semantics to work
% 
% % Semantics are already available in vendor provided models! We extract them, even for large, 1000+ line Verilog models of DSPs
% 
% 
% % Our tool lakeroad encapsulates all of these techniques
% 
% % our results
% 
% %
% 
% 
% \hline
% 
% %Powerful FPGA synthesis tools
% %  are critical
% %  in the hardware design process.
% FPGA synthesis tools
%   enable hardware designers
%   to be productive.
% Rather than needing to write
%   low-level, FPGA-specific
%   HDL 
%   (hardware description language)
%   code,
%   a hardware designer is instead
%   able to write
%   high-level,
%   architecture-independent
%   HDL,
%   which the synthesis tool
%   will compile into a low-level implementation
%   which efficiently uses
%   the FPGA's resources.
% 
% Synthesis tools
%   are massive engineering projects.
% Many of the best tools---%
%   such as Xilinx's Vivado~\cite{vivado}
%   and Lattice's Diamond~\cref{diamond}---%
%   are developed by teams of many engineers
%   at large FPGA companies.
% Yosys~\cite{wolf2013yosys},
%   an open-source FPGA synthesis tool,
%   has over 11,000 commits
%   representing contributions 
%   from nearly 200 people.
% 
% One of the biggest hurdles
%   in building synthesis tools
%   is in supporting new FPGA architectures.
% Not only does this require experties
%   in the synthesis tool itself,
%   but it also requires knowledge
%   of the underlying FPGA architecture.
% Each architecture can add 
% 
%   which can be a high bar 
%   especially
%   for developers
%   of open-source FPGA synthesis tools.
%   
% To reduce some of the implementation burden,
%   FPGA synthesis tools rely on
%   \textit{technology mapping}
%   tools 
%   %such as ABC
%   to automatically, 
%   flexibly map designs
%   to 
%   FPGA-specific primitives.
% Traditionally, however,
%   technology mapping has been limited to small, 
%   fixed-function primitives, 
%   and does not support large programmable units like DSPs.
% %  
% In this paper,
%   we present a new method of technology mapping
%   which can utilize
%   all primitives available on an FPGA architecture---%
%   not just LUTs, but carries and even DSPs.
% Our method utilizes
%   \textit{sketch-guided program synthesis}
%   and \textit{semantics extraction from HDL}
%   to determine the behavior
%   of FPGA primitives automatically.
% Our method requires little user input,
%   and integrates into and enhances 
%   existing FPGA synthesis approaches.
% 
% 
% \hl{make it clear up front that we're doing tech mapping, not placement}
% 
% \hl{we need to put the comparison-on-carry trick somewhere}
% 
% Field-programmable gate arrays (FPGAs)
%   are a popular platform
%   for developing custom hardware
%   due to their
%   performance,
%   affordability,
%   and reprogrammability.
%  FPGA technology
%   continues to advance, with
%   FPGAs becoming increasingly
%   complex.
% Whereas early FPGAs
%   were homogeneous arrays of 
%   \textit{lookup tables} (LUTs)---%
%   configurable memory devices that can be programmed
%   to implement bitvector functions ---%
%   modern FPGAs are 
%   heterogeneous,
%   containing
%   increasingly complex
%   specialized units
%   such as dedicated
%   carry chains
%   and digital signal processors (DSPs).
%   
% Though FPGA hardware has advanced,
%   their software toolchains have not, and legacy toolchains
%   struggle to support modern heterogeneous
%   FPGAs~\cite{lavin2018rapidwright}.
% %
% Legacy toolchains use \textit{hardware synthesis}---a complex process
% that attempts to infer high-level structure (e.g., a pipelined multiplier)
% from a low-level representation (e.g., an and-inverter graph).
% %
% Hardware synthesis is at the root of legacy toolchains'
% struggle or outright inability to utilize
% specialized units of modern FPGAs.
% 
% Legacy toolchains struggle to utilize specialized units on FPGAs
%   because their approach to \textit{hardware synthesis}
%   attempts to translate input programs to FPGA designs in
%   ``one big step''.
% Such tools attempt to automatically infer high-level structure---%
%   such as an entire pipelined multiplier---%
%   from a low-level representation---%
%   such as an and--inverter graph---%
%   via heuristics which have not scaled well
%   as FPGA heterogeneity increases.
% 
% % At the root of 
% %  legacy toolchains' difficulty
% %  in utilizing specialized units
% %  is
% %  the tools' use of
% %  \textit{hardware synthesis,}
% %  a complex process which attempts to infer
% %  high-level structure---%
% %  such as an entire pipelined multiplier---%
% %  from a low-level representation---%
% %  such as an and--inverter graph---%
% %  via a brittle process of pattern matching.
% 
% 
% In contrast,
%   software compilers typically generate
%   their output by progressively lowering
%   source-level code down to machine-level code via
%   a sequence of semantics-preserving transformations.
% Several recent hardware compilers designed to target FPGAs
%   have also adopted such a progressive lowering strategy~\cite{
%     vega2021reticle, nigam2021compiler, circt}.
% As in traditional compilers,
%   the lowest-level IR in these compilers must be transformed into
%   output code by an target-specific backend,
%   e.g., to target a Xilinx UltraScale+ FPGA,
%   such compilers would need a pass that translates
%   the lowest-level hardware-agnostic intermediate representation (IR)
%   into UltraScale+ specific HDL code.
% 
% 
% Compared to traditional hardware synthesis,
%   progressive compilation facilitates
%   mapping high-level expressions down to
%   complex FPGA components by preserving
%   high-level structure until late in the
%   compilation pipeline.
% In contrast, traditional synthesis
%   translates entire designs into
%   graphs of gates, thus losing high-level information.
%   (TODO PATCH UP THIS PARA)
% 
% 
% % Recently,~\citet{vega2021reticle} introduced Reticle,
% %   a compiler for FPGA designs,
% %   which replaces hardware synthesis with
% %   \textit{progressive lowering compilation.}
% % In this style of compilation,
% %   FPGA hardware designs are lowered gradually
% %   from high-level (e.g., Verilog) to low-level (e.g., LUT and DSP configurations),
% %   inferring hardware primitives along the way.
% % This allows high-level expressions
% %   with complex low-level implementations
% %   (such as multiplies)
% %   to be discovered and mapped to specialized hardware
% %   more easily.
% 
% % Software compilers typically generate
% %   their output by progressively lowering
% %   source-level code down to machine-level code via
% %   a sequence of semantics-preserving transformations.
% % Several recent hardware compilers designed to target FPGAs
% %   have also adopted such a progressive lowering strategy~\cite{
% %     vega2021reticle, nigam2021compiler, circt}.
% % As in traditional compilers,
% %   the lowest-level IR must be transformed into
% %   output code by an target-specific backend,
% %   e.g., to target a Xilinx UltraScale+ FPGA,
% %   such compilers would need a pass that translates
% %   the lowest-level hardware-agnostic intermediate representation (IR)
% %   into an UltraScale+ specific HDL code.
% 
% 
% % Progressive lowering compilers
% %   transform programs to a target lowest-level representation
% %   often called the instruction set architecture or ISA.
% % Building a progressive lowering compiler
% %   requires a well-defined 
% %   lowest level of representation,
% %   often called the
% %   \textit{instruction set architecture (ISA)},
% %   to which a design should be lowered.
% % Several recent compilers designed to target FPGAs
% %   adopt a progressive lowering strategy.
% % As in traditional compilers,
% %   the lowest-level IR must be transformed into
% %   output code by an target-specific backend.
% 
% % This low-level IR
% %   must be then compiled to FPGA-specific code
% %   for each FPGA backend the compiler targets.
% % This has problems x y z...
%   
%   \hl{Ben: the following disembodied hunk seems left over from an edit}
%   several recent compilers for FPGAs
%   released in the past five years 
%   are designed
%   
%   include
%   an ISA at the core of their design.
% For example, the ISAs of
%   Reticle~\cite{vega2021reticle},
%   Calyx~\cite{nigam2021compiler},
%   and the MLIR CIRCT project~\cite{circt}
%   are composed of
%   logic instructions such as \texttt{and} and \texttt{or},
%   arithmetic instructions such as \texttt{add} and \texttt{sub},
%   and other instructions such as
%   \texttt{mux} and shifts.
%  
% Modern FPGA compilers use one
%   of two approaches to implement
%   their ISAs, and each of these
%   approaches have their own
%   limitations.
% The first method,
%   used by Calyx and MLIR CIRCT,
%   generates high-level
%   \textit{behavioral Verilog},
%   and then relies on traditional
%   hardware synthesis
%   for compilation.
% This approach loses
%   many of the benefits
%   we gain
%   from switching to
%   progressive lowering-based compilation.
%   
% The second method,
%   used by Reticle,
%   implements
%   the ISA for each backend manually
%   by providing a low-level
%   \textit{structural Verilog}
%   implementation
%   of each instruction
%   in terms of the specific FPGA's
%   primitives (e.g.~LUTs, DSPs, and carry chains).
% This method retains the
%   benefits of progressive
%   lowering compilation lost
%   by the first method, but
%   currently requires a hand-written
%   ISA which does not scale:
%   as the number of ISA instructions 
%   and the number of FPGA backends grow
%   (e.g., as we consider fusions of instructions,
%   or instructions specialized with constant values)
%   it becomes infeasible to implement
%   each instruction
%   for each backend.
% Implementing low-level ISAs by hand
%   can also lead to bugs,
%   especially on FPGA architectures
%   with complicated hardware primitives
%   such as DSPs.
% Additionally,
%   implementing ISAs by hand
%   requires expertise,
%   and as FPGAs become more heterogeneous,
%   implementers may miss
%   crucial opportunities
%   to utilize all available specialized units---%
%   for example, utilizing arithmetic carry chains
%   to implement non-arithmetic functions
%   such as comparisons~\cite{todo} % there are two citations for this.
% \hl{This point might motivate us needing
% to implement more than one version of an ISA, and this
% can be used to argue that implementin by hand is
% not scalable. Is there a way to put this before
% that point?}
% Finally,
%   this approach locks in a single instruction implementation
%   for the entire compiler,
%   but different optimization goals
%   (e.g.~design latency vs design area) might require different implementations.
%   
% 
% Implementing FPGA ISAs is an ideal use case
%   for sketch-guided program synthesis---%
%   a technique that
%   uses an SMT solver
%   to fill in holes
%   in \textit{program sketches}.
% Generally, sketch-guided program synthesis
%   performs best
%   when the domain 
%   is finite and loop-free,
%   and the program being synthesized
%   is small.
% FPGA ISA instruction implementations
%   fit this description.
% Their domain is the domain of bitvectors,
%   which SMT solvers reason about
%   efficiently.
% Furthermore, an instruction implementation
%   will be small and simple,
%   generally composing just a few FPGA primitives
%   to implement the requested instruction.
% 
% \hl{Ben: I'm gonna take another stab at these paragraphs, but I'm leaving
% the original in}
% While the domain of implementing FPGA ISAs
%   is an ideal application for sketch-guided
%   program synthesis, program synthesis
%   requires the user to provide the
%   semantics of the target
%   language---in our case, the semantics
%   of the target FPGA's primitives.
% Generally users of program synthesis
%   have to provide these semantics by
%   hand-writing an interpreter for their
%   domain.
% This would be too much work to ask of end users,
%    and we avoid this by automatically generating
%    interpreters for FPGA primitives from
%    vendor-provided Verilog simulation models
%    of the primitives.
% 
% \hl{original version}
% However, program synthesis
%   requires the user to provide
%   the semantics of the target language---%
%   in our case, the language of hardware design.
% Generally, users of program synthesis
%   provide these semantics
%   by writing an interpreter
%   for their domain.
% However, FPGA vendors release
%   Verilog simulation models
%   of their FPGAs' primitives;
%   these simulation models provide
%   exact semantics for the primitives.
% We need only to make these semantics
%   available to the program synthesis tool
%   to be able to do synthesis for a given FPGA.
% \hl{end original}
% 
% 
% In this work
%   we use sketch-guided program synthesis
%   to synthesize ISA implementations
%   for different FPGA backends.
% To represent sketches,
%   we present 
%   a domain-specific language,
%   \lrir,
%   with two levels of abstraction:
%   an architecture-independent level
%   of \textit{sketch templates,}
%   which capture abstractions
%   common among many FPGAs,
%   and an architecture-specific level.
% Furthermore,
%   we demonstrate how to automatically extract
%   the
%   semantics
%   of architecture-specific FPGA primitives
%   necessary for program synthesis
%   directly from the Verilog models
%   released by hardware vendors.
% \lr is fast \hl{insert some result} and
%   its outputs are correct by construction:
%   we provide a formalization of \lr
%   and argue for its correctness.
% \lr also allows users to explore
%   tradeoffs between instruction implementations
%   by discovering multiple implementations
%   for a given instruction.
% Lastly, \lr
%   can enable support for new architectures
%   with little effort from the end user.
%   \hl{should emphasize this way more}
%   
%   
% % For framing the contributions
% % https://www.cs.tufts.edu/~nr/pubs/tiler.pdf
% %https://theory.stanford.edu/~aiken/publications/papers/pldi16a.pdf
% %https://pp.ipd.kit.edu/uploads/publikationen/buchwald18cgo.pdf
% 
%   
% %Through our work,
%   %we also seek to demonstrate our thesis
%   %that compilation
%   %should originate
%   %from the semantics of hardware---%
%   %semantics which are formally captured
%   %in many forms today,
%   %such as in Verilog implementations of the design.
% %
% %Furthermore, beyond our tool,
%   %we propose a fundamental shift
%   %in how the field thinks about
%   %hardware design.
% %Namely, we demonstrate that
%   %\textit{formal hardware models}
%   %of a hardware platform's primitives
%   %are useful for more than
%   %validation or verification
%   %of human-made designs---%
%   %they can in fact be used
%   %to build automated reasoning tools
%   %which design hardware automatically.
% %In this paper,
%   %we present our first demonstration of this idea
%   %in the limited scope of FPGAs,
%   %as FPGAs are well-established
%   %and FPGA vendors generally release
%   %Verilog models of their architectures.
% %However, 
%   %we believe this idea extends to
%   %\textit{any} hardware platform
%   %whose primitive blocks
%   %are modeled formally.
% 
% Concretely, our contributions are:
% \begin{itemize}
% \item The conceptual insight that sketch-based program synthesis
%   can be used to implement
%   FPGA ISAs.
%   
% \item A two-level domain-specific language, \lr.
% 
% \item Sketches implemented in \lr
%   which capture design patterns
%   common across multiple FPGA platforms.
% These sketches are sufficient for synthesizing entire ISA
%   implementations
%   on new FPGA architectures.
%   
% \item A framework which allows users
%   to easily generate new
%   architecture-independent
%   or
%   architecture-specific sketches.
% 
% \item A method for extracting hardware semantics directly from
%   Verilog simulation files
%   provided by FPGA vendors,
%   and an open-source implementation
%   of the method.
%   
% \item An abstraction which allows
%   the semantics of stateful designs
%   to be represented in SMTLib-like syntax.
% 
% 
% \item An evaluation of Lakeroad, including
%   \begin{enumerate}
%       \item A per instruction quantiatative analysis of our ISA for Xilinx Ultrascale+, Lattice ECP5, and SOFA\cite{sofa}.
%       \item A demonstration of integrating \lr-generated instructions into multiple external frameworks (Calyx and MLIR CIRCT).
%       \item A case study, demonstrating the ability of \lr to generate implementations for 
%         SOFA, an FPGA architecture
%         otherwise unsupported
%         by most hardware compilers.
%   \end{enumerate}
%   
% \item A functional, open-source, and documented implementation of the tool, available on GitHub.
% \end{itemize}
% %
% %\hl{A key part of the story: FPGAs are going to keep getting more diverse. See recent Google work (FPGA22, HPCA? talk to luis, see slack) about Google's work on new FPGAs}
% 
% % \hl{end intro from Generals}
% 
% % \hl{luis begin}
% % 
% % There is an increasing number of domain-specific languages and compiler
% % infrastructure built for the purpose of describing hardware more efficiently,
% % including calyx, llhd, circt, etc. (add more information about these languages here)
% % 
% % All of these languages use behavioral Verilog as a low-level IR, which in turn can be used for both programming FPGAs and designing ASICs.
% % 
% % Nevertheless, behavioral Verilog is known to be inefficient for programming modern
% % FPGAs, requiring programmers to write brittle low-level and target-dependent implementations to unleash the maximum potential of these architectures.
% % Interestingly, some recent work (reticle) has shown a new approach to program
% % modern FPGAs using software compiler techniques, based on instruction selection,
% % leading to faster compilation times at expense of resource utilization in some
% % cases.
% % 
% % Sadly, one challenge of this work is that the target description or rewrite rules,
% % used by the instruction selector, are written by hand which it is error-prone and
% % limits the number of architectures that can be supported over time. The main goal
% % of an intermediate representation is to support as many targets as possible.
% % 
% % We propose a technique (or case study) on how to use program synthesis plus
% % something else to automatically learn/derive/search these implementation without
% % human intervention. We show that this approach cannot only be leverage by reticle-like
% % languages, but also other languages like calyx or dialects in circt. These languages
% % now can be lowered directly to FPGA primitives without relying on traditional
% % hardware synthesis, and target at the same time all these new FPGA architectures that
% % are going to be available (we can lean hard on the fact that people are building
% % their own FPGAs now because of OpenFPGA frameworks and this is not a story
% % of Amd and Intel anymore). The more the targets the better it is to have a technique
% % that automatically figure all this out.
% % \hl{say "dialect", people like that}
% % 
% % Maybe we can say also that another benefit of this work is that equivalence
% % checking is no longer required because the process of translating an intermediate
% % language to FPGA primitves is now sound, due to program synthesis, compared
% % to traditional hardware synthesis. I am not so sure about this but we can
% % see how the stoke paper was written.
% % 
% % \hl{luis end}
% 
% 
% \hl{The rest of this paper is organized
%   as follows...}

==> text/old-overview.tex <==
{\Large OLD OVERVIEW}
%\section{Overview}
%\label{sec:overview}

\begin{figure}
    \centering
    \includegraphics[width=.8\columnwidth]{assets/lakeroad-diagram.drawio.png}
    \caption{\lr system diagram. \hl{instr. spec should be removed, remove design fragment?}}
    \label{fig:lakeroad-diagram}
\end{figure}
  
\cref{fig:lakeroad-diagram}
  illustrates \lr's high-level design.
In this section we discuss the design components,
  and we illustrate \lr's flow with
  an example mapping a MAC (multiply accumulate) onto
  a Xilinx Ultrascale+ DSP48E2.
\hl{change running example to something that doesn't work on Vivado}
  
\lr takes three inputs:
  (1) an \textit{HDL module} specifying
    the FPGA program 
    to be implemented
    for a given architecture,
  (2) an \textit{architecture description} YAML file
    that describes the ports and parameters
    of an architecture's 
    hardware primitives,
  and (3) \textit{vendor-provided Verilog models}
    for the target FPGA architecture.
\hl{Which are user provided?}
\hl{the three inputs come from three different places: hdl model written by user, arch description written by...lakeroad maintainers? and vendor-supplied verilog. This might need a separate sentence.}
% The HDL module is the design which the low-level
%   Verilog will implement.
% The architecture description is a short configuration file
%   describing the ports/parameters of architecture-specific
%   hardware primitives.
% Lastly, the vendor-provided
%   Verilog models correspond to the implementations of
%   architecture-specific primitives
%   (e.g., \texttt{DSP48E2.v} on Xilinx).

These inputs are passed to the \lr pipeline,
  which is responsible for mapping the high-level
  HDL module to an architecture-specific
  implementation.
\cref{fig:firstpage} gives an example
  of \lr's inputs for
  implementing a MAC on a Xilinx
  Ultrascale+ DSP48E2,
  and the resulting
  output.
  
The \lr pipeline consists of
  three main components:
  \textit{sketch generation},
  \textit{program synthesis},
  and \textit{HDL compilation},
  which
  we now describe 
  in greater detail.
 % Together with automated semantics extraction
 %  from vendor-supplied Verilog models of
 %  target FPGA primitives, or manual effort from the user.
  
% \lr takes as input
%   (1) a high-level specification of an instruction,
%   (2) a description of a target FPGA architecture, and
%   (3) vendor-provided Verilog
%   models of the target FPGA's combinational primitives.
% Given these inputs,
%   \lr automatically generates
%   an implementation of the instruction
%   in low-level, architecture-specific
%   Verilog.


\subsection{Sketch Generation}

\lr uses the HDL module and
  the architecture description
  to perform
  \textit{sketch generation}.
Sketch generation
  specializes architecture-independent
  representations of FPGA programs, called
  \textit{sketch templates},
  into architecture-dependent
  \textit{program sketches}.

A \textit{sketch template} specifies
  the \textit{structure}
  of an
  FPGA program
  without specifying
  low-level details;
  rather than describing the concrete
  computations that an FPGA will
  perform, a sketch template describes
  how a program should wire together
  abstract computational components
  called \textit{primitive interfaces}.
In particular,
  sketch templates do \textit{not} specify
  the configurations of programmable
  primitives like LUTs or DSPs. 
Sketch templates also permit 
  some flexibility in wire routing,
  allowing for different common
  wiring patterns
  (e.g., reversing)
  to be explored
  during program synthesis.
\lr
  includes a series of default
  sketch templates,
  but a user can easily add their own if needed.

\hl{Would it be useful to draw parallels 
  between sketches and things similar to sketches
  in existing tools? E.g. Yosys essentially
  has sketches as the right-hand sides of its
  rewrites.}
To synthesize a MAC operation onto a DSP48E2,
  the \texttt{dsp} sketch template would be employed.
  This sketch template is quite simple, and consists of the
  primitive interface of a generic DSP with two inputs and an output.
  The DSP primitive interface does not include any information
  about the internal ports/parameters, as those are architecture-specific.
  
% \lr provides a default set of
%   sketch templates,
%   but a user may
%   define their own
%   if needed.

% In the case of synthesizing a MAC operation,
%   the sketch template would consist of an
%   architecture-agnostic representation of a DSP.
%   The sketch generation process would specialize
%   this template to a representation of a Xilinx-specific
%   DSP.
% \hl{mention how the architecture
%   description gets used here}

Although the \texttt{dsp} sketch template is simple, sketch templates can
  also represent more complex structures of primitives.
  For example, the Bitwise Sketch Template
  captures the structure of
  bitwise operations such as
  bitwise \texttt{\&}
  or bitwise \texttt{|}.
This template takes
  $k$ $n$-bit
  inputs,
  routes the $i$th bit of
  each input
  to a primitive interface
  representing an
  abstract $k$-input LUT,
  and routes the outputs
  of the $i$th LUT primitive
  interface to the $i$th output
  bit. 
  
% Using the provided architecture description,
%   \lr specializes these sketch templates
%   for specific architectures by
%   systematically expanding the abstraction
%   in terms of available primitives,
%   e.g., using a sequence of 4-bit LUTs
%   to concretely implement an abstract 6-bit LUT.
  
% Using sketch templates enables \lr
%   to abstract over common implementation strategies,
%   and thus reuse them across different FPGA architectures,
%   and reduces the input required from the user.
% Sketch templates specialized to an FPGA also serve as the
%   ``sketches'' that Lakeroad leverages during
%   sketch-guided synthesis to fill in.
% Sketches specify the overall structure of
%   a potential low-level implementation,
%   but leave unspecified ``holes'' for
%   LUT, DSP, and carry chain configuration
%   parameters which are then synthesized by
%   a reduction to a sequence of SMT solver queries~\cite{torlak2013growing}.

%\paragraph{(Example) 4-Bit Adder:}
  

% {\it (Example) 4-Bit Adder:}
%   For a more complicated example,
%   consider building a 4-bit binary adder
%   that adds 4-bit bitvectors \texttt{a} and \texttt{b}.
  
% On Xilinx's Ultrascale+ this would
%   be built with four LUT2s,
%   each with configuration
%   \texttt{.INIT(4'h6)} to compute
%   the sum bits,
%   and a CARRY8.
% The outputs of the LUT2s would
%   be wired into the CARRY8's \texttt{.S} ports,
%   and \texttt{a} would
%   be wired into the \texttt{.DI} ports
%   of the CARRY8 to allow carry bit
%   generation.
% On Lattice ECP5 this could be built
%   by connecting 4 CCU2C components
%   into an 8-bit carry chain and connecting
%   8 LUT4s with configuration \hl{specify config}
%   into the carry chain's input.

% On SOFA, which only has LUT4s and does not
%   have a fixed carry-chain unit,
%   the sum bits would be computed with
%   four frac\_lut4s (SOFA's LUT4 primitive) with
%   configuration \texttt{.sram(16'hf77f)}.
%   The outputs of these LUTs as well
%   as one of the inputs (e.g., \texttt{a})
%   would be passed into a complicated
%   carry-chain structure
%   built from frac\_lut4s.
  
% Details differ between architectures but
%   both programs share a common shape:
%   both have four LUTs feeding into a
%   carry chain structure.
% A sketch template captures this
%   similarity by specifying that it wants four LUTs fed
%   into a carry chain.
% It does \textit{not} detail 
%   which FPGA components will be used, or
%   what their configurations will be.\hfill $\qed$

% \hl{is this qed intentional?}

Sketch generation then
  specializes
  sketch templates
  to partially complete
  architecture-specific
  FPGA programs called
  \textit{program sketches}. A program sketch
  contains \textit{holes};
these holes allow flexibility
  in potential program implementations
  and will be filled in later by the Program
  Synthesis component.

% This is repetitive?
A program sketch, like a sketch template, still
  represents the \textit{shape} of an FPGA program
  rather than the program itself:
  while it is now FPGA-specific,
  many of the computational
  components in a program
  sketch are unconfigured,
  and retains the
  same flexibility
  in wire routing
  choices that
  existed in the
  sketch template.
  
With a Xilinx architecture description, sketch
  generation would convert the DSP primitive interface
  to a partially complete representation of the DSP48E2.
  The ports and parameters at this point would be included
  in the representation, but their configuration would
  remain symbolic and need to be solved during Program
  Synthesis.
  
% \lr's templates capture common 
%   implementation patterns
%   used in FPGAs.
% For example,
%   to implement multiple-bit
%   logic operations
%   like 
%   \texttt{a \&\& b}
%   on most FPGAs,
%   the common strategy is to use
%   a one Look-up Table (LUT)
%   per pair of bits,
%   e.g.~\texttt{LUT(a[0], b[0])},
%   \texttt{LUT(a[1], b[1])},
%   and so on.
% Arithmetic operations
%   are implemented similarly,
%   but with an arithmetic carry chain
%   to carry information between bits.
% \lr's templates
%   capture these high-level patterns
%   in an architecture-independent way.

% \lr's templates rely on \textit{primitive interfaces}
%   that represent computations in
%   an architecture-independent way.
% For instance, the LUT-$n$ primitive
%   interface represents
%   an $n$-input 1-output lookup table,
%   and the Carry-$n$ represents an $n$-bit
%   carry chain.
% Architecture descriptions provide implementations
%   for primitive interfaces.
% These implementations may be done with a
%   single hardware primitive
%   or with a combination of hardware
%   primitives.
% \lr also provides logic to perform common
%   primitive combinations, such as
%   recursively building
%   a larger LUT from smaller LUTs.
  

% \textit{Sketch generation}
%   transforms a template to
%   a \textit{sketch}.
% A sketch is a \lrir program with
%   \textit{holes}, or symbolic values
%   that will be later filled in by
%   synthesis to make a concrete \lrir program.
% Sketch generation 
%   queries an
%   \textit{architecture configuration}
%   to find architecture-specific
%   implementations for a
%   template's primitive interfaces.
% These implementations may still be
%   symbolic (that is, they may have holes).

\subsection{Program Synthesis}
\lr uses \textit{sketch-guided program synthesis}~\cite{??}
  to find a low-level, architecture-specific
  FPGA implementation.
Sketch-guided program synthesis is a
  technique that uses a solver
  to look for values to fill in
  a sketch's holes so that it
  implements the specified instruction. For a MAC,
  the end result of program synthesis would be a
  correct configuration of the ports/parameters of
  the DSP48E2 that would implement the operation.

Sketch-guided program synthesis
  requires an interpreter to define
  the semantics of the language that
  the sketch is written in, and
  this usually requires up-front
  investment from
  the user.
This is often a barrier to
  entry and is not an option
  for our use-case.
To avoid this problem, \lr
  \textit{automatically constructs}
  an interpreter by
  (i) providing a base interpreter
  that specifies all
  FPGA-independent semantics
  (e.g., wiring operations, etc),
  and
  (ii) \textit{automatically importing}
  the semantics of FPGA-specific primitives
  from vendor-supplied Verilog models;
A user only
  needs to provide
  a high-level
  description of 
  the target FPGA
  architecture rather
  than explicitly
  writing the interpreter.


This final program will be in \lrir,
  \lr's domain-specific synthesis language.
Both sketch templates and program sketches
  are partial \lrir programs.
  
\subsection{HDL Compilation} 

After program synthesis,
  the \lrir program has filled in all holes
  corresponding to programmable primitive configuration and thus represents a complete low-level design.
Finally, the \lrir program
  is compiled to a HDL that can
  be placed on the physical FPGA.
This compilation is purely syntactic:
  it does no optimization and simply
  maps from one structure to another.
This translation is a simple
  one-to-one correspondence to
  help ensure the correctness
  of the \lrir implementation
  and the compiled HDL program.
For a MAC, this would be a conversion from \lrir to
  the corresponding low-level Verilog.

%\section{\ThePlatonicApproach{} (old)}
%\label{sec:overview}
%
%In this section we introduce \textit{\theplatonicapproach{}}, a novel approach for
%automatically implementing ISA instructions for a target FPGA architecture from
%formal models of the ISA instructions and of  the target architecture.
%%
%\note{Note: I want \theplatonicapproach to include the DSL...THIS IS PART OF THE TECHNIQUE! How do we phrase this?}
%Central to \ThePlatonicApproach is a \textit{customizable} and \textit{extensible} domain specific language (DSL).
%%
%Here is an outline of \theplatonicapproach:
%\begin{itemize}
%    \item A user encodes formal models of each target ISA instruction in the DSL
%    \item The user models \textit{primitives} for the target FPGA architecture by extending the DSL
%    \item \note{are users providing templates/search spaces for the program we are synthesizing? should we be explicit here?}
%    \item \Theplatonicapproach invokes an SMT solver to find a program in the DSL that
%          implements the encoded ISA instruction for the FPGA architecture
%\end{itemize}
%\note{\ldots just a solver? why \textit{constrain}  ourselves (yuk yuk yuk) to SMT solvers?}
%
%\hl{
%System diagram
%
%non-eval contributions explained at a high level
%
%when you finish the overview, you should have an idea of the blocks within lakeroad, but you shouldn't know how they're implemented.
%
%want to mention that it's solver aided
%
%
%what do we care about/what do we want people to continue caring about for the next n years
%
%we want people to care that this is solver-aided
%
%we want people to care that it is user-extensible, to easily support new architectures
%}
%
%\hl{put synthesis statement in overview:}
%FIND \textit{init}\ .\ $\forall a,b,c,d$\ .\  lut(a,b,c,d, \textit{init}) == bvand(a, b)

==> text/old-proof.tex <==

\begin{lemma}
    \label{lemma:non-termination-of-rule-implies-recursive-call}
    If \textsc{Interp} fails to execute
    on node $n$, then this non-termination
    must be due to a recursive call to 
    \textsc{Interp}.
\end{lemma}
\begin{proof}
Suppose $\textsc{Interp}(p,e,t,n)$
    fails to terminate.
$n$ is one of five types of nodes:
    $\SynBv$,
    $\SynVar$,
    $\Op$, 
    \IRReg,
    and \IRPrim;
    \textsc{Interp} is not defined for holes
    $\blacksquare_{x_i}$.
    
Interpreting a $\SynBv$ node
    returns a bitvector constant,
    and this terminates.

Interpreting a $\SynVar$ node
    performs an environment
    lookup.
An environment is formed either by an
    explicit mapping of
    variables to concrete streams,
    or by the lambda abstraction
    in the rule for primitives.
Looking up a concrete mapping always
    terminates.
Executing the body of lambda abstraction
    formed in the primitives rule
    involves a single recursive call to \textsc{Interp},
    so if this abstraction fails to terminate
    it must be from a non-terminating recursive call.
    
Interpreting a \IRReg{} node when time $t=0$
    returns a bitvector constant, which terminates.
Interpreting a \IRReg{} node when time $t > 0$
    involves a single recursive call to \textsc{Interp};
    thus if execution fails to terminate then this
    recursive call must fail to terminate.

Interpreting an $\Op$ node performs a
    map of recursive calls to \textsc{Interp}
    to a finite list of operands,
    and then applies the semantics 
    of $\llbracket op \rrbracket$
    to the result.
Mapping function $f$ over a finite list $xs$ always
    terminates whenever $f$ is guaranteed to
    terminate, so for our map invocation to
    diverge, one of the recursive
    calls to \textsc{Interp}
    must fail to terminate.
Computing the operator semantics
    $\llbracket op \rrbracket$
    could fail to terminate in theory,
    but in practice these operators are
    simple bitvector operations
    and always terminate (e.g., bitvector addition).
    
Interpreting a \IRPrim{} node
    performs lambda abstraction and then
    passes the abstraction to a recursive
    call to \textsc{Interp}.
Lambda abstraction always terminates.
Thus, if interpreting a primitive node
    diverges this must be due to the
    recursive call failing to terminate.

This, if $\textsc{Interp}(p,e,t,n)$ fails to
    terminate, this must be due to a non-terminating recursive
    call to \textsc{Interp}, as was to be shown.
\end{proof}

We define a \textit{recursive call sequence}
    to be (possibly infinite) sequence of \textsc{Interp} executions 
    $\{\mathcal{I}_i\}$,
    where  $\mathcal{I}_i = \textsc{Interp}(p_i, e_i, t_i, n_i)$
    for some $p_i$, $e_i$, $t_i$ and $n_i$,
    such that $\mathcal{I}_i$ recursively invokes $\mathcal{I}_{i+1}$,
    such that the final execution $\mathcal{I}_f$ in the sequence,
    if it exists,
    does not recursively call \textsc{Interp}.
We say that a recursive call sequence $\{\mathcal{I}_i\}$ is
    \textit{divergent} if all $\mathcal{I}_i$ are divergent.
\begin{lemma}
    \label{lemma:non-termination-implies-infinite-recursion}
    A recursive call sequence of finite length cannot be divergent.
\end{lemma}
\begin{proof}
Let $\{\mathcal{I}_i\}$, $i = 1\ldots L$, be a finite length
    recursive call sequence.
By definition the final execution $\mathcal{I}_L$
    must not recursively call \textsc{Interp},
    and by Lemma~\ref{lemma:non-termination-of-rule-implies-recursive-call}
    $\mathcal{I}_L$ must terminate,
    and $\{\mathcal{I}_i\}$ is not divergent.
\end{proof}

\begin{lemma}
    If executing $\textsc{Interp}(p, e, t, n)$ diverges,
    then there must exist an infinite recursive call sequence
    $\{\mathcal{I}_i\}$ 
    starting with $\mathcal{I}_1 = \textsc{Interp}(p, e, t, n)$.
\end{lemma}
\begin{proof}
We prove by contradiction.
Suppose executing $\textsc{Interp}(p, e, t, n)$ diverges,
    and suppose that all recursive call sequences
    starting with $\mathcal{I}_1 = \textsc{Interp}(p, e, t, n)$ do
    not diverge.
An infinite length recursive
    call sequence corresponds to
    infinite recursion which is divergent,
    and so all recursive
    call sequences starting with $\mathcal{I}_1$
    must have finite length.

\end{proof}


\begin{lemma}
    \label{lemma:infinite-recursion-impossible}
    If program $p$ is well-formed, then
    $\textsc{Interp}\ p\ e\ t\ p.root$
    cannot recurse infinitely.
\end{lemma}
\begin{proof}
We prove by contradiction.
Suppose 
    $\textsc{Interp}(p, e, t, r)$ diverges.
Let $T$ be the execution tree
    defined by the divergent execution
    of $\textsc{Interp}(p, e, t, r)$,
    whose (1) tree nodes are the 
    individual executions of \textsc{Interp}
    on the program nodes of $p$,
    and (2) edges between
    tree nodes $N_i$ and $N_j$ are
    recursive invocations of \textsc{Interp}.
Since \textsc{Interp} can execute
    on a single program node $n_i$ multiple times,
    a program node $n_i$ can correspond to
    multiple tree nodes $N_{n_i, 1}, N_{n_i, 2}, \ldots$,
    one for each time \textsc{Interp}
    executes on $n_i$.
From the preceding arguments, the execution of each
    tree node is finite.
Since execution diverges, 
    $T$ must be \textit{infinite}
    and in particular have
    infinitely many tree nodes.

Each rule for \textsc{Interp}
    directly invokes \textsc{Interp} finitely
    many times, so each tree node has
    finitely many children.
This implies that for $T$
    to be infinite, it
    must have infinite depth,
    and it follows that
    there exists
    an infinite path
    $P$ through $T$.
Since our program $p$ has finitely many nodes,
    there must be program node $n$
    that is executed infinitely many
    times in path $P$ via nodes
    $N_{n,1}, N_{n,2}, \ldots$
This and well-formedness rule
    \textbf{W6} imply the existence
    of infinitely many tree nodes
    $N_{r,1}, N_{r,2}, \ldots$
    in $P$ corresponding to the
    execution of register program nodes.
There are two cases: $n$ itself is a
    register node, or
    $n$ is not a register node.
If $n$ is a register node, then
    our claim trivially holds:
    it exists within infinitely many tree
    nodes $N_{n,1}, N_{n,2}, \ldots$
    in $P$, and we are done.
Otherwise, $n$ is not a register node,
    and $n$ has a self-dependency.
By \textbf{W6}, program $p$ cannot have combinational
    cycles, meaning self-dependencies
    must be broken by a register
    node, and each subpath in $P$
    starting and ending with an execution of $n$
    must contain the execution of a register.

But a path through an execution tree
    cannot contain infinitely many register nodes:
    each execution of a register node decrements
    time, and no rules in \textsc{Interp} ever
    increment a time value.
Since time at the top of the path must
    be some natural number $t_P$, the path
    contains at most $t_P + 1$ register nodes.
This contradicts that $P$ has infinitely many
    register nodes: $P$ must be finite,
    $T$ must be finite,
    and $\textsc{Interp}(p, e, t, r)$
    must terminate when $p$ is free
    of combinational cycles.
\end{proof}


{\color{green}
THE FOLLOWING IS AN OLD PROOF THAT WE CAN RECYCLE, ARGUING THAT ROSETTE TERMINATES. WE DONT WANT TO MAKE IT A THEOREM, SO INSTEAD THIS WILL BE A PROSE ARGUMENT
\begin{proof}
Rosette searches through
  all possible ways of
  filling in a sketch's holes
  and uses \textsc{Interp} to
  check if the resulting program
  is equivalent to the behavioral
  specification.
There are finitely many holes,
  and each hole has
  finitely many possible completions.
Thus there are finitely many ways to
    fill the holes of a sketch,
    and as long as \textsc{Interp} always
    terminates, Rosette's synthesis query
    is guaranteed to terminate, and the
    entire search space can in theory
    be explored.

To show that \textsc{Interp} is guaranteed
    to terminate on well-formed programs,
    we show two intermediate results,
    proved below: 
    %
    (i) non-termination of \textsc{Interp}
    implies infinite recursion, 
    (Lemma \ref{lemma:non-termination-implies-infinite-recursion}),
    %
    and (ii) infinite recursion is impossible on
    a well-formed program
    (Lemma \ref{lemma:infinite-recursion-impossible}).
These two facts 
    combine to imply that \textsc{Interp}
    is guaranteed to terminate on well-formed
    programs.
\end{proof}
}

==> text/old-quality-of-outputs.tex <==
\subsection{Quality of Output}
To evaluate the quality of \lr's output,
  we compare \lr against four tools---%
  Yosys,
  Vivado,
  Diamond,
  Quartus---%
  on the task of mapping
  a set of benchmark designs
  to DSPs
  on three FPGA architectures---%
  Xilinx UltraScale+,
  Lattice ECP5,
  \hl{todo intel something?}.
Note that we do not include
  SOFA,
  as the SOFA architecture
  does not include DSPs.

Our set of DSP benchmarks
  is assembled from GitHub.
Using GitHub's advanced search tool,
  we searched through Verilog projects
  on GitHub
  which had submodules
  intended to be compiled onto
  the DSPs of various FPGA platforms.
These submodules were identified
  in a number of ways:
  for example, by searching for
  the Xilinx-specific
  \texttt{(* use\_dsp = "yes" *)}
  annotation.
We attempt to compile \textit{every}
  benchmark
  on \textit{every}
  architecture,
  although most benchmarks
  were written
  for a specific FPGA architecture.

\cref{tab:dsp-benchmarks}
  shows our results.
  
\hl{We are comparable in quality to
  existing, proprietary tools.}

\hl{We enable broader support
  for targeting DSPs
  in open-source tools like Yosys.}




  
Furthermore, to highlight \lr's
  utility to existing open-source tools,
  we directly integrated 
  integrated \lr 
  into Yosys
  as the 
  \texttt{\lowercaselr}
  subcommand,
  using only 75 lines
  of C++.
Thus, when we mention
  \lr in this section,
  we actually mean
  the
  \texttt{\lowercaselr}

\hl{The below section is  text from the old
``support for complex primitives'' section.
Tasks: (1) determine whether to keep
the stuff about yosys integration,
or where else we might put it
(2) fold the ``synthetic'' benchmarks 
into our benchmark suite, if we don't find
existing benchmarks that do those things
}


In this section,
  we evaluate \lr's ability
  to utilize complex FPGA primitives.
To do so,
  we integrated \lr 
  into Yosys
  as the 
  \texttt{\lowercaselr}
  subcommand,
  using 75 lines
  of C++.
We then compare 
  the output of the 
  \texttt{\lowercaselr}
  subcommand
  against the output of
  Yosys's existing
  \texttt{synth\_xilinx}
  and
  \texttt{synth\_ecp5}
  subcommands,
  which target Xilinx UltraScale+
  and Lattice ECP5
  respectively.
These results highlight how \lr's approach
  enables providing high-quality technology mapping
  in Yosys with little manual implementation effort,
  suggesting ease of adding support for new
  future FPGA architectures.

To evaluate \lr's ability
  to map to complex primitives
  on Xilinx UltraScale+,
  we use the
  \texttt{\lowercaselr}
  and 
  \texttt{synth\_xilinx}
  subcommands
  to attempt to map
  a set of Verilog modules
  to an UltraScale+ DSP.
Specifically,
  our set of modules
  implement the set of computations
  listed in tables 2-1 and 2-2
  of Xilinx's
  UltraScale Architecture DSP Slice User Guide~\cite{userguide}.
These tables list
  the functions implemented
  by the UltraScale+ DSP;
  thus, we know that all of
  the modules in our set
  should map one-to-one
  to UltraScale+ DSPs.
  
The results for UltraScale+
  are listed in
  \cref{tab:yosys-xilinx}.
As you can see,
  the \texttt{\lowercaselr}
  subcommand of Yosys
  is able to map all expressions
  to a single DSP
  by automatically determining
  the correct configuration
  of the DSP's 20+ ports
  and 40+ parameters.
Meanwhile,
  Yosys's
  \texttt{synth\_xilinx}
  can only map to DSPs
  via manually written
  patterns,
  and currently, 
  Yosys only implements patterns
  for mapping multiplication.
Thus,
  \texttt{synth\_xilinx}
  is able to capture the multiplication
  portion of each target module,
  but it maps the rest of the computation
  (e.g., additions, subtractions,
  or logic functions)
  to LUTs and carry chains.
Note that the runtimes
  of the two passes are comparable,
  except in the case of the $(a-b)^2-c$
  expression,
  when the \texttt{\lowercaselr}
  subcommand
  is an order of magnitude slower;
  we speculate this is due to unpredictable
  behavior in the underlying SAT solver.
  
To evaluate \lr's ability
  to map to complex primitives
  on Lattice ECP5,
  we use the
  \texttt{\lowercaselr}
  and 
  \texttt{synth\_ecp5}
  subcommands
  to attempt to map
  a set of Verilog modules
  to a Lattice ECP5 DSP.
The Lattice ECP5 DSP
  is split into multiple primitives;
  we evaluate \lr's ability to map
  to the multiplier (MULT18X18D)
  and ALU (ALU24B) primitives.
The results are shown
  in \cref{tab:yosys-lattice}.
Similar to the Xilinx UltraScale+ results,
  we demonstrate that 
  Yosys's \texttt{synth\_ecp5}
  subcommand
  fails to map all expressions
  to the ECP5 DSP,
  with some of the computation
  being implemented onto CCU2Cs.
Note that
  \texttt{\lowercaselr}
  uses 1 multiplier and 1 ALU
  for the expression $a \times b$,
  while \texttt{synth\_ecp5}
  correctly uses just a single multiplier.
  this is because \lr's DSP sketch
  always instantiates both
  a multiplier and an ALU.
Detecting when the ALU is not necessary
  can be implemented using optimization features
  of modern SAT and SMT solvers;
  we leave this development
  for future work.
  
\begin{table}
    \centering
    \begin{tabular}{c|c}
    \end{tabular}
    \caption{Completeness of \lr against other tools.}
    \label{tab:mylabel}
\end{table}

We also demonstrate \lr's robustness across workloads
  compared to SOTA synthesis tools on three architectures. 
On a number of benchmarks, \lr succeeds in mapping 
  to DSPs compared to Yosys, and the architecture's corresponding proprietary synthesis tool.

%\subsection{RQ5: Usability by Real Frameworks}
%\label{sec:rq5}
%
%To demonstrate the ease of integrating \lr output with existing tools we
%replace the ISA implementations of the Calyx compiler with \lr's output.
%Calyx~\cite{nigam2021compiler}
%  is a language
%  and compiler
%  for hardware designs.
%  it supports multiple frontend languages,
%  including their own Calyx
%  language,
%  Dahlia~\cite{nigam2020predictable},
%  and TVM~\cite{chen2018tvm}.
%Calyx
%  compiles designs
%  into synthesizable,
%  architecture-independent
%  behavioral Verilog,
%  relying on hardware synthesis tools
%  to finish compilation
%  to the target FPGA
%  (currently, they focus on
%    Xilinx boards).
%
%To test correctness,
%  we run the modified Calyx's entire 
%  test suite
%  and ensure all tests pass.
%\hl{Do any of the tests
%  actually test the resulting Verilog?
%  Yes, I'm fairly certain a number of them
%  Verilate the code and simulate
%  and check the results.
%  So we need to make sure we say that,
%  in case a reviewer thinks
%  that the tests will pass no matter
%  what.}
%
%To test performance,
%  we compile smaller sample Calyx programs
%  found within Calyx's test suite,
%  and larger hardware designs
%  found in Calyx's evaluation repository. 
%We then run Calyx's
%  of Calyx's test suite
%  and evaluation,
%  allowing us to compile 
%  
%
%The purpose of our end-to-end
%  evaluation
%  is not to demonstrate
%  improved performance.
%To truly compete
%  with legacy logic synthesis
%  and optimization,
%  we would need an entire
%  FPGA compiler pipeline
%  designed to target an ISA
%  and with built-in 
%  optimization passes.
%Calyx includes optimization
%  passes \hl{(is that true?)},
%  but still relies on
%  hardware synthesis tools
%  like Vivado
%  for final optimization.
%Instead, we aim to match
%  previous performance,
%  while demonstrating
%  the ease of integration of an ISA
%  with a toolchain,
%  implying that future FPGA compilers
%  can gain the benefits of \lr-generated
%  ISAs
%  (quick support of new architectures,
%    multiple implementations of instructions,
%    etc.)
%    
%Note that our
%  ISA does not cover
%  the entire Calyx ISA.
%Notably,
%  we do not cover
%  their register-/memory-related
%  instructions.
%We also do not
%  support 
%  instructions
%  outside of their
%  ``core'' ISA;
%  i.e.~we do not
%  cover their
%  math instruction set.
%
%\subsection{Pareto Frontier Exploration}
%
%\hl{
%This might not need to be 
%  its own subsection,
%  but we need to highlight
%  the ability
%  to generate multiple implementations
%  per instruction.}


\hl{
The below text is from the 
``proof of concept''
section added during response.
(1) fold the table into the new DSP benchmark 
table.
(2) determine what text below we should keep.
}

\begin{table}[]
\hl{Fold this into DSP benchmark suite}
    \normalsize
    \centering
    \caption{
Synthesizing sequential designs
  onto a Xilinx DSP48E2
  using our approach.
All designs are 16 bit.}
    \label{tab:sequential}
    \begin{tabular}{c|c}
\hline
design & synthesis time (s) \\
\hline
2-stage $a\times b + c$ &  3.3 \\
3-stage $(a + b) \times c + d$ &  3.4 \\
3-stage $(a + b) \times c \oplus d$ &  3.3 
    \end{tabular}
\end{table}
  
The techniques presented
  can be applied to sequential logic
  as well.
Our method for extracting semantics 
  from Verilog
  (\cref{sec:implementation:importing-semantics})
  converts Verilog to the btor format~\cite{btor},
  which natively supports
  sequential logic
  with its \texttt{state} and \texttt{next}
  expressions.
This, in combination with 
  modifications to \lrir,
  enable support for synthesizing
  sequential logic.
A full handling
  of large sequential designs
  requires techniques
  in addition to just program synthesis:
for example,
  using richer 
  hardware design languages
  to convey timing information, 
and
  applying efficient term rewriting
  techniques
  such as equality saturation~\cite{willsey2021egg}
  to automatically decompose large designs.
We plan to present these techniques
  in future work.
Here, though, we present
  proof-of-concept evidence
  that program synthesis
  can be applied not only
  to combinational designs,
  but to sequential designs as well.

To demonstrate
  our technique's ability to handle
  sequential logic,
  we run synthesis tasks
  similar to those presented
  in \cref{tab:xilinx-resource-utilization}.
\cref{tab:sequential}
  presents the results.
Each line represents a sequential
  design which is synthesized into
  an instantiation of a Xilinx DSP48E2.
As our results show,
  we are able to map
  interesting sequential circuits,
  such as pipelined multiply--accumulators,
  onto DSPs,
  in timescales similar to those shown in
  \cref{tab:xilinx-resource-utilization,tab:lattice-resource-utilization,tab:sofa-resource-utilization,tab:yosys-lattice,tab:yosys-xilinx}.



